The spectral energy distributions of K+A galaxies from the UV to the mid-IR: stellar populations, star formation and hot dust

We present spectrum synthesis fits to 808 K+A galaxies selected from the Sloan Digital Sky Survey (SDSS) and population synthesis of their spectral energy distributions, extending from the far UV (0.15 micron) to the mid IR (22 micron), based on the results of STARLIGHT code fitting to the SDSS spectra. Our modelling shows that K+A galaxies have undergone a large starburst, involving a median 50% of their present stellar masses, superposed over an older stellar population. The metal abundance of the intermediate-age stars shows that star formation did not take place in pristine gas, but was part of a dramatic increase in the star formation rates for originally gas-rich objects. We find no evidence for on-going QSO activity in the UV, which is well modeled by the emission of intermediate-age stars. We use K+A galaxies as local counterparts of high redshift objects to test for the presence of Thermally Pulsing AGB stars in similarly-aged populations and find no excess in the infrared due to emission from such stars, arguing that more distant galaxies are indeed old and massive at their redshift. All of our galaxies show significant excesses in the mid-IR compared to the light from their stars. We fit this ad hoc with a 300K blackbody. Possible sources include TP-AGB stars, obscured young star clusters and hidden AGNs, heating a significant dust component.

==> pops.tex <==
#lista                 vname      _zz  _MTOT    _Av   _AvF _N2_Ha   _WHa   _WO3   _WO2 _young i_poor  i_sol i_rich o_poor  o_sol      o_rich
#
   1& 001027.392-104341.71&  0.1329&  20.9&  0.32&  0.08&   1.2&   4.9&   7.6&   2.3&   0.0&  23.4&   0.5&  37.5&   8.4&   0.0&  30.2 \\ 
   2& 001551.253-102317.92&  0.1982&  26.9&  0.38&  0.10&   1.0&   1.1&  -0.2&   1.4&   0.2&   3.7&   0.0&  85.4&   0.1&  10.2&   0.0 \\ 
   3& 010823.370-094356.22&  0.1834&  40.0&  0.07&  0.17&   1.4&   0.7&   0.4&   0.4&   0.1&   5.0&   0.3&  30.2&  10.1&  46.5&   7.7 \\ 
   4& 011942.227+010751.63&  0.0900&  24.9&  0.05&  0.05&   0.3&   1.8&  -0.2&   1.9&   0.2&   7.7&   0.9&   6.1&   3.7&  28.8&  52.0 \\ 
   5& 012015.683-095920.12&  0.1369&  25.5&  0.03&  0.14&   2.5&   0.6&   0.2&   1.5&   0.4&  12.9&   0.9&  37.8&  11.6&  35.5&   0.0 \\ 
   6& 014327.340-011342.55&  0.1963&  59.7&  0.20&  0.04&   1.5&   4.2&   5.2&   2.1&   0.1&   5.5&   0.4&   9.7&  26.9&  28.6&  27.8 \\ 
   7& 014838.633-093259.77&  0.2170&  29.1&  0.16&  0.05&   1.8&   0.8&   0.3&   3.1&   0.4&  21.0&   0.0&  73.1&   0.0&   2.6&   0.0 \\ 
   8& 015107.018-005636.72&  0.1981&  29.7&  0.10&  0.04&   1.3&   0.9&  -0.2&   0.5&   0.0&  18.3&   1.2&  68.9&  11.6&   0.0&   0.0 \\ 
   9& 020505.984-004345.25&  0.1134&  16.8&  0.56&  0.01&   0.6&   4.5&   0.9&   3.5&   0.2&   8.4&   0.3&  25.6&  34.6&  20.8&   9.4 \\ 
  10& 021007.624-095431.19&  0.0412&   1.9&  0.34&  0.01&   0.4&   4.2&   0.5&   4.6&   0.1&  12.7&   0.0&   3.6&  81.6&   2.1&   0.0 \\ 
  11& 022427.085-093739.48&  0.0883&   7.9&  0.08&  0.04&   1.9&   1.0&   0.9&   1.9&   0.0&   7.5&   2.8&  89.8&   0.0&   0.0&   0.0 \\ 
  12& 022743.211-001523.04&  0.2192&  65.6&  0.34&  0.04&   1.1&   3.4&  -0.1&   1.5&   1.1&   4.1&   3.4&  46.4&   8.1&  34.3&   0.0 \\ 
  13& 022957.373-005412.86&  0.0859&  11.1&  0.37&  0.03&   0.8&   5.0&   1.3&   1.6&   0.0&   4.9&   0.0&  34.4&  60.7&   0.0&   0.0 \\ 
  14& 023446.381+003035.87&  0.1405&  10.4&  0.06&  0.03&   1.6&   1.0&   0.5&   1.6&   0.0&  23.0&   0.0&  77.0&   0.0&   0.0&   0.0 \\ 
  15& 025203.278-081839.42&  0.1977&  45.1&  0.29&  0.13&   2.0&   0.9&   0.8&   1.3&   0.1&   5.5&   0.5&  55.6&   0.0&  37.5&   0.2 \\ 
  16& 025559.311-010823.08&  0.1937&  35.8&  0.50&  0.17&   1.3&   2.0&   0.2&   1.5&   0.0&  13.7&   0.0&  56.4&  29.1&   0.0&   0.0 \\ 
  17& 025850.526+003458.72&  0.1942& 131.6&  0.65&  0.21&   1.2&   5.8&   1.4&   3.6&   0.0&   8.0&   0.5&   9.8&   1.2&  12.5&  67.3 \\ 
  18& 030228.430-005618.13&  0.1684&  51.2&  0.57&  0.27&   1.3&   2.9&   0.0&   2.4&   0.1&  17.1&   1.0&  29.1&   0.0&  22.1&  29.4 \\ 
  19& 032033.650-002021.24&  0.0379&   4.2&  0.73&  0.19&   0.6&   5.8&   0.7&   6.6&   0.1&   3.2&   1.7&   8.7&  51.4&  12.4&  22.5 \\ 
  20& 073214.273+390405.81&  0.1471&  19.8&  0.23&  0.21&   1.2&   1.8&   0.1&   1.6&   0.0&   3.8&   0.0&  76.8&   0.0&  15.2&   2.5 \\ 
  21& 073420.839+314419.72&  0.0617&   6.3&  0.14&  0.16&   0.3&   1.3&  -0.3&   1.8&   0.3&   1.6&   0.0&   6.2&  22.2&   9.7&  59.8 \\ 
  22& 073537.325+393345.70&  0.1083&  30.4&  0.33&  0.32&   3.8&   0.3&  -0.3&   1.2&   0.5&   5.8&   1.5&  31.0&   4.3&  56.5&   0.0 \\ 
  23& 073724.079+382438.81&  0.1273&  26.5&  0.12&  0.25&   0.8&   1.2&   0.4&   1.4&   0.0&   1.5&   2.3&  16.1&   1.7&  65.8&  11.6 \\ 
  24& 074541.458+220821.98&  0.1229&  32.9&  0.62&  0.14&   1.9&   3.0&   0.5&   2.8&   0.3&  14.4&   1.5&  30.2&  14.8&  34.8&   0.0 \\ 
  25& 074630.900+333318.81&  0.1592&  35.0&  0.73&  0.15&   0.5&   5.1&  -0.0&   0.7&   0.0&   3.9&   0.9&  39.1&   0.0&   8.8&  47.3 \\ 
  26& 074650.321+224937.12&  0.1300&  39.7&  0.19&  0.20&   6.2&   0.1&   0.0&   0.5&   0.1&   5.2&   0.3&  39.0&  22.8&  27.6&   4.7 \\ 
  27& 074820.234+175952.67&  0.0457&   0.8&  0.20&  0.13&   0.5&   0.0&   0.3&   1.5&   0.5&  29.9&   8.0&  10.9&  50.5&   0.0&   0.0 \\ 
  28& 075056.918+480245.92&  0.0801&  14.7&  0.20&  0.30&   1.5&   0.7&   0.5&   0.1&   0.0&   5.7&   3.9&  48.1&  17.1&  22.1&   3.1 \\ 
  29& 075246.207+382928.46&  0.1268&  31.1&  0.26&  0.19&   0.6&   1.8&  -0.3&   0.7&   0.4&   1.3&   2.0&  30.9&   0.5&  63.2&   0.0 \\ 
  30& 075255.994+384330.63&  0.1263&  16.8&  0.09&  0.19&   1.8&   0.7&   0.5&   1.8&   0.1&  15.2&   4.9&  14.9&  33.4&   0.0&  31.5 \\ 
  31& 075318.070+450307.92&  0.0493&   1.7&  0.30&  0.22&   0.7&   4.2&  -0.1&   3.9&   0.2&   7.7&   2.9&  11.6&  26.9&   3.2&  47.7 \\ 
  32& 075323.098+243300.56&  0.0610&  12.7&  0.32&  0.24&   1.0&   1.1&   0.0&   0.1&   0.0&  14.9&   0.9&  76.8&   7.4&   0.0&   0.0 \\ 
  33& 075339.602+301125.88&  0.2104&  31.6&  0.25&  0.12&   1.0&   2.0&   0.2&   1.3&   0.0&  10.4&   0.8&  88.0&   0.0&   0.0&   0.0 \\ 
  34& 075423.026+375230.72&  0.1654&  49.1&  0.38&  0.20&   1.2&   3.0&  -0.1&   3.6&   0.3&   4.0&   1.4&  26.6&   3.8&   6.0&  56.5 \\ 
  35& 075440.183+124510.74&  0.2124& 101.5&  0.28&  0.08&   1.1&   1.9&  -0.1&   1.2&   0.0&   0.7&   0.7&  29.9&   0.0&  64.5&   1.5 \\ 
  36& 075528.968+213038.24&  0.2734&  43.6&  0.33&  0.21&   1.8&   1.3&  -0.5&   2.3&   0.0&   6.4&   0.0&  88.7&   0.3&   4.6&   0.0 \\ 
  37& 075658.898+362255.14&  0.1773&  70.5&  0.41&  0.20&   1.6&   1.8&  -0.4&   3.0&   0.2&   6.9&   0.4&  15.0&   0.0&  74.4&   2.0 \\ 
  38& 075710.942+142736.10&  0.1915&  44.5&  0.24&  0.08&   1.5&   1.3&   0.4&   1.4&   0.2&   2.7&   0.4&  42.8&   0.8&  40.7&  11.5 \\ 
  39& 080037.058+261356.59&  0.1765&  62.8&  0.24&  0.06&   0.5&   1.5&  -1.5&  -0.1&   0.4&   4.1&   0.1&  11.2&   0.0&  60.5&  21.9 \\ 
  40& 080103.761+344144.57&  0.1603&  59.8&  0.56&  0.19&   1.6&   2.0&   0.3&   2.0&   0.0&   6.3&   0.5&  28.6&   0.0&  45.2&  19.2 \\ 
  41& 080127.970+321017.28&  0.1897&  59.7&  0.47&  0.19&   1.6&   1.0&   0.0&   0.2&   0.2&   6.1&   0.6&  24.4&  19.1&  43.8&   4.7 \\ 
  42& 080218.394+323207.81&  0.0383&   6.6&  0.11&  0.23&   1.8&   1.2&   0.5&   2.1&   0.1&  13.3&   5.1&  48.0&  19.4&  14.0&   0.0 \\ 
  43& 080246.610+085110.92&  0.1130&  30.5&  0.14&  0.01&   1.0&   1.0&  -0.1&   0.4&   0.0&   2.3&   4.2&  52.5&   0.0&  34.0&   6.5 \\ 
  44& 080330.523+310840.02&  0.0982&  13.2&  0.96&  0.15&   0.4&   6.0&   0.8&   5.7&   0.3&  19.7&   0.0&   5.3&  22.1&  11.8&  40.9 \\ 
  45& 080346.450+291816.84&  0.1896&  65.7&  0.00&  0.12&  21.6&  -0.0&  -0.3&  -0.3&   0.0&   1.3&   1.5&  20.6&  19.2&  32.1&  25.3 \\ 
  46& 080446.742+104641.74&  0.0353&   1.7&  0.48&  0.01&   0.6&   4.7&   0.1&   1.4&   0.4&  13.3&   2.5&   2.4&  20.5&  23.1&  37.5 \\ 
  47& 080532.772+372801.05&  0.0327&   0.6&  0.19&  0.16&   0.4&   4.4&   0.7&   4.7&   0.1&   9.3&   5.1&  11.9&  73.3&   0.0&   0.0 \\ 
  48& 080725.159+362222.68&  0.1596&  25.3&  0.42&  0.14&   0.3&   1.5&  -0.1&   1.6&   0.0&  11.5&   1.0&  29.8&  16.0&  41.6&   0.0 \\ 
  49& 080738.412+385625.57&  0.0390&   4.8&  0.11&  0.18&   0.7&   2.2&   0.2&   1.6&   0.1&   7.0&   0.7&  29.8&  36.6&  22.7&   3.0 \\ 
  50& 080801.699+393145.96&  0.1217&  18.2&  0.39&  0.17&   0.8&   2.7&   0.6&   3.4&   0.2&   7.6&   5.1&  14.4&  25.1&   2.0&  42.2 \\ 
  51& 080925.082+305652.85&  0.0836&  40.3&  0.11&  0.19&   1.6&   1.9&   0.3&   2.5&   0.1&   5.3&   5.0&  21.8&  19.2&  42.2&   5.9 \\ 
  52& 081120.626+352147.40&  0.0694&   4.4&  0.28&  0.14&   1.3&   3.2&   0.6&   2.9&   1.5&   9.8&   0.4&  12.1&  23.5&  30.3&  20.4 \\ 
  53& 081412.485+103744.38&  0.0533&   4.7&  0.34&  0.06&   0.6&   3.0&   0.2&   4.9&   0.3&  13.7&   1.5&  12.3&  46.5&  25.4&   0.0 \\ 
  54& 081415.432+081359.90&  0.2449&  49.7&  0.43&  0.03&   1.5&   3.5&   1.6&   3.2&   0.0&   7.5&   1.8&  83.1&   7.1&   0.0&   0.0 \\ 
  55& 081525.771+372025.85&  0.0397&   5.0&  0.49&  0.13&   0.9&   4.6&   1.6&   1.5&   1.2&   5.5&   1.4&  21.9&  27.9&   2.0&  39.9 \\ 
  56& 081629.940+291559.34&  0.1694&  37.7&  0.73&  0.09&   1.4&   1.8&  -0.2&   1.1&   0.0&  34.4&   1.9&  52.7&   0.0&   0.2&  10.8 \\ 
  57& 081641.124+221847.78&  0.1675&  75.0&  0.97&  0.14&   0.8&   3.9&   0.2&   2.6&   0.2&   8.0&   2.1&  16.4&   2.0&  18.8&  52.1 \\ 
  58& 081802.412+281232.23&  0.1287&  20.8&  0.27&  0.09&   0.9&   2.7&   0.6&   2.3&   0.0&   5.1&   2.5&  35.1&  14.1&  33.0&   9.0 \\ 
  59& 081912.014+405856.41&  0.2357&  94.6&  0.34&  0.14&   0.8&   4.0&   0.3&   1.8&   0.1&   0.2&  14.2&  10.4&  34.1&   0.0&  40.7 \\ 
  60& 081922.205+062523.11&  0.1343&  15.0&  0.33&  0.03&   1.0&   2.0&   0.1&   2.4&   0.0&  12.4&   0.0&  52.8&   8.5&  26.1&   0.0 \\ 
  61& 081936.794+282405.62&  0.1623&  20.2&  0.37&  0.06&   2.5&   0.9&   0.6&   2.1&   0.0&  44.8&   0.0&  55.2&   0.0&   0.0&   0.0 \\ 
  62& 081953.532+041409.22&  0.2966& 152.1&  0.29&  0.04&   1.2&   4.8&   3.0&   2.3&   0.4&   0.0&   1.5&   9.1&   1.6&   0.0&  73.8 \\ 
  63& 082134.238+432301.03&  0.2280&  30.4&  0.45&  0.26&   1.4&   3.4&   0.6&   3.5&   0.0&   3.6&   0.4&  94.7&   0.0&   0.0&   0.0 \\ 
  64& 082254.881+192128.22&  0.0626&   7.2&  0.85&  0.14&   0.6&   3.4&   0.9&   1.4&   0.1&  13.6&   0.1&   5.5&  69.5&   0.0&  11.0 \\ 
  65& 082518.910+412039.78&  0.1533&  15.4&  0.17&  0.16&   1.2&   1.9&   0.4&   2.6&   0.0&  18.8&   0.0&  74.3&   6.6&   0.0&   0.0 \\ 
  66& 082655.471+135059.51&  0.3937&  48.6&  0.55&  0.12&  64.6&   0.0&   0.4&   2.0&   0.0&   9.7&  21.1&  69.3&   0.0&   0.0&   0.0 \\ 
  67& 082752.838+260502.48&  0.0958&   7.9&  0.37&  0.10&   0.9&   2.6&   0.3&   2.7&   0.3&  19.1&   4.1&  43.9&  31.1&   0.0&   0.0 \\ 
  68& 082858.685+274101.33&  0.0569&   8.3&  0.14&  0.10&   0.8&   3.2&   0.5&   4.8&   0.2&   7.8&   6.6&  10.1&  48.6&  16.5&  10.2 \\ 
  69& 082930.302+350216.51&  0.1599&  47.3&  0.64&  0.14&   1.3&   1.5&  -0.1&   1.1&   0.1&  11.5&   0.4&  17.8&  12.5&  14.5&  42.8 \\ 
  70& 083035.626+492719.22&  0.1323&  51.2&  0.19&  0.13&   2.3&   0.2&   0.0&   0.2&   0.1&   6.1&   0.2&  48.4&  13.6&  30.5&   0.0 \\ 
  71& 083036.559+071347.61&  0.2038&  21.8&  0.47&  0.07&   1.5&   2.5&   1.4&   3.2&   0.0&  24.6&   0.0&  73.5&   0.9&   0.3&   0.0 \\ 
  72& 083130.043+403729.62&  0.1286&  12.6&  0.28&  0.13&   1.1&   3.8&  -0.0&   3.5&   1.0&  11.3&   3.9&  52.0&   0.0&   8.8&  20.5 \\ 
  73& 083231.308+492440.69&  0.1831&  31.3&  0.23&  0.13&   1.4&   0.9&   0.1&   1.7&   0.0&   0.1&   0.2&  57.4&   2.9&  16.6&  18.4 \\ 
  74& 083317.222+413533.32&  0.1833& 120.8&  0.47&  0.12&   1.3&   2.9&   0.1&   2.5&   0.0&   5.5&   0.5&   4.0&   0.0&  40.0&  49.4 \\ 
  75& 083319.171+370436.93&  0.0418&   6.4&  0.68&  0.11&   1.0&   3.6&  -0.1&   2.5&   0.0&   5.8&   4.0&   5.8&  33.6&  46.3&   4.4 \\ 
  76& 083340.301+534258.55&  0.1413&  23.6&  0.30&  0.11&   0.9&   2.3&   0.3&   2.1&   0.0&   0.3&   1.0&  80.6&   0.0&  16.7&   0.0 \\ 
  77& 083415.653+375157.09&  0.1682&  83.9&  0.46&  0.12&   1.4&   2.0&   0.2&   1.6&   0.0&   3.0&   0.5&  33.0&   0.0&  18.3&  45.0 \\ 
  78& 083433.708+172046.34&  0.0479&   9.1&  0.33&  0.07&   1.6&   0.6&   0.3&   0.7&   0.0&  14.3&   2.1&  29.3&  54.3&   0.0&   0.0 \\ 
  79& 083449.697+100049.52&  0.1347&  15.1&  0.24&  0.13&   1.3&   1.2&   0.4&   2.4&   0.0&   2.9&  10.8&  62.6&   0.0&  23.0&   0.0 \\ 
  80& 083454.797+251258.51&  0.1322&  63.3&  0.28&  0.08&   0.8&   1.8&  -0.3&   1.0&   0.1&   1.3&   1.1&  38.4&   3.9&  45.4&   7.9 \\ 
  81& 083503.108+524039.26&  0.1178&  18.4&  0.44&  0.14&   1.0&   1.7&   0.4&   3.7&   0.5&  17.0&   0.5&   3.5&  42.5&  22.6&  12.9 \\ 
  82& 083521.230+423936.03&  0.0917&  12.9&  0.12&  0.11&   1.5&   1.4&   0.9&   0.5&   0.0&   6.4&   0.7&  92.9&   0.0&   0.0&   0.0 \\ 
  83& 083651.588+173207.98&  0.0419&   5.2&  0.35&  0.09&   0.5&   2.7&   0.5&   3.9&   0.2&  16.1&   1.5&   7.7&  59.4&  12.2&   2.6 \\ 
  84& 083913.284+120350.42&  0.2345&  75.7&  0.35&  0.11&   1.3&   2.1&   0.3&   2.0&   0.0&   3.8&   1.0&  39.6&  22.2&  24.6&   7.6 \\ 
  85& 083914.256+620825.00&  0.1204&  73.3&  0.60&  0.14&   0.9&   1.3&   0.4&   2.8&   0.1&   0.0&   0.0&   0.5&   8.1&  91.0&   0.3 \\ 
  86& 083948.425+543450.70&  0.0447&   8.1&  0.38&  0.10&   1.2&   2.0&   0.0&   2.9&   0.1&   3.1&   0.5&  11.0&  49.1&  15.8&  20.2 \\ 
  87& 084032.004+324747.40&  0.1504&  27.1&  0.46&  0.15&   0.7&   1.5&   2.1&   0.3&   0.0&   2.2&   0.6&  29.4&   0.0&  67.7&   0.0 \\ 
  88& 084041.004+190343.79&  0.1843&  87.2&  0.03&  0.05&   1.1&   0.6&  -0.2&   0.5&   0.0&   4.6&   0.2&  29.4&  20.9&   3.1&  41.8 \\ 
  89& 084056.131+175731.14&  0.1053&  26.2&  0.34&  0.06&   1.1&   0.9&   0.4&   1.1&   0.0&   3.5&   1.3&  38.0&   2.0&  54.8&   0.0 \\ 
  90& 084141.134+264239.20&  0.0898&   9.7&  0.24&  0.08&   1.0&   0.9&   0.3&   1.8&   0.0&   2.0&   1.2&  34.6&   3.0&  56.6&   2.6 \\ 
  91& 084211.446+401040.79&  0.1057&  14.5&  0.29&  0.14&   2.0&   1.4&   0.3&   1.5&   0.0&   0.2&   3.5&  48.8&   0.0&  34.1&  13.3 \\ 
  92& 084305.762+214200.91&  0.1071&  11.0&  0.36&  0.09&   1.5&   1.3&   0.0&   1.9&   0.3&   0.0&   0.9&  97.4&   0.0&   0.0&   0.0 \\ 
  93& 084414.678+023426.77&  0.1885&  60.3&  0.80&  0.10&   1.1&   1.9&   0.1&   1.8&   0.0&   0.8&   0.5&  33.9&   2.5&  51.8&  10.5 \\ 
  94& 084416.632+263303.35&  0.0793&   8.0&  0.56&  0.11&   0.6&   5.2&   0.2&   0.7&   0.6&  17.5&   0.9&   3.0&  21.7&   9.3&  46.0 \\ 
  95& 084457.482+074510.86&  0.0963&   4.2&  0.13&  0.25&   1.1&   1.3&   2.9&   1.2&   0.1&   6.5&   8.2&  81.2&   3.9&   0.1&   0.0 \\ 
  96& 084532.462+302339.75&  0.1052&  16.1&  0.28&  0.17&   1.4&   1.1&   0.6&   1.4&   0.1&   2.6&   0.5&  38.9&   1.5&  26.0&  29.6 \\ 
  97& 084542.703+292932.81&  0.1475&  16.1&  0.78&  0.16&   1.8&   2.3&   0.2&   2.3&   0.0&  25.2&   1.9&  23.3&  32.9&  11.7&   5.0 \\ 
  98& 084632.710+172445.96&  0.2050&  71.3&  0.11&  0.05&   1.0&   0.6&   0.4&   0.4&   0.0&   0.2&   0.3&  23.7&  49.6&  14.3&  11.8 \\ 
  99& 084715.854+315510.88&  0.1485&  19.6&  0.01&  0.06&   1.2&   6.7&   0.7&   1.8&   0.6&  22.6&  19.7&  48.4&   7.5&   0.0&   0.0 \\ 
 100& 084738.868+084446.31&  0.1636&  12.0&  0.35&  0.18&   1.1&   1.7&  -0.1&   1.1&   0.2&  68.3&   7.4&  24.1&   0.0&   0.0&   0.0 \\ 
 101& 084918.888+462252.58&  0.0410&   9.0&  0.33&  0.09&   1.0&   2.3&  -0.2&   2.3&   0.3&   4.4&   8.0&  13.3&  62.0&  10.4&   0.0 \\ 
 102& 085021.089+355705.80&  0.1453&  35.7&  0.76&  0.07&   1.0&   4.2&   0.0&   2.7&   0.2&  12.3&   1.4&  18.5&   9.5&   9.0&  48.8 \\ 
 103& 085030.449+115410.58&  0.1676&  13.2&  0.18&  0.06&   1.2&   0.6&   0.5&   0.0&   0.2&   9.1&   0.0&  88.5&   0.0&   0.0&   0.0 \\ 
 104& 085210.860+271031.44&  0.2332& 107.4&  0.23&  0.08&   0.9&   1.0&   0.1&   0.2&   0.0&   0.6&   0.2&  15.3&  49.0&  14.9&  19.4 \\ 
 105& 085230.000+230223.79&  0.1589&  42.4&  0.10&  0.12&   0.4&   1.1&  -0.1&   0.2&   0.1&   4.7&   0.2&  30.8&  23.4&   8.5&  32.1 \\ 
 106& 085233.876+355124.37&  0.0871&   9.3&  0.22&  0.06&   2.2&   1.1&   0.5&   2.5&   0.3&   6.9&   0.9&  58.8&  32.8&   0.0&   0.0 \\ 
 107& 085336.605+164311.67&  0.1492&  42.8&  0.47&  0.01&   0.6&   4.9&   0.2&   2.8&   0.4&   2.0&   6.9&  37.3&   0.0&  28.8&  22.2 \\ 
 108& 085812.391+480829.41&  0.1914&  42.6&  0.69&  0.08&   1.0&   2.2&   0.4&   1.9&   0.0&  17.4&   0.8&  43.9&  11.9&  25.4&   0.0 \\ 
 109& 085958.872+590832.95&  0.2692& 161.7&  0.21&  0.16&   3.6&   0.4&   0.1&   1.4&   0.0&   0.0&   1.2&  21.9&   0.0&  22.7&  54.2 \\ 
 110& 090005.244+131707.45&  0.3761&  55.7&  0.38&  0.07&  -5.4&  -0.6&   1.0&   2.0&   0.0&   0.0&   0.0&  44.3&   0.0&  46.9&   0.0 \\ 
 111& 090008.556+205039.80&  0.0611&   8.6&  0.14&  0.08&   1.7&   1.8&   0.6&   3.2&   0.0&   5.4&   8.3&  14.3&  56.6&  14.9&   0.0 \\ 
 112& 090255.800+325546.56&  0.1161&  17.5&  0.42&  0.04&   0.7&   5.5&   0.6&   3.6&   0.2&  17.8&   1.3&  26.3&  40.2&   0.0&  13.2 \\ 
 113& 090424.900+535614.06&  0.1405&  10.8&  0.33&  0.01&   1.7&   2.3&   0.2&   1.6&   0.1&  42.8&   0.0&  57.1&   0.0&   0.0&   0.0 \\ 
 114& 090601.090+073423.79&  0.1113&  11.9&  0.28&  0.10&   1.5&   1.6&   0.5&   1.8&   0.0&  30.0&   0.0&  69.7&   0.0&   0.0&   0.0 \\ 
 115& 090619.932+522150.00&  0.0987&   5.1&  0.10&  0.01&   1.3&   0.7&   2.2&   0.9&   0.2&  25.7&   0.0&  51.2&  20.8&   0.0&   0.0 \\ 
 116& 090621.408+274319.04&  0.1561&  57.1&  0.03&  0.05&   2.0&   0.4&   0.2&   0.5&   0.1&   2.0&   0.0&  18.1&  18.2&  53.9&   7.4 \\ 
 117& 090645.792+432817.31&  0.1797&  28.6&  0.35&  0.01&   2.6&   0.8&   0.5&   2.2&   0.1&  38.3&   9.1&  46.8&   5.6&   0.0&   0.0 \\ 
 118& 090747.448+295159.44&  0.1689&  21.1&  0.08&  0.04&   0.2&  -0.0&   0.2&   0.2&   0.0&  16.3&   0.8&  82.9&   0.0&   0.0&   0.0 \\ 
 119& 090811.400+262658.69&  0.0809&   9.9&  0.29&  0.10&   2.3&   1.5&  -0.3&   1.7&   0.8&  14.8&  13.9&  41.5&  24.8&   0.0&   0.0 \\ 
 120& 091140.692+274111.15&  0.1578&  56.5&  0.33&  0.04&   1.4&   2.2&  -0.5&   1.2&   0.0&   5.3&   0.4&  43.0&   0.0&  43.1&   7.0 \\ 
 121& 091158.819+152433.52&  0.1790&  31.5&  0.02&  0.08&   1.2&   1.0&   0.3&   0.9&   0.0&   0.5&   1.3&  40.0&   0.0&  35.7&  22.4 \\ 
 122& 091227.782+534222.95&  0.2223&  40.3&  0.49&  0.02&   3.6&   0.6&   0.2&   0.8&   0.1&  14.5&   3.1&  80.5&   0.0&   0.0&   0.0 \\ 
 123& 091318.257+492556.36&  0.2965&  37.0&  0.30&  0.01&   0.7&   4.4&   0.2&   1.2&   7.7&  10.2&   2.8&  58.8&   0.0&   0.0&   0.0 \\ 
 124& 091338.633+334627.93&  0.2624&  44.3&  0.37&  0.03&   1.5&   3.6&   0.4&   2.4&   0.0&  10.6&   0.0&  89.3&   0.0&   0.0&   0.0 \\ 
 125& 091411.227+091136.07&  0.1346&  24.3&  0.52&  0.13&   1.3&   1.5&   0.5&   1.9&   0.0&  13.7&   1.8&  84.5&   0.0&   0.0&   0.0 \\ 
 126& 091606.929+170000.77&  0.1984&  54.0&  0.44&  0.07&   1.0&   1.3&  -0.3&   1.2&   0.1&  12.2&   6.7&  27.7&   0.0&   9.1&  44.2 \\ 
 127& 091618.096+315807.69&  0.2599& 190.1&  0.69&  0.01&   1.3&   1.9&   0.4&   1.7&   0.0&   8.4&   0.5&   3.1&  24.3&  11.1&  51.7 \\ 
 128& 092006.437+015807.65&  0.0850&  83.7&  1.14&  0.06&   0.7&   4.2&   0.0&   2.0&   0.0&   4.4&   0.6&   0.1&  50.8&  16.7&  27.4 \\ 
 129& 092023.182+394039.10&  0.0690&   3.0&  0.00&  0.00&   2.7&   0.9&   1.6&   0.0&   0.2&   1.9&  19.3&  60.4&   0.4&  17.3&   0.0 \\ 
 130& 092252.289+155754.77&  0.1343&  17.3&  0.30&  0.10&   1.3&   2.6&   0.3&   2.0&   0.3&  22.9&   1.7&  46.6&   3.6&  20.8&   0.0 \\ 
 131& 092316.298+311429.66&  0.3131&  54.4&  0.22&  0.01&   1.5&   3.8&   0.6&   1.5&   0.3&   0.0&   0.0&  66.8&  13.2&   0.0&   0.0 \\ 
 132& 092420.102+031454.70&  0.1291&  15.5&  0.00&  0.11&   4.6&   0.2&   0.1&   1.4&   0.0&   3.9&   6.4&  89.7&   0.0&   0.0&   0.0 \\ 
 133& 092438.057+133134.95&  0.1784&  47.1&  0.40&  0.08&   0.9&   4.4&  -1.3&   2.9&   0.0&   5.4&   1.6&  46.8&   0.0&  46.1&   0.0 \\ 
 134& 092503.821+404602.82&  0.1168&   8.1&  0.18&  0.01&   1.6&   1.0&   0.5&   1.9&   0.0&   7.0&   0.0&  51.5&  41.4&   0.0&   0.0 \\ 
 135& 092539.823+600729.85&  0.1576&  21.4&  0.28&  0.06&   1.0&   1.3&   0.6&   1.5&   0.0&  12.5&   4.2&  75.7&   7.6&   0.0&   0.0 \\ 
 136& 092610.469+054710.10&  0.3384& 159.0&  0.21&  0.11&   0.8&   4.5&   0.8&   1.2&   0.0&   0.5&   1.1&  28.6&  29.1&  22.0&  18.7 \\ 
 137& 092637.212+532550.96&  0.1853&  78.9&  0.68&  0.02&   1.8&   3.0&   1.1&   1.4&   0.0&   6.2&   1.3&   3.2&  13.9&  38.3&  37.1 \\ 
 138& 092657.689+423136.63&  0.1114&  21.9&  0.47&  0.01&   1.3&   3.8&   0.7&   3.3&   1.1&   1.2&   7.6&  56.1&   0.0&  29.1&   0.0 \\ 
 139& 092717.047+262344.70&  0.2078&  34.5&  0.14&  0.07&   1.4&   3.2&   2.5&   0.6&   0.0&   5.4&   0.3&  41.1&  40.4&  12.2&   0.0 \\ 
 140& 092823.455+454806.45&  0.2438&  61.6&  0.41&  0.04&   2.3&   1.3&   0.8&   1.7&   0.0&   0.0&   0.0&  98.1&   0.0&   1.9&   0.0 \\ 
 141& 092952.692+062528.69&  0.2616&  18.7&  0.67&  0.13&   1.0&   4.3&   0.2&   3.2&   0.2&  10.7&   4.5&  67.0&   0.0&   0.0&   0.0 \\ 
 142& 093057.662+244822.79&  0.0601&   6.5&  0.27&  0.04&   2.1&   0.8&  -0.0&   0.7&   0.0&   5.3&   0.0&  44.9&  20.0&   0.8&  28.8 \\ 
 143& 093123.995+441857.32&  0.1433&  20.3&  0.17&  0.08&   2.2&   0.5&   0.1&   1.2&   0.1&   7.8&  11.4&  47.1&   9.6&   7.6&  16.1 \\ 
 144& 093223.952+180303.80&  0.1420&  73.7&  0.57&  0.11&   1.1&   4.2&   0.1&   2.1&   0.0&   5.6&   0.8&  16.8&  10.5&  20.9&  44.0 \\ 
 145& 093225.889+603346.86&  0.1015&  47.9&  0.18&  0.08&   1.5&   1.4&   0.0&   1.1&   0.1&   5.4&   2.2&  21.5&   0.0&  38.0&  31.9 \\ 
 146& 093258.555+103152.14&  0.1476&  14.1&  0.31&  0.07&   1.2&   2.5&   1.7&   1.4&   0.4&  29.9&   4.7&  50.2&   2.3&   0.0&  11.2 \\ 
 147& 093401.978+131236.15&  0.2184&  22.4&  0.30&  0.06&   0.8&   1.3&   0.8&   0.4&   0.0&  21.6&   0.0&  78.5&   0.0&   0.0&   0.0 \\ 
 148& 093414.381+480456.26&  0.1584&  21.4&  0.25&  0.03&   1.0&   2.2&   1.7&   2.6&   0.1&   5.9&   0.0&  24.6&  47.7&   0.0&  20.5 \\ 
 149& 093609.132+532855.40&  0.1989&  66.8&  0.31&  0.02&   1.1&   2.7&   0.3&   2.9&   0.0&   0.1&   2.6&  27.7&   5.2&  46.8&  16.7 \\ 
 150& 093713.886+323453.77&  0.1273&  18.4&  0.53&  0.03&   1.6&   3.4&   0.9&   3.0&   0.0&   8.6&   2.9&  14.4&  35.5&  37.3&   0.0 \\ 
 151& 093842.905+000148.68&  0.0907&  33.4&  0.57&  0.11&   1.5&   1.6&  -0.1&   3.0&   0.1&   8.2&   0.5&  13.6&  26.2&   4.3&  46.9 \\ 
 152& 093948.094+340556.40&  0.1390&  12.3&  0.41&  0.00&   1.5&   1.5&   1.1&   2.5&   0.1&  19.8&   2.7&  74.0&   2.8&   0.0&   0.0 \\ 
 153& 093956.566+235922.67&  0.0846&  23.5&  0.53&  0.01&   2.1&   2.0&   0.8&   2.1&   0.0&  19.1&   0.7&  79.9&   0.0&   0.0&   0.0 \\ 
 154& 094039.792+144551.47&  0.0869&   6.6&  0.21&  0.10&   1.1&   1.5&   0.0&   1.8&   0.2&  24.0&   6.3&  44.0&  14.2&   5.5&   4.6 \\ 
 155& 094055.862+400715.19&  0.2356&  54.0&  0.46&  0.02&   1.5&   1.8&  -0.0&   1.5&   0.0&  10.2&   0.0&  40.1&  46.0&   0.0&   0.0 \\ 
 156& 094140.699+212102.49&  0.1758&  19.8&  0.22&  0.04&   1.4&   1.5&  -0.1&   1.8&   0.0&  18.1&   0.0&  64.1&  17.7&   0.0&   0.0 \\ 
 157& 094209.310+130553.84&  0.1312&  92.2&  0.24&  0.06&   1.2&   1.1&  -0.1&  -0.1&   0.0&   0.6&   0.5&  24.8&   0.0&  33.3&  40.6 \\ 
 158& 094320.914+371132.22&  0.1944&  35.5&  0.29&  0.00&   2.8&   1.1&   0.5&   2.0&   0.0&   1.1&   2.3&  81.4&   0.0&  15.2&   0.0 \\ 
 159& 094347.544+020557.95&  0.0927&   5.5&  0.12&  0.15&   1.3&   0.3&   0.6&   1.6&   0.5&  11.3&   5.8&  28.5&  45.5&   8.3&   0.0 \\ 
 160& 094353.873+125512.47&  0.3060& 114.7&  0.21&  0.05&   1.2&   2.4&   0.1&   1.6&   0.1&   1.6&   2.5&  33.8&   0.0&   3.3&  57.4 \\ 
 161& 094514.155+115124.29&  0.1882&  22.6&  0.10&  0.03&   1.9&   1.1&   0.9&   0.5&   0.1&  14.0&  13.0&  69.9&   0.0&   0.0&   3.0 \\ 
 162& 094555.742+104542.90&  0.1190&  11.8&  0.16&  0.04&   2.5&   0.7&   0.5&   0.7&   0.1&   8.3&   0.4&  84.6&   1.5&   4.7&   0.0 \\ 
 163& 094604.426+185641.15&  0.0533&  32.7&  0.79&  0.04&   1.6&   5.4&   0.0&   2.7&   0.0&  10.5&   1.7&   0.0&  29.7&   0.0&  57.8 \\ 
 164& 094659.530+225207.47&  0.2298&  41.6&  0.18&  0.03&  -1.4&   0.2&   0.4&   0.5&   0.0&  15.3&   0.0&  81.2&   2.4&   1.0&   0.0 \\ 
 165& 094701.490+600720.12&  0.1229&  20.8&  0.70&  0.03&   1.0&   2.1&   0.2&   1.0&   0.1&  25.4&   8.6&  15.2&  49.8&   0.0&   0.0 \\ 
 166& 094704.462+543044.40&  0.0454&   1.9&  0.00&  0.01&   3.4&  -0.1&  -0.2&   2.3&   0.1&   1.3&   0.0&   4.7&  63.1&  19.8&  10.9 \\ 
 167& 094744.465+405914.72&  0.1531&  42.4&  0.58&  0.01&   1.8&   2.4&   0.9&   3.9&   0.1&  13.7&   0.5&  11.3&  46.4&   0.0&  27.9 \\ 
 168& 094818.677+023004.16&  0.0604&   9.6&  0.29&  0.11&   2.7&   0.7&   0.1&   2.0&   0.3&   8.5&   1.0&  14.4&  43.6&  22.7&   9.2 \\ 
 169& 094915.845+204412.77&  0.0651&  18.9&  0.28&  0.03&   1.1&   1.9&  -0.3&   2.2&   0.3&   6.6&   1.3&   8.8&  22.3&  59.9&   0.0 \\ 
 170& 094952.824-002104.82&  0.2153&  49.5&  0.18&  0.17&   1.5&   0.6&  -1.5&  -0.2&   0.0&  11.6&   0.0&  43.3&   3.7&  40.9&   0.0 \\ 
 171& 095006.482+163106.02&  0.2265&  32.0&  0.09&  0.08&   1.3&   0.6&  -0.1&   1.1&   0.0&   2.6&   0.0&  92.1&   0.9&   4.2&   0.0 \\ 
 172& 095053.155+091931.49&  0.1707&  25.9&  0.35&  0.03&   1.5&   2.9&   1.2&   2.7&   0.2&   0.8&  22.4&  34.2&  31.8&   2.3&   7.3 \\ 
 173& 095136.689+284458.12&  0.1347&  13.4&  0.00&  0.01&   1.6&   1.2&   0.0&   2.0&   0.0&  19.3&  11.4&  57.8&  11.4&   0.0&   0.0 \\ 
 174& 095224.634+641657.66&  0.0739&   4.8&  0.32&  0.16&   0.6&   4.6&   0.4&   3.4&   0.1&   0.4&  12.2&   4.6&  70.4&   0.9&  11.5 \\ 
 175& 095336.144+292543.28&  0.1810&  40.9&  0.35&  0.02&   1.4&   1.9&   0.3&   2.8&   0.0&   7.3&   2.2&  20.6&  14.3&  43.7&   7.7 \\ 
 176& 095531.781+445733.97&  0.2115&  49.0&  0.38&  0.00&   1.1&   2.0&  -0.1&   2.0&   0.1&  14.1&   0.0&  58.7&  27.1&   0.0&   0.0 \\ 
 177& 095636.199+543220.94&  0.3423&  49.7&  0.49&  0.00&   1.0&   2.7&   0.3&   1.7&   0.0&   0.0&  26.1&  46.0&  19.3&   0.0&   0.0 \\ 
 178& 095729.906+024942.07&  0.2161&  28.5&  0.00&  0.03&   1.6&   0.9&   0.2&   0.7&   0.1&   6.7&   0.0&  50.1&   7.5&  25.9&   9.4 \\ 
 179& 095824.622+003203.16&  0.0927&  18.6&  0.23&  0.06&   0.5&   1.2&  -0.3&   2.5&   0.3&   2.2&   0.4&  11.6&  23.6&  47.5&  13.7 \\ 
 180& 095842.643+631845.50&  0.2426&  74.3&  0.45&  0.09&   1.6&   2.3&   0.4&   2.8&   0.0&   7.4&   0.6&  58.8&  12.1&  20.3&   0.0 \\ 
 181& 095851.290+075910.25&  0.2373&  30.2&  0.07&  0.03&   1.4&   1.0&   0.2&   1.1&   0.0&   1.7&   1.7&  96.6&   0.0&   0.0&   0.0 \\ 
 182& 100027.310+104928.02&  0.1624&  29.8&  0.29&  0.06&   0.8&   2.7&   0.4&   2.7&   0.0&   4.9&   0.0&  51.7&  21.3&   4.8&  17.2 \\ 
 183& 100031.169+375759.06&  0.2284& 145.2&  0.48&  0.01&   3.0&   0.8&  -0.1&   1.2&   0.0&   1.3&   0.3&  19.9&   4.0&  30.3&  44.1 \\ 
 184& 100111.930+192933.52&  0.2110&  50.7&  0.14&  0.04&   1.2&   1.1&   0.1&   1.0&   0.0&   5.3&   1.1&  48.1&  31.5&   4.3&   9.5 \\ 
 185& 100113.642+092859.67&  0.0586&   1.6&  0.05&  0.06&   0.5&   2.3&   1.2&   1.5&   0.1&  29.6&   1.0&  15.2&  45.7&   5.9&   2.4 \\ 
 186& 100402.383+550647.40&  0.1380&  11.8&  0.37&  0.00&   1.4&   1.9&   0.2&   3.0&   0.0&  22.6&   4.5&  72.9&   0.0&   0.0&   0.0 \\ 
 187& 100409.672+355646.11&  0.1678&  24.8&  0.05&  0.01&   0.7&   0.7&   0.2&   1.5&   0.0&   8.1&   0.0&  28.4&  25.1&  11.8&  25.7 \\ 
 188& 100522.452+072728.30&  0.0630&   3.8&  0.25&  0.02&   1.4&   1.4&   0.4&   0.7&   0.0&   1.3&   0.8&  58.9&   0.8&  38.2&   0.0 \\ 
 189& 100529.796+291645.33&  0.0949&  10.0&  0.12&  0.05&   0.7&   3.1&   1.5&   1.7&   0.0&   2.1&   1.8&  20.7&  59.4&  16.1&   0.0 \\ 
 190& 100618.310+194131.66&  0.1559&  16.7&  0.13&  0.11&   2.1&   0.8&   0.2&   1.6&   0.0&  19.5&   9.7&  58.7&  11.9&   0.0&   0.0 \\ 
 191& 100626.726+520906.04&  0.1266&  10.6&  0.52&  0.01&   1.6&   3.2&   2.2&   2.1&   0.0&  26.4&   0.0&  46.3&  17.9&   8.3&   0.0 \\ 
 192& 100650.868+014133.99&  0.0458&   4.2&  0.02&  0.04&   0.6&   1.0&  -0.5&   3.5&   0.2&   0.7&   0.5&  10.3&  45.0&  18.5&  24.8 \\ 
 193& 100743.618+554934.54&  0.0452&   4.5&  0.04&  0.00&   1.6&   1.5&   0.5&   2.0&   0.0&  25.6&   8.6&  65.8&   0.1&   0.0&   0.0 \\ 
 194& 100752.675+291104.78&  0.3763&  49.0&  0.37&  0.06&   1.7&   3.7&   1.1&   2.3&   0.0&  35.0&   0.0&  65.0&   0.0&   0.0&   0.0 \\ 
 195& 100755.092+392139.13&  0.2570& 148.6&  0.40&  0.00&   1.7&   1.8&  -0.1&   0.1&   0.0&   2.0&   0.6&  25.8&   0.0&  71.3&   0.0 \\ 
 196& 100907.284-000157.86&  0.0959&  16.9&  0.90&  0.03&   0.6&   4.5&   0.8&   1.8&   0.0&  15.1&   0.0&   2.1&  47.0&  29.4&   5.9 \\ 
 197& 100918.542+374228.31&  0.2111&  55.3&  0.27&  0.06&   1.8&   1.3&  -0.1&   1.3&   0.3&   0.5&   0.2&  49.8&   0.0&  18.2&  30.9 \\ 
 198& 101004.738+183613.74&  0.1453&  21.6&  0.09&  0.08&   1.6&   0.7&   0.1&  -0.1&   0.0&  19.2&   0.0&  80.8&   0.0&   0.0&   0.0 \\ 
 199& 101009.833+145732.15&  0.1842&  21.3&  0.09&  0.10&   1.3&   1.6&   0.8&   2.2&   0.0&  24.6&   0.6&  61.1&   7.4&   5.7&   0.0 \\ 
 200& 101108.878+614156.53&  0.1989&  23.7&  0.52&  0.01&   2.9&   0.3&   0.3&   0.6&   0.0&  18.2&   0.2&  81.6&   0.0&   0.0&   0.0 \\ 
 201& 101241.698+641102.30&  0.1286&  23.9&  0.27&  0.03&   0.5&   3.7&   0.3&   2.7&   0.4&   0.0&   4.5&  34.3&  29.5&  30.0&   0.0 \\ 
 202& 101342.775+125135.28&  0.1391&  16.0&  0.27&  0.09&   1.3&   4.7&   2.4&   1.0&   0.2&  11.7&   2.3&  83.1&   0.0&   0.0&   0.0 \\ 
 203& 101437.649+010926.79&  0.1442&  35.0&  0.13&  0.01&   1.8&   0.4&  -0.1&   0.2&   0.1&   3.3&  10.8&  37.0&  41.9&   0.0&   6.5 \\ 
 204& 101519.687+010341.63&  0.2159&  39.8&  0.28&  0.04&   1.0&   0.8&  -0.1&   0.4&   0.1&   1.1&   5.2&  90.2&   0.7&   0.0&   0.0 \\ 
 205& 101624.362+580136.72&  0.2253& 108.0&  0.91&  0.01&   0.8&   4.4&  -0.2&   2.1&   0.0&  19.2&   2.2&  20.1&   0.0&   0.0&  58.5 \\ 
 206& 101629.210-000137.12&  0.1046&  11.3&  0.45&  0.03&   0.4&   3.9&  -0.1&   1.2&   0.8&  15.2&   3.0&   3.5&  34.0&   0.0&  43.5 \\ 
 207& 101658.481+282425.47&  0.1342&  24.2&  0.15&  0.09&   1.6&   1.5&   0.2&  -0.1&   0.0&   2.6&   0.5&  47.2&   0.7&  19.9&  29.0 \\ 
 208& 101906.120+192100.31&  0.0282&   0.2&  0.08&  0.09&   0.7&   1.4&  -0.0&  -0.9&   0.2&  38.4&  27.9&  23.6&  10.0&   0.0&   0.0 \\ 
 209& 102000.211+081333.81&  0.0491&  18.5&  1.08&  0.03&   1.4&   2.2&  -0.2&   1.0&   0.0&   1.8&   0.9&   6.2&  75.6&   3.7&  11.7 \\ 
 210& 102054.334+100624.00&  0.0969&  27.7&  0.21&  0.08&   1.0&   2.9&   0.9&   3.7&   0.3&   2.5&   0.5&  27.8&   1.4&  36.7&  30.5 \\ 
 211& 102103.542+304108.90&  0.1823&  30.9&  0.33&  0.07&   1.1&   2.5&  -0.2&   1.2&   3.5&   7.0&   0.6&  69.2&   8.7&   0.0&   0.0 \\ 
 212& 102200.787+220947.44&  0.1130&  38.7&  0.48&  0.04&   2.0&   2.4&  -0.0&   1.8&   0.0&  13.1&   5.6&  48.3&  13.4&  16.4&   0.0 \\ 
 213& 102206.982+201009.31&  0.1221&  11.6&  0.36&  0.07&   0.7&   1.3&  -0.0&   2.1&   0.0&  37.0&   5.8&  44.0&  13.2&   0.0&   0.0 \\ 
 214& 102518.962+131918.06&  0.1066&   6.0&  0.08&  0.12&   3.9&   0.2&   0.5&   0.6&   0.0&  30.0&   2.8&  50.2&  16.6&   0.3&   0.0 \\ 
 215& 102544.676+025824.45&  0.1923&  52.8&  0.44&  0.05&   0.9&   4.2&   0.8&   2.7&   0.6&  10.9&   2.0&  22.3&   0.1&  43.0&  20.2 \\ 
 216& 102552.646+043949.59&  0.1420&  72.3&  0.50&  0.02&   1.3&   2.7&   0.1&   2.6&   0.0&   9.2&   0.7&  15.1&  28.2&   2.6&  43.4 \\ 
 217& 102607.469+562330.00&  0.1406&  19.7&  0.47&  0.00&   2.2&   2.2&   0.9&   2.0&   0.0&  14.9&   2.3&  51.5&   0.2&  10.3&  20.7 \\ 
 218& 102724.199+370421.02&  0.1035&  12.1&  0.83&  0.00&   0.9&   2.6&   0.5&   2.7&   0.0&  25.6&   4.3&  12.4&  41.2&   0.0&  15.8 \\ 
 219& 102808.544+294933.32&  0.1238&   8.5&  0.33&  0.05&   1.4&   1.5&   0.2&   0.7&   0.0&  11.5&   0.0&  88.5&   0.0&   0.0&   0.0 \\ 
 220& 102812.180+121501.90&  0.1916&  77.4&  0.64&  0.05&   0.9&   2.6&  -0.1&   3.2&   0.0&   4.9&   3.0&  50.1&   0.0&  16.2&  25.9 \\ 
 221& 102842.110+031129.41&  0.2584&  72.4&  0.09&  0.07&   3.1&   0.3&  -0.5&   0.4&   0.0&   3.7&   0.3&  44.1&  19.1&  32.8&   0.0 \\ 
 222& 102856.978+450910.94&  0.1702&  15.3&  0.19&  0.00&   1.6&   4.2&   5.2&   2.8&   0.0&  40.9&   2.5&  56.5&   0.0&   0.0&   0.0 \\ 
 223& 102925.404+122244.89&  0.1807&  44.3&  0.19&  0.07&   0.6&   2.2&   0.3&   3.0&   0.0&   6.6&   0.5&  19.6&   2.8&  51.8&  18.4 \\ 
 224& 103000.478+205517.53&  0.1354&  42.0&  0.34&  0.01&   1.9&   1.3&  -0.1&   1.4&   0.1&   2.9&   2.8&  21.8&  22.1&  27.1&  22.7 \\ 
 225& 103138.582+112816.84&  0.1054&  17.6&  0.88&  0.08&   0.7&   2.7&  -0.6&   1.2&   0.1&   0.9&   9.1&  22.4&   0.0&  36.8&  30.5 \\ 
 226& 103320.513+243559.14&  0.2263&  31.0&  0.27&  0.00&   1.5&   0.5&  -0.1&   0.2&   0.1&   1.9&   0.0&  97.8&   0.0&   0.0&   0.0 \\ 
 227& 103618.626+054409.41&  0.2176&  87.0&  0.00&  0.07&   0.8&   0.1&  -0.4&   0.2&   0.0&   0.0&   0.0&  23.3&  43.8&   7.6&  24.9 \\ 
 228& 103748.274+115342.67&  0.0940&  11.0&  0.15&  0.13&   3.8&   0.3&   0.2&   1.5&   0.2&  17.1&  10.6&  42.2&   0.0&  29.3&   0.0 \\ 
 229& 103811.402+153514.61&  0.1420&   9.4&  0.04&  0.07&  -3.2&  -0.3&   0.6&   0.1&   0.1&  34.0&  10.7&  55.0&   0.2&   0.0&   0.0 \\ 
 230& 103826.587+182331.09&  0.0558&  10.6&  0.16&  0.03&   3.6&   0.4&   0.6&   1.4&   0.0&  11.7&   1.6&  35.3&  51.1&   0.0&   0.0 \\ 
 231& 103928.058+011242.06&  0.1218&  13.6&  0.08&  0.10&   2.0&   1.1&   0.6&   2.4&   0.1&  12.1&  16.6&  18.7&  15.9&  22.2&  13.7 \\ 
 232& 103934.512+060425.00&  0.1631&  24.1&  0.12&  0.04&   0.9&   1.0&   0.3&   1.6&   0.0&  21.0&   0.0&  79.0&   0.0&   0.0&   0.0 \\ 
 233& 104033.662+373627.14&  0.1731&  35.8&  0.35&  0.00&   1.2&   1.7&   0.4&   2.2&   0.0&   3.4&   0.0&  87.7&   8.4&   0.4&   0.0 \\ 
 234& 104128.630+371545.82&  0.0233&   1.3&  0.44&  0.00&   1.1&   1.4&   0.3&   2.1&   0.1&   1.7&   0.9&   6.7&  70.2&  20.2&   0.0 \\ 
 235& 104144.486+191405.27&  0.1837&  34.8&  0.37&  0.03&   1.8&   2.0&  -0.2&   1.6&   0.0&  10.2&   1.4&  32.2&   0.0&  53.1&   0.0 \\ 
 236& 104152.382+522444.82&  0.2876&  55.4&  0.21&  0.00&   1.2&   2.1&   0.3&   1.8&   0.1&   2.2&   0.0&  97.8&   0.0&   0.0&   0.0 \\ 
 237& 104204.135+293323.41&  0.0398&   7.7&  0.22&  0.02&   1.8&   1.1&   0.4&   1.2&   0.0&   7.5&   2.8&  25.1&  33.0&  31.5&   0.0 \\ 
 238& 104215.170+140636.31&  0.0543&  10.1&  0.14&  0.07&   1.4&   1.3&   0.2&   1.8&   0.3&   6.9&   2.5&  21.4&  67.8&   0.0&   0.0 \\ 
 239& 104218.238+370756.34&  0.1539&  56.7&  0.93&  0.00&   0.8&   3.9&  -0.4&   4.9&   0.1&   5.3&   0.0&   0.1&  23.9&  21.4&  49.2 \\ 
 240& 104220.143+564855.80&  0.0910&  58.9&  0.42&  0.00&   1.6&   1.5&  -0.0&   2.7&   0.0&   4.1&   0.3&  19.1&  27.4&   7.0&  41.5 \\ 
 241& 104230.550+003442.00&  0.1000&  22.7&  0.42&  0.07&   2.2&   2.8&   0.6&   3.4&   0.6&  17.6&   3.7&  18.7&  29.5&  16.5&  11.5 \\ 
 242& 104349.877+420923.41&  0.2341&  60.7&  0.37&  0.00&   1.3&   1.2&   0.2&  -0.0&   0.6&   1.6&   2.1&  74.5&   5.7&  11.1&   0.0 \\ 
 243& 104410.435+394908.57&  0.0868&   8.6&  0.30&  0.00&   2.1&   0.4&   0.4&   1.0&   0.2&  29.0&   0.5&  21.9&  15.8&  32.5&   0.0 \\ 
 244& 104619.330+071452.32&  0.1735&  51.5&  0.29&  0.07&   1.3&   1.2&  -0.1&  -0.1&   0.4&   0.2&   0.2&  22.6&   0.0&  73.2&   0.6 \\ 
 245& 104655.553+150742.25&  0.1005&   8.7&  0.38&  0.04&   1.4&   2.7&   1.1&   1.6&   0.0&   8.2&   1.2&  51.0&  39.6&   0.0&   0.0 \\ 
 246& 104710.562+180217.20&  0.1303&  33.9&  0.54&  0.03&   1.0&   1.6&   0.1&   2.7&   0.2&   6.4&   0.5&  21.9&  25.8&  28.0&  16.7 \\ 
 247& 104902.102+443556.87&  0.0501&   3.5&  0.36&  0.00&   0.5&   4.2&  -0.1&   3.4&   1.5&  13.8&   5.9&   5.4&  73.2&   0.0&   0.0 \\ 
 248& 104933.866+323911.15&  0.0730&  12.1&  0.17&  0.01&   1.1&   2.5&   0.4&   1.8&   0.7&   7.7&   0.8&   2.4&  25.7&  56.9&   4.7 \\ 
 249& 104935.983+132235.39&  0.1784&  39.7&  1.06&  0.07&   0.9&   2.9&   0.6&   2.2&   0.0&  20.2&   2.1&   9.0&   1.8&  34.5&  31.9 \\ 
 250& 104953.318+564551.33&  0.1819&  51.5&  0.32&  0.00&   1.9&   1.2&   0.4&   0.5&   0.1&   4.2&   0.9&  20.0&   7.6&  62.0&   5.2 \\ 
 251& 105220.450+054941.59&  0.0413&  12.9&  0.19&  0.09&   1.8&   0.9&   0.1&   1.3&   0.1&  10.1&   0.8&  19.7&  28.4&  13.8&  26.9 \\ 
 252& 105228.742+574213.74&  0.2079&  39.0&  0.47&  0.00&   1.5&   1.2&   0.6&   2.1&   0.1&  13.2&   5.1&  81.6&   0.0&   0.0&   0.0 \\ 
 253& 105302.563+345739.24&  0.1822&  40.9&  0.09&  0.00&   1.4&   0.8&  -0.0&   0.5&   0.0&   7.2&   0.0&  92.4&   0.0&   0.0&   0.0 \\ 
 254& 105411.851+082006.31&  0.2232&  13.0&  0.18&  0.04&   1.2&   3.1&   0.9&   2.3&   0.2&   0.0&  13.0&  83.8&   1.6&   0.0&   0.0 \\ 
 255& 105435.515+555738.18&  0.0479&   1.1&  0.06&  0.00&   0.5&   1.0&   0.1&   0.7&   0.2&  11.0&  13.8&   9.7&  49.0&  15.2&   0.1 \\ 
 256& 105532.426+135220.27&  0.1396&  12.5&  0.07&  0.03&  -8.9&  -0.1&   0.4&  -0.2&   0.0&   3.7&  20.7&  55.7&   2.3&  15.7&   1.6 \\ 
 257& 105555.291+440326.92&  0.0372&   0.3&  0.00&  0.00&   1.1&   0.3&   0.3&   3.0&   0.1&  12.2&  14.2&  10.1&  63.3&   0.0&   0.0 \\ 
 258& 105743.939+123539.91&  0.1193&  27.6&  0.23&  0.01&   1.3&   1.4&  -0.0&   0.9&   0.0&  17.4&   0.0&  82.5&   0.0&   0.0&   0.0 \\ 
 259& 105755.265+334041.54&  0.0583&   4.5&  0.30&  0.00&   2.1&   0.8&   0.4&   1.8&   0.1&  22.5&   6.2&  24.1&  37.4&   9.8&   0.0 \\ 
 260& 110100.307+395525.95&  0.1503&  54.9&  0.75&  0.00&   0.7&   3.8&   0.2&   1.0&   0.1&   3.6&   0.2&   8.3&  10.1&  48.7&  29.0 \\ 
 261& 110106.809+061552.90&  0.1961&  42.9&  0.43&  0.05&   0.7&   2.6&   0.2&   1.1&   0.1&  13.3&   0.6&  35.0&   1.6&   0.0&  48.7 \\ 
 262& 110320.189+544848.12&  0.1527&  12.2&  0.55&  0.00&   1.5&   2.7&   0.5&   4.1&   0.0&  35.6&  10.4&  54.0&   0.0&   0.0&   0.0 \\ 
 263& 110322.090+360210.18&  0.1328&  20.8&  0.00&  0.07&   1.2&   0.8&   0.1&   1.4&   0.0&   3.0&   8.6&  71.2&  17.0&   0.0&   0.0 \\ 
 264& 110334.481+024220.00&  0.1473&  14.2&  0.21&  0.17&   0.7&   1.5&   0.5&   0.1&   0.3&  23.2&   9.4&  33.5&   5.1&  27.5&   0.0 \\ 
 265& 110409.655+441535.77&  0.2230&  71.0&  0.28&  0.00&   1.1&   1.3&   0.2&   0.9&   0.0&   3.3&   0.0&  27.4&  27.0&  30.8&  11.3 \\ 
 266& 110520.364+301719.55&  0.0706&   8.8&  0.80&  0.00&   0.5&   5.5&   1.1&   2.9&   0.1&   0.0&   0.0&  10.7&  26.6&  60.9&   1.7 \\ 
 267& 110540.706+055954.26&  0.0543&  21.0&  0.40&  0.10&   2.4&   1.5&   3.2&   1.4&   0.0&   7.0&   2.0&  27.6&  63.5&   0.0&   0.0 \\ 
 268& 110618.312+493538.77&  0.0741&  14.5&  0.24&  0.00&   1.2&   1.0&   0.3&   1.4&   0.1&  11.3&   5.8&  12.7&  18.9&  19.4&  31.5 \\ 
 269& 110618.382+032641.58&  0.2100&  32.9&  0.47&  0.14&   0.6&   5.4&   0.8&   1.9&   0.2&  15.9&  18.7&  43.9&   1.8&  11.6&   7.6 \\ 
 270& 110653.736+405736.41&  0.1000&   8.5&  0.41&  0.00&   1.8&   1.5&   0.3&   0.8&   0.0&  16.6&   6.9&  45.1&  29.6&   0.0&   0.0 \\ 
 271& 110724.391+361222.55&  0.0731&  19.8&  0.09&  0.00&   2.6&   1.0&   0.1&   2.0&   0.1&   8.9&   0.9&  15.3&  51.4&  12.7&  10.7 \\ 
 272& 110752.838+442144.83&  0.0759&   2.0&  0.00&  0.00&   0.4&   1.8&   3.3&   0.3&   0.0&  21.1&  24.1&  35.8&  19.1&   0.0&   0.0 \\ 
 273& 110905.542+190615.10&  0.0855&  18.0&  0.41&  0.00&   1.3&   1.7&  -0.1&   3.1&   0.2&  24.1&   2.1&   9.4&  25.2&   0.0&  39.0 \\ 
 274& 110933.732+221155.81&  0.0689&   8.2&  0.05&  0.00&   1.6&   1.6&   0.4&   1.8&   0.0&   5.7&   3.9&   5.9&  52.1&  30.0&   2.4 \\ 
 275& 111002.215+023527.17&  0.1076&  16.0&  0.58&  0.10&   2.2&   1.4&   0.2&   1.8&   0.2&  40.0&   8.5&  33.8&  17.3&   0.0&   0.0 \\ 
 276& 111028.634+293239.51&  0.2133&  87.7&  0.35&  0.00&   3.1&   0.5&  -0.3&   0.8&   0.1&   6.8&   5.0&  15.1&  11.5&   3.7&  57.3 \\ 
 277& 111050.945+005531.00&  0.1520&  75.7&  0.63&  0.10&   1.5&   2.2&   0.1&   3.1&   0.6&   6.4&   1.8&  11.2&  22.3&  13.2&  43.8 \\ 
 278& 111053.676+315759.88&  0.1645&  16.7&  0.16&  0.00&   1.6&   1.3&   1.1&   1.2&   0.0&  10.9&   0.0&  77.8&  10.9&   0.0&   0.0 \\ 
 279& 111108.081+004048.79&  0.1844&  12.8&  0.43&  0.11&   1.4&   1.6&   0.3&   1.9&   1.8&   3.6&  10.7&  80.2&   0.0&   0.0&   0.0 \\ 
 280& 111109.778+044035.33&  0.0414&   1.2&  0.47&  0.17&   0.4&   4.2&  -0.1&   1.2&   0.2&  16.8&   0.0&   9.4&  60.8&  12.9&   0.0 \\ 
 281& 111155.709+281858.11&  0.0322&   0.4&  0.23&  0.00&   0.4&   0.8&   0.1&   5.6&   0.2&  13.4&   1.1&  13.5&  71.7&   0.0&   0.0 \\ 
 282& 111212.624-003628.39&  0.1220&  24.1&  0.42&  0.09&   1.3&   1.7&   0.2&   0.1&   0.0&  14.2&   0.5&  85.4&   0.0&   0.0&   0.0 \\ 
 283& 111314.093+322115.41&  0.0759&  16.8&  0.53&  0.04&   0.7&   4.4&   0.2&   1.8&   0.2&  10.6&   2.0&   8.4&  48.4&   5.6&  24.2 \\ 
 284& 111327.958-005409.53&  0.0411&   1.0&  0.00&  0.09&  -0.5&   0.2&   0.7&  -0.7&   0.0&   9.4&   1.9&  88.7&   0.0&   0.0&   0.0 \\ 
 285& 111333.060+005001.37&  0.1524&  13.5&  0.00&  0.12&   1.9&   1.6&   0.1&   2.2&   0.0&   2.3&   0.0&  97.5&   0.0&   0.0&   0.0 \\ 
 286& 111403.134+533652.86&  0.1715&  35.1&  0.33&  0.00&   0.8&   3.6&  -0.3&   2.6&   0.1&   3.7&   0.1&  31.8&  18.9&   6.3&  38.5 \\ 
 287& 111441.611+593029.94&  0.1442&  35.5&  0.56&  0.00&   0.9&   4.7&   0.6&   3.0&   2.4&   2.6&   5.3&  29.1&   0.0&  52.4&   0.0 \\ 
 288& 111531.320+540946.33&  0.1079&   9.1&  0.38&  0.00&   2.0&   1.4&   1.9&   1.6&   0.2&  16.1&   1.7&  53.3&  24.1&   4.3&   0.0 \\ 
 289& 111536.701+302522.15&  0.0279&   0.5&  0.09&  0.00&   0.5&   5.2&   0.7&   4.9&   0.1&   7.8&   9.8&  17.3&  60.9&   4.0&   0.0 \\ 
 290& 111658.824+413955.28&  0.1237&  15.6&  0.70&  0.01&   1.1&   2.5&   0.0&   2.1&   0.1&  33.8&   0.0&   7.7&  44.9&  12.8&   0.0 \\ 
 291& 111731.195+370239.52&  0.1068&  11.6&  0.36&  0.00&   1.0&   0.6&   0.7&  -0.6&   0.1&  10.3&  18.2&  48.7&  16.7&   0.0&   5.6 \\ 
 292& 111806.742+183856.35&  0.0496&   2.2&  0.00&  0.00&   2.4&   2.1&   5.5&   3.0&   0.3&  19.6&   5.6&  11.2&  29.8&  19.7&  13.8 \\ 
 293& 111849.922+195424.30&  0.2144&  38.9&  0.43&  0.00&   1.6&   4.1&   2.6&   2.1&   0.6&   7.3&   4.2&  83.0&   0.0&   0.2&   0.0 \\ 
 294& 111946.435+351803.48&  0.1037&   9.2&  0.20&  0.04&   0.7&   3.2&   0.6&   3.5&   0.8&  17.1&   6.5&  43.5&   8.7&  14.3&   8.0 \\ 
 295& 112021.691+353553.94&  0.0811&  13.4&  0.28&  0.04&   0.4&   3.6&   0.2&   0.9&   0.3&   9.4&   0.4&   9.8&  54.0&   9.9&  15.0 \\ 
 296& 112202.470+070632.18&  0.2316&  57.7&  0.30&  0.15&   1.3&   1.3&   0.0&   1.1&   0.0&   4.4&   0.0&  74.5&   9.0&  11.1&   0.0 \\ 
 297& 112208.234+193236.20&  0.0880&  60.7&  0.25&  0.00&   3.2&   0.3&  -0.3&   0.3&   0.1&   3.1&   0.6&  21.2&  15.5&  38.2&  20.9 \\ 
 298& 112222.990+484047.58&  0.0631&  12.9&  0.20&  0.00&   2.8&   0.5&   0.1&   0.5&   0.0&  16.1&   2.2&  20.1&  34.8&  21.4&   5.3 \\ 
 299& 112223.246+242330.91&  0.2935& 145.9&  0.60&  0.00&   1.4&   2.4&   2.1&   2.0&   0.0&  14.5&   0.0&  14.9&   0.0&  48.9&  21.6 \\ 
 300& 112253.614+512030.28&  0.0342&   2.1&  0.30&  0.00&   1.3&   2.2&   0.5&   1.9&   0.0&  19.2&   9.6&   8.9&  52.4&   0.0&   9.8 \\ 
 301& 112306.144+020254.77&  0.1380&  20.0&  0.29&  0.09&   4.9&   0.3&   0.5&   0.1&   0.2&  16.2&   9.4&  53.0&   0.0&   5.4&  15.1 \\ 
 302& 112333.962+010735.58&  0.0722&   5.5&  0.30&  0.09&   0.3&   4.4&   0.0&   1.8&   0.1&   0.0&   0.0&  16.3&   3.3&  80.3&   0.0 \\ 
 303& 112342.204+193816.42&  0.0748&  41.5&  0.93&  0.00&   1.1&   6.0&   2.0&   2.8&   0.0&   4.8&   0.8&   1.1&  58.7&  13.9&  20.4 \\ 
 304& 112405.489+140053.82&  0.2063&  65.1&  0.55&  0.09&   1.3&   1.8&  -0.2&   1.5&   0.0&   7.3&   1.2&   9.1&   9.8&  12.8&  58.4 \\ 
 305& 112415.972+250235.71&  0.1845&  64.1&  0.36&  0.00&   1.3&   1.3&  -0.1&   1.1&   0.0&   4.2&   0.2&  11.5&   4.5&  47.7&  31.8 \\ 
 306& 112442.454+385909.32&  0.1588&  28.6&  0.23&  0.00&   1.4&   1.9&   0.1&   3.5&   0.0&   4.4&   0.0&  95.0&   0.1&   0.0&   0.0 \\ 
 307& 112555.174+004958.76&  0.1807&  25.3&  0.31&  0.08&   1.2&   1.9&  -0.0&   1.4&   0.0&  32.1&   1.0&  66.8&   0.0&   0.0&   0.0 \\ 
 308& 112611.611+351753.12&  0.0375&   9.0&  0.55&  0.00&   1.7&   5.2&   0.9&  -0.3&   0.4&   7.0&   1.9&   0.0&  34.5&  14.5&  40.6 \\ 
 309& 112617.110+520457.25&  0.0340&   2.1&  0.58&  0.00&   0.4&   3.8&   0.3&   2.9&   0.5&   9.2&   0.9&   2.9&  66.1&  20.0&   0.0 \\ 
 310& 112702.311+083615.05&  0.1463&  12.7&  0.15&  0.13&   1.2&   1.5&   1.1&   2.3&   0.0&  15.3&   1.5&  83.2&   0.0&   0.0&   0.0 \\ 
 311& 112737.846+443444.22&  0.1470&  13.4&  0.25&  0.00&   1.3&   2.3&   0.7&   1.0&   0.4&  14.5&   0.2&  80.4&   4.3&   0.0&   0.0 \\ 
 312& 112750.220+245202.15&  0.1143&  24.2&  0.42&  0.00&   1.1&   1.9&   0.1&   1.4&   0.0&  12.6&   5.9&  60.8&  18.5&   0.0&   0.0 \\ 
 313& 112814.059+575034.54&  0.1210&  37.6&  0.52&  0.00&   1.6&   1.4&  -0.2&   1.6&   0.0&  13.4&   0.4&  28.6&  57.6&   0.0&   0.0 \\ 
 314& 112844.189+234053.38&  0.1318&  48.7&  0.66&  0.00&   1.0&   4.0&  -0.2&   3.3&   0.2&   8.2&   0.6&   9.3&  14.2&  10.1&  56.5 \\ 
 315& 112856.294-011722.24&  0.1456&  15.7&  0.13&  0.07&   0.8&   0.7&   0.2&   0.2&   0.0&  15.2&   0.0&  48.0&  20.1&  14.7&   1.6 \\ 
 316& 112857.187+475300.95&  0.1107&  18.6&  0.18&  0.01&   1.9&   0.3&   0.3&  -0.3&   0.2&   1.8&   3.5&  39.9&   1.1&  37.4&  15.6 \\ 
 317& 112911.326+621331.19&  0.1920&  84.5&  0.43&  0.00&   1.0&   2.6&   1.5&   1.3&   0.1&   8.1&   0.7&   7.5&   0.0&  12.0&  71.3 \\ 
 318& 112916.368+602853.14&  0.1109&  20.3&  0.38&  0.00&   1.8&   1.8&   0.3&   2.3&   0.0&  20.7&   0.1&  79.2&   0.0&   0.0&   0.0 \\ 
 319& 113040.846+562910.04&  0.0622&  27.2&  0.48&  0.00&   3.8&   0.6&   0.2&   1.8&   0.3&  10.7&   2.9&  17.8&  16.5&  40.7&  10.8 \\ 
 320& 113042.686+153846.38&  0.2982& 172.3&  0.21&  0.04&   0.9&   1.1&   0.3&   0.6&   0.0&   2.4&   1.1&  28.7&   0.0&  67.7&   0.0 \\ 
 321& 113043.870+452939.20&  0.1817&  15.7&  0.31&  0.00&   1.8&   2.5&   0.5&   2.0&   0.1&  26.0&   0.0&  71.2&   0.0&   0.0&   0.0 \\ 
 322& 113053.258+111440.79&  0.3396&  41.8&  0.12&  0.08&   6.8&   0.8&  -0.0&   1.7&   0.0&   0.0&   0.0&  94.0&   0.0&   6.0&   0.0 \\ 
 323& 113104.411+552455.15&  0.0936&   9.8&  0.18&  0.00&   1.5&   1.7&   0.3&   3.3&   0.1&  14.9&   3.3&  13.8&  58.8&   8.9&   0.0 \\ 
 324& 113209.343-023551.87&  0.1054&  22.5&  0.77&  0.14&   0.7&   5.0&  -0.4&   3.2&   0.1&   3.8&   0.6&   2.4&   9.8&  26.8&  56.5 \\ 
 325& 113233.089+142615.93&  0.0741&   2.7&  0.03&  0.00&   1.5&   0.6&   0.1&   0.7&   0.0&  28.4&   8.6&  49.1&  13.9&   0.0&   0.0 \\ 
 326& 113338.642+041146.22&  0.3359&  62.3&  0.27&  0.02& -46.2&  -0.0&   0.2&   1.2&   0.0&   0.0&   9.1&  52.8&  31.4&   0.0&   0.0 \\ 
 327& 113340.646+062001.73&  0.3735&  47.5&  0.31&  0.10&   1.9&   3.8&  -0.1&   2.9&   0.0&   5.7&   0.7&  60.9&  32.7&   0.0&   0.0 \\ 
 328& 113349.613+020514.98&  0.1778&  19.2&  0.23&  0.06&   0.7&   0.9&  -0.4&   1.1&   0.1&  26.5&   0.0&  73.4&   0.0&   0.0&   0.0 \\ 
 329& 113351.934+572715.75&  0.1626&  16.2&  0.04&  0.00&   2.8&   0.3&   0.1&   1.7&   0.0&  31.5&   0.0&  68.4&   0.0&   0.0&   0.0 \\ 
 330& 113437.522+250301.86&  0.1325&  14.3&  0.38&  0.00&   1.6&   2.3&   0.4&   2.2&   0.0&  24.6&   0.0&  75.2&   0.0&   0.0&   0.0 \\ 
 331& 113509.103+360935.21&  0.1992&  31.3&  0.00&  0.00&   0.3&   0.8&  -0.4&   0.1&   0.0&   4.9&   0.7&  60.9&   9.1&  24.2&   0.0 \\ 
 332& 113753.921+392157.84&  0.1242&  23.2&  0.26&  0.00&   1.8&   1.3&   0.0&   1.6&   0.1&   2.4&   1.1&  61.9&   0.0&  33.7&   0.0 \\ 
 333& 113800.526+335556.51&  0.2381& 129.2&  0.21&  0.00&   0.9&   1.1&   0.5&   0.7&   0.0&   1.7&   0.8&  27.8&   9.5&  13.6&  46.4 \\ 
 334& 113929.244+235325.53&  0.0715&  21.6&  0.90&  0.00&   1.0&   1.3&   0.4&   1.7&   0.0&   3.3&   0.0&   4.4&  41.3&  43.8&   7.1 \\ 
 335& 113941.926+360915.87&  0.1273&  12.8&  0.29&  0.01&   2.3&   1.7&   2.5&   2.3&   0.0&  20.2&   0.0&  62.2&  16.6&   0.0&   0.0 \\ 
 336& 114039.694+034534.13&  0.1955&  24.2&  0.06&  0.00&   3.1&  -0.1&  -0.1&   0.5&   0.0&   3.2&   1.1&  94.1&   0.0&   1.6&   0.0 \\ 
 337& 114043.404+265201.48&  0.1994&  98.1&  0.07&  0.02&   1.3&   2.3&  -0.3&   2.0&   0.0&   1.5&   2.6&  15.4&   1.2&  36.2&  43.1 \\ 
 338& 114056.146+140212.39&  0.1002&  13.8&  0.32&  0.11&   1.9&   1.3&   0.4&   2.7&   0.1&   6.0&   0.9&  44.6&  11.5&  31.5&   4.1 \\ 
 339& 114146.169+354628.83&  0.1287&  16.3&  0.02&  0.00&   1.4&   1.3&   0.4&   1.7&   0.0&   3.0&   6.3&  90.5&   0.0&   0.0&   0.0 \\ 
 340& 114159.400+265700.06&  0.0508&  10.7&  0.09&  0.05&   1.7&   1.3&  -0.1&   2.0&   0.2&  21.8&   1.6&  46.9&   2.0&  26.4&   0.0 \\ 
 341& 114315.900+095305.77&  0.0896&  10.6&  0.19&  0.11&   0.6&   1.9&   1.1&   2.3&   0.0&   7.2&   2.1&   9.4&  51.9&  29.4&   0.0 \\ 
 342& 114318.211+082127.19&  0.1856&  19.0&  0.00&  0.02&  -7.4&  -0.1&   0.2&   0.7&   0.0&   0.0&   0.0& 100.0&   0.0&   0.0&   0.0 \\ 
 343& 114342.730+511937.87&  0.1460&  46.0&  0.75&  0.00&   1.0&   6.9&   2.3&   3.1&   0.0&  23.3&   6.2&  15.9&  17.6&   0.0&  34.6 \\ 
 344& 114407.430+264717.72&  0.1336&  18.3&  0.10&  0.05&   1.3&   0.8&   0.2&   0.7&   0.0&   3.1&  17.0&  63.4&  16.4&   0.0&   0.0 \\ 
 345& 114411.018+053735.62&  0.1775&  35.1&  0.66&  0.00&   2.5&   0.9&   1.8&   1.5&   0.2&  10.4&   0.7&  28.4&   0.8&  59.4&   0.0 \\ 
 346& 114627.895+201258.75&  0.0966&  10.3&  0.30&  0.00&   1.8&   3.2&   1.9&   2.1&   0.0&  13.9&   4.5&  81.6&   0.0&   0.0&   0.0 \\ 
 347& 114657.358+323914.31&  0.0328&   1.2&  0.09&  0.01&   0.7&   1.1&   0.4&   2.1&   0.0&  37.7&   0.2&  61.4&   0.7&   0.0&   0.0 \\ 
 348& 114741.110+375938.16&  0.1629&  19.2&  0.51&  0.02&   1.0&   2.4&   0.5&   1.9&   0.0&  34.8&   0.0&  41.7&  23.5&   0.0&   0.0 \\ 
 349& 114903.382+245842.99&  0.1741&  68.0&  0.67&  0.04&   1.2&   2.8&  -0.4&   2.6&   0.0&   6.6&   1.5&  17.7&   0.0&  55.1&  18.6 \\ 
 350& 115037.526+013000.57&  0.0778&  11.8&  0.49&  0.04&   1.7&   2.0&   0.4&   0.6&   0.0&  12.2&   5.6&  82.3&   0.0&   0.0&   0.0 \\ 
 351& 115052.982+460448.19&  0.2895& 114.2&  0.18&  0.00&   0.9&   1.8&   0.7&   1.3&   0.0&   1.1&   0.4&  53.2&  15.4&  29.7&   0.0 \\ 
 352& 115208.570+481658.37&  0.0547&   3.1&  0.33&  0.03&   0.6&   2.0&  -0.3&   2.1&   0.6&   4.3&   1.0&  17.1&  55.2&   8.5&  12.6 \\ 
 353& 115225.538-011602.85&  0.0606&  20.2&  0.59&  0.03&   3.2&   2.5&   2.1&   1.6&   0.3&   6.6&   1.0&   3.0&  35.8&  22.3&  30.3 \\ 
 354& 115311.890+005030.74&  0.2834& 161.9&  0.31&  0.04&   2.4&   0.9&   0.0&   1.5&   0.0&   0.8&   0.0&  19.9&  10.0&  50.6&  18.0 \\ 
 355& 115355.538-031035.27&  0.0884&  13.4&  0.37&  0.04&   1.5&   2.6&   0.4&   3.4&   0.4&  12.5&   2.6&  20.7&  29.3&  28.5&   5.3 \\ 
 356& 115431.471+312024.15&  0.1587&  26.3&  0.25&  0.03&   1.7&   1.2&   0.2&   0.7&   0.0&  16.3&   0.0&  83.7&   0.0&   0.0&   0.0 \\ 
 357& 115446.094+300830.45&  0.1781&  23.2&  0.23&  0.00&   1.6&   1.8&   0.1&   1.2&   0.1&   7.0&   0.0&  92.6&   0.0&   0.0&   0.0 \\ 
 358& 115640.214+583031.94&  0.2099&  38.5&  0.58&  0.00&   1.9&   2.3&   1.8&   2.9&   0.0&  33.4&   1.6&  64.9&   0.1&   0.0&   0.0 \\ 
 359& 115730.590+210925.93&  0.0687&   3.2&  0.10&  0.08&   0.7&   4.8&   1.7&   3.8&   0.0&   0.0&   8.6&  11.6&  60.6&  19.1&   0.0 \\ 
 360& 115821.650+363820.46&  0.0656&  36.6&  0.18&  0.00&   1.1&   1.0&  -0.2&   0.5&   0.3&   3.3&   2.1&  15.4&  18.3&  38.5&  21.6 \\ 
 361& 115837.723-021710.95&  0.0880&  27.4&  0.30&  0.04&   1.2&   0.9&   0.2&   0.6&   0.1&  12.8&   0.6&  30.2&  12.9&  43.1&   0.0 \\ 
 362& 115931.855+430842.78&  0.3168&  69.7&  0.21&  0.00&   2.2&   0.8&  -0.1&   0.8&   0.0&   7.5&   0.0&  91.5&   0.0&   0.0&   0.0 \\ 
 363& 115950.669+191523.45&  0.2362& 112.7&  0.41&  0.06&   1.4&   2.1&   0.4&   1.9&   0.0&   6.2&   0.0&  15.8&   1.3&  17.8&  58.6 \\ 
 364& 120144.575+375612.04&  0.0788&   5.6&  0.19&  0.00&   1.2&   1.0&   0.2&   1.6&   0.0&   0.8&   0.0&   7.9&  43.1&  48.2&   0.0 \\ 
 365& 120222.212+243419.19&  0.0436&   2.8&  0.43&  0.00&   0.7&   2.0&  -0.0&   2.5&   0.1&  12.5&   0.0&  21.6&  58.7&   7.0&   0.0 \\ 
 366& 120251.859+402448.09&  0.1813&  36.4&  0.34&  0.00&   2.2&   1.4&  -0.0&   2.3&   0.0&  18.4&   2.0&  79.4&   0.0&   0.0&   0.0 \\ 
 367& 120336.979+604812.24&  0.0637&   2.4&  0.03&  0.00&   9.8&   0.1&   0.9&   0.2&   0.1&  22.4&   2.0&  19.2&  56.0&   0.0&   0.0 \\ 
 368& 120353.909+064554.65&  0.1462&  10.6&  0.18&  0.00&   1.5&   2.4&   1.5&   1.5&   0.4&   4.4&   4.3&  89.8&   0.0&   0.0&   0.0 \\ 
 369& 120419.075-001855.82&  0.0938&  17.1&  0.17&  0.03&   1.3&   1.2&   0.4&   0.7&   0.0&   0.0&   0.0& 100.0&   0.0&   0.0&   0.0 \\ 
 370& 120454.713+001840.08&  0.1002&  10.6&  0.46&  0.03&   0.4&   5.7&   0.2&   2.1&   0.0&   4.6&   6.0&  31.0&  48.8&   1.3&   8.0 \\ 
 371& 120541.890+184154.48&  0.1774&  36.3&  0.33&  0.02&   1.0&   4.5&   0.2&   2.3&   0.2&   2.6&   1.0&  24.2&  12.3&  45.2&  13.0 \\ 
 372& 120543.690+513741.13&  0.0893&   8.3&  0.44&  0.00&   0.8&   1.6&   2.4&   1.5&   0.0&  26.7&   1.9&  18.2&  53.3&   0.0&   0.0 \\ 
 373& 120620.518+245619.89&  0.0895&   6.6&  0.45&  0.06&   1.8&   3.0&   0.7&   2.7&   0.0&  12.3&   7.3&  33.3&  22.2&  11.3&  13.5 \\ 
 374& 120627.955+253423.64&  0.0989&  13.2&  0.42&  0.06&   1.1&   1.9&   0.2&   2.3&   0.0&  10.4&   6.5&  83.0&   0.0&   0.0&   0.0 \\ 
 375& 120630.811+091855.15&  0.1788&  14.6&  0.18&  0.00&   1.0&   1.6&  -1.3&   1.1&   0.0&   3.6&   3.8&  92.5&   0.0&   0.0&   0.0 \\ 
 376& 120708.652+065244.84&  0.1726& 101.8&  0.54&  0.00&   2.7&   1.7&   0.9&   2.0&   0.1&   4.8&   1.1&  25.2&   0.2&  24.3&  43.5 \\ 
 377& 120811.275+402151.24&  0.1126&  17.5&  0.15&  0.00&   1.7&   1.7&   0.5&   1.4&   0.0&   0.7&   4.2&  95.0&   0.0&   0.0&   0.0 \\ 
 378& 121117.789+400715.89&  0.1955&  54.3&  0.44&  0.00&   1.2&   2.1&   0.1&   1.4&   0.0&   0.8&   0.3&  34.0&   9.4&  19.1&  33.8 \\ 
 379& 121136.034+142023.25&  0.1455&   9.0&  0.29&  0.13&  34.5&   0.0&   0.7&   0.2&   0.0&  13.2&   1.9&  84.9&   0.0&   0.0&   0.0 \\ 
 380& 121258.150+121753.46&  0.2035&  50.4&  0.13&  0.03&   2.7&   0.6&  -0.0&   1.6&   0.1&   0.3&   2.2&  32.8&  12.4&  37.3&  14.7 \\ 
 381& 121333.026+142900.10&  0.0640&   3.3&  0.44&  0.12&   0.8&   2.2&   0.7&   0.9&   0.4&  24.0&   6.7&   7.3&  60.5&   1.2&   0.0 \\ 
 382& 121658.049+262829.45&  0.1313&  23.2&  0.50&  0.10&   0.6&   4.5&   0.2&   1.4&   0.0&  19.8&   4.6&  24.7&   7.6&   3.9&  39.2 \\ 
 383& 121702.429+390437.33&  0.0654&   8.6&  0.51&  0.00&   0.8&   2.3&  -0.4&   1.8&   0.0&  11.0&   3.3&  11.6&  58.4&   0.9&  14.4 \\ 
 384& 121744.033+284912.46&  0.1108&   6.5&  0.13&  0.10&   1.6&   1.5&   1.3&   1.8&   0.3&  31.7&   4.9&  50.2&  12.1&   0.0&   0.0 \\ 
 385& 121937.704+435924.54&  0.1247&  19.9&  0.22&  0.00&   1.7&   1.1&  -0.0&   2.7&   0.3&  11.6&   0.7&  23.4&   9.6&  33.8&  19.6 \\ 
 386& 121937.906+380245.18&  0.0520&   2.7&  0.25&  0.00&   0.6&   2.7&  -0.3&   3.7&   0.6&   1.4&   0.5&  21.7&   4.3&  71.5&   0.0 \\ 
 387& 122156.458+000948.22&  0.1063&  18.3&  0.43&  0.03&   1.8&   1.6&   0.7&   0.8&   0.2&  35.2&   8.6&  55.6&   0.1&   0.0&   0.0 \\ 
 388& 122206.689+113156.10&  0.1414&  20.5&  0.17&  0.00&   2.1&   0.8&   0.0&   0.6&   0.0&  14.2&   1.0&  84.7&   0.0&   0.0&   0.0 \\ 
 389& 122240.466+150205.49&  0.0724&   1.1&  0.26&  0.06&   0.4&   3.1&   0.4&   1.2&   2.2&  15.0&  13.1&  23.8&  45.3&   0.0&   0.0 \\ 
 390& 122256.134-011247.99&  0.1462&  24.0&  0.35&  0.04&   1.3&   1.1&   1.9&   2.8&   0.1&   3.1&   0.0&  21.6&   5.2&  36.4&  33.6 \\ 
 391& 122422.781+213352.28&  0.0756&  20.3&  0.50&  0.07&   1.2&   3.4&   0.5&   2.6&   0.0&   9.5&   3.6&  31.0&  18.6&  36.0&   0.2 \\ 
 392& 122424.122+533442.54&  0.2137&  83.6&  0.53&  0.05&   1.2&   2.6&   0.1&   1.4&   0.0&  14.8&   0.5&  28.3&   9.7&   0.0&  46.2 \\ 
 393& 122636.197+225953.55&  0.0681&   4.8&  0.12&  0.09&   2.4&   1.3&   3.2&   1.2&   0.2&  12.7&   9.7&  17.2&  34.2&  24.1&   1.1 \\ 
 394& 122700.286+295058.69&  0.2079&  59.5&  0.00&  0.04&   0.2&   0.3&   0.1&   0.2&   0.0&   0.0&   0.0&  42.4&   0.0&  37.3&  20.0 \\ 
 395& 122718.550-002428.53&  0.1141&   9.0&  0.00&  0.04&   2.0&   0.7&  -0.1&   1.6&   0.0&  35.9&   0.0&  53.3&   7.6&   3.2&   0.0 \\ 
 396& 122909.250+100435.36&  0.1377&  15.5&  0.18&  0.00&   0.7&   1.0&   0.0&   1.0&   0.0&  14.7&   1.6&  44.9&  27.1&   0.0&  11.8 \\ 
 397& 123015.010+021457.70&  0.1029&  17.0&  0.09&  0.00&   0.8&   1.2&   0.1&   2.2&   0.2&  12.8&  10.4&  19.1&  18.0&  15.0&  24.2 \\ 
 398& 123032.861+215848.31&  0.2183&  45.4&  0.22&  0.05&   0.4&   1.2&   0.1&   0.3&   0.1&   7.3&   7.2&  50.2&  22.1&   0.0&  12.3 \\ 
 399& 123054.458+103831.59&  0.2223&  52.2&  0.09&  0.02&   4.7&   0.4&  -0.2&   1.0&   0.2&   0.1&   0.0&  56.8&   0.0&   0.0&  42.2 \\ 
 400& 123114.863+412840.63&  0.2171&  99.1&  0.10&  0.00&   1.1&   1.1&   0.3&   1.3&   0.0&   0.4&   0.1&  22.8&   0.8&  21.6&  54.3 \\ 
 401& 123126.964+032744.64&  0.1425&  63.5&  0.77&  0.04&   1.7&   3.3&   0.4&   2.0&   0.0&   9.8&   2.5&  12.2&  46.7&   0.0&  28.2 \\ 
 402& 123305.035+480000.32&  0.2138&  75.8&  0.39&  0.00&   1.6&   2.3&  -0.3&   3.0&   0.3&   4.8&   1.5&   7.7&  21.7&  12.7&  50.4 \\ 
 403& 123339.146+270817.64&  0.2282&  33.3&  0.49&  0.04&   2.3&   2.4&   0.7&   1.3&   0.2&  12.8&   0.0&  87.0&   0.0&   0.0&   0.0 \\ 
 404& 123443.783+612453.67&  0.0994&  18.0&  0.02&  0.00&   1.5&   1.1&   0.1&   1.2&   0.0&   8.3&   0.0&  91.4&   0.0&   0.0&   0.0 \\ 
 405& 123614.983+015809.80&  0.1399&  18.2&  0.44&  0.00&   2.0&   2.1&   0.1&   2.0&   0.5&  11.8&   6.7&  37.0&  19.8&   0.2&  20.9 \\ 
 406& 123820.722+482220.99&  0.1973&  60.2&  0.74&  0.00&   1.1&   1.9&   0.0&   1.1&   0.0&   6.5&   0.9&  40.1&   0.0&  51.6&   0.8 \\ 
 407& 123822.282+473301.46&  0.2491& 103.1&  0.60&  0.00&   0.7&   1.4&   0.4&  -0.3&   0.0&   9.7&   0.0&  26.3&   0.0&   0.1&  63.3 \\ 
 408& 123827.545+603019.77&  0.1569&  48.9&  0.31&  0.00&   0.9&   1.7&   0.3&   1.8&   0.5&   4.2&   3.5&   9.2&   7.4&  72.5&   0.0 \\ 
 409& 123841.064+591119.08&  0.1183&  36.8&  0.67&  0.00&   1.0&   2.1&  -0.4&   1.5&   0.2&  14.5&   7.1&   7.2&  16.4&  20.8&  31.9 \\ 
 410& 123846.505+363639.19&  0.1919&  32.0&  0.10&  0.00&   1.7&   1.2&  -0.1&   1.1&   0.0&   4.7&   0.0&  41.5&  19.3&  25.1&   8.2 \\ 
 411& 123904.289+364530.70&  0.1911&  45.6&  0.21&  0.00&   1.1&   2.2&   0.1&   1.3&   0.0&   1.8&   0.0&  38.6&  32.0&  18.2&   9.3 \\ 
 412& 123928.978+580300.67&  0.1506&  53.7&  0.28&  0.00&   1.6&   1.1&   0.3&   0.7&   0.0&   2.2&   0.4&  47.2&   0.0&  19.9&  29.6 \\ 
 413& 123936.050+122620.00&  0.0409&  19.4&  0.20&  0.11&   1.0&   2.1&  -0.5&   1.8&   0.3&   0.9&   0.3&   6.0&  10.1&  67.4&  14.5 \\ 
 414& 124018.902+164629.92&  0.0705&  26.0&  0.20&  0.02&   1.0&   2.4&   0.1&   2.3&   0.7&   3.0&   2.8&  39.6&  44.1&   8.9&   0.0 \\ 
 415& 124100.271+452832.96&  0.1569&  20.8&  0.30&  0.00&   0.8&   1.4&   0.1&   1.3&   0.0&   0.3&   1.6&  64.5&   0.0&  31.3&   2.3 \\ 
 416& 124204.380+272346.96&  0.0576&  15.5&  0.20&  0.11&   1.1&   1.1&   0.8&   1.1&   0.0&  10.5&   1.0&  22.7&   6.1&  25.0&  34.8 \\ 
 417& 124204.666+150905.67&  0.0872&  31.8&  0.20&  0.03&   1.3&   1.3&  -0.2&   1.3&   0.3&   3.8&   3.4&  28.1&  22.2&  25.5&  15.1 \\ 
 418& 124246.428+114849.30&  0.2336&  87.6&  0.00&  0.06&   0.6&   1.3&  -0.2&   0.5&   0.0&   0.0&   0.0&  37.1&  30.8&   2.4&  29.5 \\ 
 419& 124252.958+023700.90&  0.0844&   7.0&  0.36&  0.01&   0.6&   2.7&   0.4&   2.0&   0.8&  18.3&   5.8&  14.6&  22.1&  21.6&  15.5 \\ 
 420& 124309.629+270024.42&  0.1761&  16.1&  0.28&  0.09&   0.9&   0.9&  -0.0&   1.2&   0.0&  11.9&  24.0&  26.7&  37.4&   0.0&   0.0 \\ 
 421& 124350.398+315324.87&  0.1058&  18.0&  0.05&  0.04&   1.7&   0.9&   0.6&   0.6&   0.0&   5.8&   0.0&  94.0&   0.0&   0.0&   0.0 \\ 
 422& 124354.629+163309.49&  0.1295&   5.2&  0.10&  0.03&   0.5&   1.3&   0.9&   1.6&   0.0&   6.7&   0.2&  83.0&  10.1&   0.0&   0.0 \\ 
 423& 124406.722+621036.21&  0.2339&  46.2&  0.17&  0.02&   0.1&   0.6&   0.1&   0.7&   0.0&   0.3&   0.0&  81.4&   9.7&   7.5&   0.0 \\ 
 424& 124427.307+400733.86&  0.2479&  79.3&  0.25&  0.00&   0.9&   1.3&   0.5&   0.8&   0.1&   2.8&   3.8&  24.2&  28.1&  12.4&  28.5 \\ 
 425& 124458.783+140618.37&  0.2278&  64.0&  0.66&  0.03&   1.2&   1.8&   0.1&   2.3&   0.0&  10.9&   0.8&  37.6&   0.0&   3.2&  47.2 \\ 
 426& 124521.422-014735.49&  0.2155&  37.8&  0.49&  0.02&   1.5&   2.8&  -0.0&   2.4&   0.1&  14.6&   2.8&  75.1&   3.7&   1.2&   0.0 \\ 
 427& 124534.169+402559.13&  0.0822&  24.5&  0.28&  0.00&   1.1&   1.8&  -0.0&   1.8&   0.0&   3.6&   0.0&  35.3&   0.0&  60.8&   0.0 \\ 
 428& 124645.722+345835.08&  0.1600&  47.6&  0.40&  0.01&   1.0&   1.7&   0.0&   0.2&   0.9&   1.6&   1.2&  39.4&   0.0&  35.2&  20.6 \\ 
 429& 124700.254+351817.02&  0.1684&  19.6&  0.16&  0.04&   0.6&   1.1&   1.0&   0.8&   0.0&   0.1&   5.5&  84.4&  10.0&   0.0&   0.0 \\ 
 430& 124700.708+034643.72&  0.1374&  24.4&  0.03&  0.00&   1.5&   1.1&   0.1&   1.5&   0.0&   1.7&   0.0&  97.8&   0.0&   0.0&   0.0 \\ 
 431& 124728.826+384013.83&  0.1871&  30.3&  0.43&  0.00&   1.1&   2.8&   0.1&   2.1&   0.0&   8.3&   1.5&  69.4&  20.4&   0.0&   0.0 \\ 
 432& 124755.409+053630.34&  0.0796&   4.7&  0.31&  0.00&   0.6&   2.2&   0.5&   3.5&   0.4&  11.9&   1.4&  15.8&  44.5&   8.7&  16.2 \\ 
 433& 124835.986+131116.31&  0.2328&  50.4&  0.08&  0.03&   0.6&   1.0&   0.1&   0.4&   0.0&   1.4&   0.0&  82.1&   1.6&  13.6&   0.0 \\ 
 434& 124942.612+313858.65&  0.1649&  20.8&  0.19&  0.03&   1.1&   0.8&  -0.0&   1.6&   0.2&  26.8&   0.1&  73.0&   0.0&   0.0&   0.0 \\ 
 435& 125004.553+293335.00&  0.0620&   2.3&  0.00&  0.04&   2.4&   0.3&   0.5&   0.7&   0.2&   7.8&  16.4&  60.1&  15.4&   0.0&   0.0 \\ 
 436& 125017.088+632520.30&  0.1674&  23.9&  0.45&  0.01&   2.4&   1.2&   0.5&   2.6&   0.0&   5.8&   0.0&  94.0&   0.2&   0.0&   0.0 \\ 
 437& 125306.727+181527.48&  0.2071&  66.3&  0.17&  0.06&   2.3&   1.8&   0.4&   2.1&   0.0&   0.5&   0.9&  40.0&   0.0&  15.5&  42.9 \\ 
 438& 125633.547+391759.91&  0.1269&   9.7&  0.05&  0.00&   1.2&   1.2&   0.6&  -0.3&   0.0&   0.0&   0.0& 100.0&   0.0&   0.0&   0.0 \\ 
 439& 125720.429+460323.04&  0.0700&  23.9&  0.42&  0.00&   1.9&   2.6&   0.9&   2.5&   0.0&   6.4&   3.3&  12.0&  77.9&   0.0&   0.0 \\ 
 440& 125738.234+313328.00&  0.0791&  16.5&  0.00&  0.06&   0.8&   0.5&  -0.1&   0.7&   0.1&   6.6&   4.8&  40.2&  11.0&  35.2&   1.9 \\ 
 441& 125744.112+290113.38&  0.0265&   0.8&  0.12&  0.04&   0.8&   2.3&  -0.3&   0.9&   0.1&  12.3&   1.4&   4.1&  63.4&   0.8&  17.6 \\ 
 442& 125745.302+275421.54&  0.0272&   0.2&  0.05&  0.07&   0.5&   2.2&   0.4&   0.9&   1.2&  16.7&   9.9&   3.8&  67.3&   0.0&   0.0 \\ 
 443& 125754.862+270327.24&  0.1372&  23.0&  0.26&  0.01&   1.8&   0.9&   0.4&   1.1&   0.1&  16.8&   2.1&  78.1&   0.0&   1.6&   0.0 \\ 
 444& 125820.722+613039.55&  0.0907&  34.4&  0.55&  0.00&   0.7&   5.2&   0.2&   1.6&   3.1&   3.3&   3.5&  14.2&   0.0&  43.8&  29.8 \\ 
 445& 125842.590+274537.83&  0.0292&   0.0&  0.32&  0.05&   0.7&   0.5&  -0.2&  -2.0&  15.9&  40.1&  43.9&   0.0&   0.0&   0.0&   0.0 \\ 
 446& 125946.279+274446.55&  0.0326&   0.3&  0.23&  0.04&   0.6&   0.7&  -0.1&   2.3&   1.2&  30.3&   7.8&   0.0&  60.6&   0.0&   0.0 \\ 
 447& 125948.276+185400.51&  0.1743&  45.3&  0.66&  0.09&   1.4&   5.5&   1.8&   2.4&   0.0&  34.0&   7.5&  17.7&   0.2&   0.0&  38.6 \\ 
 448& 125956.251+380724.56&  0.2666&  61.3&  0.34&  0.00&   2.8&   0.9&   0.1&   0.4&   0.0&   0.0&   0.0&  87.5&   0.0&  12.5&   0.0 \\ 
 449& 130105.654+280343.38&  0.0249&   0.3&  0.19&  0.06&   0.2&   0.4&  -0.1&   3.6&   0.2&  18.4&  13.8&   9.7&  57.8&   0.0&   0.0 \\ 
 450& 130130.720+211947.58&  0.1149&  15.8&  0.47&  0.14&   1.5&   2.0&   0.9&   2.5&   0.3&  18.0&   3.2&  48.7&   8.0&  19.9&   0.0 \\ 
 451& 130501.548+071428.18&  0.1279&  22.1&  0.25&  0.04&   1.1&   1.6&   0.3&   2.9&   0.0&  14.9&   0.0&  85.1&   0.0&   0.0&   0.0 \\ 
 452& 130544.712-033416.00&  0.0841&  18.7&  1.24&  0.01&   0.8&   4.5&  -0.9&   1.8&   0.1&   3.3&   0.0&   8.5&  51.6&  14.3&  22.3 \\ 
 453& 130619.274-005855.78&  0.2461&  58.5&  0.23&  0.01&   1.4&   1.2&  -0.1&   1.1&   0.0&   0.0&   0.0& 100.0&   0.0&   0.0&   0.0 \\ 
 454& 130733.077+291941.02&  0.1280&   8.4&  0.37&  0.03&   1.5&   1.7&   0.3&   2.6&   0.7&  21.0&  18.3&  38.5&  17.7&   0.0&   0.0 \\ 
 455& 130737.766+011019.34&  0.2174& 140.1&  0.41&  0.00&   0.8&   1.9&   0.2&   0.7&   0.0&   4.6&   0.4&  16.4&   0.0&  60.4&  18.0 \\ 
 456& 130808.990+103440.12&  0.1564&  98.4&  0.74&  0.00&   1.1&   6.5&   0.7&   3.3&   0.5&   5.3&   3.0&   3.2&   7.0&  16.8&  62.5 \\ 
 457& 130843.886+611118.35&  0.2191&  32.5&  0.22&  0.01&   2.1&   1.0&   0.6&   1.7&   0.0&  19.8&   0.4&  79.7&   0.0&   0.0&   0.0 \\ 
 458& 130933.156+223318.44&  0.1813&  13.7&  0.26&  0.04&   3.0&   0.8&   1.6&   2.1&   0.0&   6.1&   0.0&  93.5&   0.0&   0.0&   0.0 \\ 
 459& 131022.390+362607.80&  0.1886&  53.2&  0.18&  0.00&   3.5&   0.3&  -0.2&  -0.7&   0.0&   5.8&   1.3&  20.8&   0.0&  19.7&  52.3 \\ 
 460& 131107.342+251951.38&  0.0803&  11.0&  0.12&  0.04&   1.4&   1.1&   0.5&   0.8&   0.0&   5.6&   1.1&  22.6&   8.4&  19.2&  43.1 \\ 
 461& 131154.862+522504.42&  0.2285&  85.4&  0.15&  0.00&   1.0&   1.6&   0.0&   2.4&   0.0&   2.5&   0.6&  19.2&   0.0&  77.1&   0.0 \\ 
 462& 131207.759+391837.33&  0.0680&   1.5&  0.12&  0.00&   0.6&   1.1&   0.2&  -0.3&   0.2&   8.0&  20.1&  41.5&  30.2&   0.0&   0.0 \\ 
 463& 131431.711+090119.59&  0.0511&   1.7&  0.00&  0.00&   0.9&   1.4&   0.2&   3.7&   0.1&  17.3&   7.6&  21.4&  39.4&  12.5&   1.4 \\ 
 464& 131558.706+042131.32&  0.0769&  10.3&  0.42&  0.06&   2.2&   0.9&   0.4&   1.3&   0.0&  25.0&   3.1&  40.0&  31.9&   0.0&   0.0 \\ 
 465& 131608.280+294911.77&  0.1385&   9.4&  0.19&  0.03&   1.8&   1.2&   0.0&   2.4&   0.0&  11.7&  13.1&  75.2&   0.0&   0.0&   0.0 \\ 
 466& 131648.499+160553.91&  0.1506&  13.6&  0.31&  0.01&   1.7&   1.8&   0.1&   1.5&   0.1&   7.2&   0.6&  91.9&   0.2&   0.0&   0.0 \\ 
 467& 131700.478+113746.29&  0.1948&  37.2&  0.21&  0.03&   2.0&   5.7&  10.3&   2.6&   0.0&   6.3&   0.0&  39.8&  12.7&  37.7&   0.0 \\ 
 468& 131722.241+462307.77&  0.1802&  41.1&  0.79&  0.00&   0.8&   1.8&  -0.0&   1.6&   0.0&  10.4&   0.4&  40.5&   0.0&   0.0&  48.7 \\ 
 469& 131740.963+174152.01&  0.0731&  51.1&  0.61&  0.02&   2.0&   0.9&  -0.3&   2.2&   0.0&   4.5&   0.9&   7.6&  51.6&  24.2&  10.9 \\ 
 470& 132021.432+163039.10&  0.1771&  76.7&  0.34&  0.00&   1.4&   2.8&   0.5&   2.3&   0.0&   1.2&   1.0&  16.3&  10.6&  51.8&  18.3 \\ 
 471& 132058.574+465433.36&  0.1527&  76.2&  0.35&  0.00&   1.3&   2.7&   0.2&   2.8&   0.5&   2.6&   1.0&   5.1&   0.0&  35.0&  53.3 \\ 
 472& 132104.735+571523.44&  0.1361&  71.8&  1.09&  0.00&   1.2&   1.8&  -1.0&   0.9&   0.1&   5.9&   0.7&   3.4&  15.3&  39.6&  34.5 \\ 
 473& 132214.945+074814.28&  0.2505&  42.9&  0.07&  0.01&   1.3&   0.8&   0.3&   0.9&   0.0&   2.7&   1.0&  96.3&   0.0&   0.0&   0.0 \\ 
 474& 132241.465+324614.58&  0.1393&  22.9&  0.13&  0.00&   1.5&   0.8&   0.5&   0.7&   0.0&   2.0&   2.0&  67.5&   0.0&  25.7&   2.8 \\ 
 475& 132256.018+103957.87&  0.3244& 123.2&  0.17&  0.00&   2.1&   0.6&  -0.1&   1.1&   0.0&   2.0&   0.0&  46.0&   0.0&  51.7&   0.0 \\ 
 476& 132309.715+630008.32&  0.1740&  43.3&  0.00&  0.01&   0.7&   1.0&   0.1&   0.9&   0.0&   2.0&   0.7&  30.0&   1.7&  43.1&  22.1 \\ 
 477& 132315.578+630726.73&  0.1754&  42.0&  0.18&  0.01&   0.5&   0.6&   1.7&   0.9&   0.0&   0.2&   1.3&  26.0&   0.0&  61.7&  10.8 \\ 
 478& 132415.139+140755.07&  0.0949&  39.3&  0.44&  0.01&   0.9&   2.8&   0.1&   1.8&   0.1&  10.9&   0.4&   9.5&   0.0&  53.0&  25.1 \\ 
 479& 132419.778+282150.71&  0.1634&  20.0&  0.00&  0.00&   1.3&   0.7&  -0.7&   0.6&   0.0&   0.0&   0.0&  83.8&   0.0&  16.0&   0.0 \\ 
 480& 132540.798+070820.95&  0.1641&  52.3&  0.38&  0.00&   0.5&   4.7&   0.9&   2.6&   0.1&   1.8&   1.9&  11.1&  35.2&  10.4&  39.5 \\ 
 481& 132542.305+325503.90&  0.2926& 108.1&  0.16&  0.00&   2.6&   0.7&   0.3&   1.0&   0.0&   4.5&   0.1&  37.6&  37.6&   0.8&  19.2 \\ 
 482& 132550.630+171410.62&  0.0790&  10.8&  0.19&  0.00&   2.5&   1.1&   0.1&   1.6&   0.1&   9.2&   4.1&  22.6&  43.0&  20.2&   0.0 \\ 
 483& 132608.417+255057.18&  0.1065&  11.3&  0.09&  0.04&   1.7&   1.5&   1.3&   1.5&   0.0&   5.6&   8.0&  66.3&   0.0&   4.8&  15.3 \\ 
 484& 132722.721+313044.18&  0.1305&  23.0&  0.31&  0.03&   1.2&   1.9&   0.2&   0.5&   1.2&   4.8&   1.7&  33.0&  10.4&  10.1&  36.8 \\ 
 485& 133024.746+022325.86&  0.0786&  18.8&  0.76&  0.04&   2.2&   1.4&  -0.2&   2.1&   0.0&   4.2&   0.8&  10.8&  55.8&  12.2&  16.0 \\ 
 486& 133044.158+224225.49&  0.1505&  18.5&  0.22&  0.03&   1.3&   1.3&   0.2&   1.4&   0.0&  13.8&   3.3&  74.9&   8.0&   0.0&   0.0 \\ 
 487& 133156.918+135813.30&  0.1978&  30.2&  0.06&  0.00&  -0.8&  -0.1&   0.1&   0.4&   0.0&   9.5&   4.5&  86.0&   0.0&   0.0&   0.0 \\ 
 488& 133323.791+532130.14&  0.1023&  26.7&  0.27&  0.00&   0.9&   2.5&  -0.1&   2.2&   0.6&   7.5&   2.9&  23.6&   0.8&  54.7&   8.3 \\ 
 489& 133350.731-001617.68&  0.1764&  33.8&  0.30&  0.02&   2.2&   0.7&   0.6&   1.5&   0.0&  18.1&   3.5&  42.7&  15.1&  20.4&   0.1 \\ 
 490& 133418.110-003956.64&  0.2042&  23.4&  0.16&  0.02&   1.4&   1.4&   0.1&   1.8&   0.4&   0.8&   0.0&  64.2&  27.9&   0.0&   6.5 \\ 
 491& 133436.547+381944.50&  0.0621&   6.0&  0.63&  0.00&   0.7&   5.5&   0.4&   3.0&   0.1&  14.4&   0.4&   0.6&  84.1&   0.0&   0.0 \\ 
 492& 133552.598+452205.97&  0.1409&  24.2&  0.00&  0.00&   1.6&   1.5&   0.7&   0.8&   0.0&  11.6&   0.0&  87.0&   1.1&   0.0&   0.0 \\ 
 493& 133602.280+322040.00&  0.1787&  36.1&  0.24&  0.00&   1.4&   4.2&   1.2&   2.9&   1.2&   0.7&   4.4&  73.0&   0.0&  15.9&   0.0 \\ 
 494& 133638.748+193448.72&  0.1109&  11.7&  0.25&  0.00&   0.9&   1.4&   0.3&   1.4&   0.0&   5.6&   2.0&  65.0&  11.0&   1.7&  14.3 \\ 
 495& 133751.302+354755.79&  0.0727&  27.5&  0.49&  0.00&   1.0&   3.6&   0.4&   1.4&   0.0&  14.7&   3.2&  15.1&  53.5&  13.4&   0.1 \\ 
 496& 134041.933+175332.48&  0.1431&  16.8&  0.54&  0.00&   2.0&   1.5&   0.7&   1.7&   0.0&  21.0&   0.8&  78.2&   0.0&   0.0&   0.0 \\ 
 497& 134043.375+070428.37&  0.1469&  18.4&  0.29&  0.01&   1.4&   1.2&   0.6&   0.9&   0.0&   0.0&   0.0& 100.0&   0.0&   0.0&   0.0 \\ 
 498& 134249.519+541238.87&  0.2085&  23.0&  0.42&  0.00&   1.1&   2.0&   0.4&   2.3&   0.7&   4.1&   1.0&  81.0&   2.0&   0.0&   8.2 \\ 
 499& 134516.118+060637.42&  0.1261&  27.3&  0.25&  0.01&   1.1&   1.1&   0.4&  -0.6&   0.0&   5.3&   0.3&  54.5&   2.4&  21.7&  15.5 \\ 
 500& 134722.030+181719.27&  0.2359&  53.5&  0.01&  0.00&   3.6&   0.5&   0.7&   0.5&   0.1&   4.5&   0.0&  55.6&  29.0&  10.7&   0.0 \\ 
 501& 134738.066+174359.34&  0.1811&  25.7&  0.18&  0.00&   1.3&   1.4&   0.3&   1.8&   0.0&   5.9&   0.0&  94.1&   0.0&   0.0&   0.0 \\ 
 502& 134802.182+020405.73&  0.0678&  14.1&  0.23&  0.04&   1.1&   1.3&  -0.2&   1.4&   0.5&  16.4&   1.2&  14.2&  18.0&  40.2&   9.2 \\ 
 503& 134804.301+445032.45&  0.1314&   8.2&  0.40&  0.00&   0.9&   5.7&   1.4&   3.4&   1.9&  43.3&  17.7&  27.9&   4.1&   0.0&   0.0 \\ 
 504& 134809.684+623612.69&  0.1989&  35.7&  0.29&  0.05&   1.0&   1.1&   0.0&  -0.0&   0.0&   0.0&   0.0& 100.0&   0.0&   0.0&   0.0 \\ 
 505& 134822.870+174847.26&  0.0646&   2.9&  0.04&  0.00&   1.7&   0.7&   0.3&   1.0&   0.1&   5.6&   8.6&  31.5&  49.9&   3.8&   0.0 \\ 
 506& 134909.103+281956.65&  0.3051&  71.9&  0.05&  0.00&   0.9&   0.8&  -0.0&   0.6&   0.0&   5.6&   0.0&  86.1&   0.5&   7.4&   0.0 \\ 
 507& 134948.118+212237.80&  0.0956&   6.7&  0.19&  0.01&   0.7&   1.6&   1.7&   2.1&   0.0&  24.5&   7.9&  67.6&   0.0&   0.0&   0.0 \\ 
 508& 135005.585-024734.67&  0.1281&  43.4&  0.49&  0.09&   1.0&   1.9&   0.2&   2.7&   0.3&   6.9&  14.8&  25.6&   0.0&  10.4&  42.0 \\ 
 509& 135026.501+325615.66&  0.1564&  41.8&  0.36&  0.00&   1.0&   3.5&   0.0&   2.5&   0.0&  13.5&   0.0&  23.1&   0.0&  54.4&   8.7 \\ 
 510& 135030.766+012804.72&  0.0728&  17.4&  0.17&  0.03&   1.4&   2.8&   0.5&   2.2&   0.1&  14.4&   4.0&  19.4&  22.2&  39.2&   0.0 \\ 
 511& 135124.773+054903.13&  0.0832&  18.2&  0.01&  0.05&   1.3&   0.9&   0.2&   0.7&   0.0&  21.4&   0.0&  77.2&   0.0&   0.0&   0.0 \\ 
 512& 135505.537+124812.27&  0.2032&  43.7&  0.41&  0.00&   1.2&   3.7&   2.0&   1.7&   0.1&  12.0&   9.6&  38.0&  18.9&   0.0&  21.3 \\ 
 513& 135535.894+084915.55&  0.1188&  20.1&  0.36&  0.03&   1.1&   2.5&   0.2&   3.2&   0.6&   3.7&  17.1&  48.9&  14.1&  11.6&   2.6 \\ 
 514& 135556.333+093526.10&  0.0557&   4.9&  0.14&  0.03&   3.4&   0.5&   0.4&   1.1&   0.1&  11.1&   9.4&  23.6&  37.8&  17.7&   0.0 \\ 
 515& 135631.582-001608.21&  0.1632&  17.1&  0.12&  0.10&   2.5&   1.8&   0.2&   3.6&   0.0&   9.9&   1.4&  88.7&   0.0&   0.0&   0.0 \\ 
 516& 135737.553-022645.98&  0.1140&  19.8&  0.56&  0.13&   0.9&   4.3&   0.9&   4.7&   0.6&   2.4&   3.4&  68.7&   6.1&  17.4&   0.0 \\ 
 517& 135908.323+272445.96&  0.1906&  18.8&  0.39&  0.00&   1.4&   1.6&   0.4&   2.7&   0.1&   6.5&   7.6&  38.2&   9.6&  18.8&  11.3 \\ 
 518& 135914.218+123653.45&  0.1203&  15.8&  0.24&  0.00&   0.8&   1.8&   0.5&   0.9&   0.0&   5.4&   0.5&  27.8&  33.8&  32.1&   0.0 \\ 
 519& 135937.757+283925.97&  0.2260&  42.8&  0.32&  0.00&   1.2&   2.3&   0.5&   2.3&   0.2&  12.6&   5.2&  30.7&  27.3&  22.7&   0.0 \\ 
 520& 135949.865+540420.02&  0.3280& 250.3&  0.78&  0.00&   0.1&   0.4&   0.3&   0.1&   0.0&   0.0&   0.0&  27.5&   0.0&   0.0&  72.5 \\ 
 521& 140000.850+001518.57&  0.1455&  35.0&  0.71&  0.12&   0.9&   2.9&   0.3&   2.5&   0.0&   9.1&  10.1&  12.1&   9.8&   0.4&  58.3 \\ 
 522& 140004.891+300533.72&  0.1469&  35.6&  0.61&  0.00&   1.4&   2.3&   0.1&   2.0&   0.0&  24.1&   6.8&  11.8&  57.2&   0.0&   0.0 \\ 
 523& 140014.345+502324.97&  0.1503&  45.4&  0.14&  0.02&   1.1&   1.1&  -0.1&   0.5&   0.0&   2.8&   1.3&  49.8&   0.0&  32.9&  13.2 \\ 
 524& 140148.566+061534.60&  0.1246&  22.8&  0.12&  0.03&   2.0&   0.2&   0.1&   0.6&   0.0&   8.5&   0.8&  47.3&   1.4&  41.8&   0.0 \\ 
 525& 140247.854+530751.61&  0.1646&  31.2&  0.28&  0.00&   2.2&   1.6&   0.6&   2.5&   0.0&  16.4&  13.5&  32.9&  36.8&   0.0&   0.0 \\ 
 526& 140348.946+271843.24&  0.1660&  38.1&  0.44&  0.00&   0.4&   5.1&  -0.3&   2.1&   0.2&   7.7&   0.0&  14.5&  28.9&   4.8&  43.9 \\ 
 527& 140429.249+102225.92&  0.1020&   6.8&  0.14&  0.00&   0.9&   2.1&   1.4&   2.7&   0.4&  14.2&   4.8&  34.1&   8.9&  28.6&   6.1 \\ 
 528& 140436.542+171804.52&  0.1985&  45.8&  0.20&  0.00&   0.9&   3.9&   0.2&   0.7&   0.1&   4.4&   0.0&  63.5&   2.6&  29.4&   0.0 \\ 
 529& 140455.613+135246.81&  0.1636&  20.0&  0.17&  0.00&   0.6&   1.1&   1.0&   1.9&   0.0&  21.0&   0.6&  78.4&   0.0&   0.0&   0.0 \\ 
 530& 140529.830+110923.79&  0.2021& 103.7&  0.33&  0.00&   1.7&   1.2&   0.2&   0.7&   0.1&   0.6&   0.0&  23.7&  23.7&  35.4&  15.4 \\ 
 531& 140535.683+070143.27&  0.1389&  21.5&  0.20&  0.03&   1.3&   1.6&   0.3&   1.7&   0.7&   4.3&   1.1&  30.9&   0.0&  52.4&   8.3 \\ 
 532& 140634.150+372142.15&  0.2108&  94.5&  0.36&  0.00&   1.8&   0.8&  -0.2&   0.8&   0.0&   2.9&   0.7&  29.0&   2.2&  45.1&  19.7 \\ 
 533& 140635.978+084523.87&  0.0874&  10.9&  0.27&  0.06&   2.2&   1.3&   0.4&   0.5&   0.4&  19.1&   5.3&  55.4&  19.0&   0.0&   0.0 \\ 
 534& 140644.287+261906.64&  0.1361&  14.9&  0.19&  0.00&   1.2&   1.5&   1.3&   1.9&   0.1&   3.7&  26.8&  69.2&   0.1&   0.0&   0.0 \\ 
 535& 140656.482+124513.74&  0.0867&   5.7&  0.30&  0.00&   0.4&   2.7&   2.2&   4.0&   0.0&   0.0&   0.0&  37.9&  53.6&   8.4&   0.0 \\ 
 536& 140713.495+163403.29&  0.0871&  18.3&  0.30&  0.00&   1.9&   1.7&   0.2&   1.7&   0.1&   3.4&   0.7&  34.7&  39.2&   0.0&  21.7 \\ 
 537& 140728.121+262451.31&  0.0749&   7.3&  0.49&  0.00&   0.7&   1.8&  -0.1&   1.9&   0.0&   2.3&   0.0&  30.6&  67.1&   0.0&   0.0 \\ 
 538& 140801.615+514226.05&  0.1599&  60.0&  0.52&  0.01&   0.8&   3.8&  -0.0&   1.4&   0.1&   6.9&   1.3&  15.3&   5.0&  26.1&  44.4 \\ 
 539& 140845.458+135041.06&  0.1312&  32.3&  0.54&  0.00&   0.8&   2.1&   0.0&   2.4&   0.0&  13.3&   0.2&  21.4&  22.0&   4.0&  38.8 \\ 
 540& 140943.224-000036.88&  0.1350&  21.3&  0.16&  0.10&   1.8&   0.3&   0.1&   0.7&   0.1&   3.6&   0.2&  25.4&  38.9&  31.4&   0.0 \\ 
 541& 141003.672+603229.82&  0.1707&  67.7&  0.26&  0.01&   1.5&   2.2&  -0.1&   2.0&   0.1&   8.3&   0.9&  26.4&   8.8&  21.9&  32.1 \\ 
 542& 141104.169+400918.45&  0.1448&  34.0&  0.59&  0.00&   1.3&   4.4&   0.2&   3.5&   0.3&  11.0&   1.1&  25.3&  10.8&  15.0&  35.7 \\ 
 543& 141109.737+265051.37&  0.1302&  10.3&  0.18&  0.00&   1.1&   1.0&   0.5&   0.7&   0.0&  21.0&  15.2&  46.1&   9.0&   8.4&   0.0 \\ 
 544& 141117.014+205233.48&  0.1934&  28.2&  0.67&  0.02&   1.3&   3.1&   0.1&   2.4&   0.0&  40.6&  17.8&  22.6&  18.9&   0.0&   0.0 \\ 
 545& 141125.037+314551.35&  0.1969&  21.3&  0.23&  0.00&   1.5&   1.2&   0.0&   1.6&   0.0&   2.8&   0.0&  92.9&   2.5&   0.0&   0.0 \\ 
 546& 141126.856+614516.65&  0.1508&  40.7&  0.34&  0.04&   1.1&   5.2&   1.2&   3.1&   0.8&   0.0&   2.2&  45.6&   0.0&  14.5&  33.9 \\ 
 547& 141127.494+243809.54&  0.0542&  11.2&  0.09&  0.00&   0.8&   2.0&   0.2&   2.2&   0.7&   7.9&   2.0&  11.5&  29.4&  39.2&   7.7 \\ 
 548& 141143.166+450353.05&  0.0685&   4.5&  0.38&  0.00&   0.8&   2.9&   0.1&   3.4&   0.0&  12.1&   7.4&  12.3&  54.8&  12.8&   0.0 \\ 
 549& 141239.722+223509.83&  0.1484&  15.7&  0.03&  0.02&   1.8&   0.6&   0.4&   1.0&   0.2&  10.3&  11.3&  59.1&   0.1&  18.9&   0.0 \\ 
 550& 141241.962+261707.15&  0.1938&  31.4&  0.35&  0.00&   4.5&   0.5&   0.1&   0.8&   0.4&  30.0&  11.7&  49.5&   7.2&   1.1&   0.0 \\ 
 551& 141256.630+223125.38&  0.1569&  44.9&  0.83&  0.02&   1.8&   2.0&  -0.2&   1.9&   0.1&  18.7&   0.8&  11.0&  11.1&  11.3&  46.7 \\ 
 552& 141342.266+522809.97&  0.2407&  74.5&  0.36&  0.00&   1.4&   3.4&   1.3&   3.1&   0.0&  11.2&   0.1&  52.6&  35.7&   0.0&   0.0 \\ 
 553& 141419.296-031111.52&  0.0471&  38.7&  0.70&  0.12&   1.2&   2.6&  -0.0&   3.5&   0.0&   0.2&   0.3&   2.7&  50.7&  31.9&  14.2 \\ 
 554& 141505.167-023339.76&  0.1985&  34.1&  0.33&  0.14&   1.0&   3.6&   5.0&   3.4&   0.0&   3.4&   1.1&  58.2&  37.4&   0.0&   0.0 \\ 
 555& 141517.150+152139.00&  0.2623&  57.1&  0.28&  0.00&   0.1&   0.7&  -0.2&   0.2&   0.1&   0.7&   5.8&  69.2&   0.0&  21.5&   0.0 \\ 
 556& 141625.630+340050.20&  0.1698&  22.7&  0.29&  0.00&   1.0&   1.8&  -0.3&   0.7&   0.4&   5.4&   5.5&  36.0&  33.7&  16.2&   0.0 \\ 
 557& 141626.558+252125.29&  0.1434&  25.7&  0.54&  0.00&   1.8&   1.2&   0.2&   1.8&   0.2&  19.1&   8.4&  31.9&   5.5&  17.7&  15.8 \\ 
 558& 141728.728+602113.88&  0.0691&   7.2&  0.12&  0.00&   1.6&   4.4&   2.0&   0.4&   5.6&   0.8&   0.0&  21.7&   4.7&  66.7&   0.0 \\ 
 559& 141808.993+401245.52&  0.1721&  36.1&  0.12&  0.00&   1.2&   0.7&   0.5&   0.8&   0.0&  11.8&   0.0&  71.5&   0.0&  16.4&   0.0 \\ 
 560& 141854.103+050547.48&  0.0795&  56.9&  1.40&  0.04&   0.8&   4.1&  -0.6&   2.4&   0.0&   4.7&   0.6&   0.0&  49.9&  17.9&  26.6 \\ 
 561& 141854.149+272738.29&  0.1418&  34.4&  0.49&  0.00&   1.5&   1.8&   0.5&   1.9&   0.0&   8.2&   1.2&  27.4&   0.0&  49.7&  13.1 \\ 
 562& 141950.878+312620.57&  0.1194&  14.9&  0.20&  0.00&   1.4&   1.3&   0.3&   1.3&   0.0&   0.5&   7.7&  71.9&   7.9&  11.8&   0.0 \\ 
 563& 142026.890+063550.99&  0.2292&  37.9&  0.75&  0.04&   1.2&   2.7&  -0.0&   2.8&   0.0&  44.8&   4.9&  44.1&   5.8&   0.0&   0.4 \\ 
 564& 142112.278+543023.69&  0.0861&   6.4&  0.05&  0.00&   0.9&   1.0&   0.3&   2.8&   0.0&   4.4&  21.3&  16.5&  50.0&   0.3&   7.4 \\ 
 565& 142257.727+225441.43&  0.0325&   0.3&  0.24&  0.05&   0.2&   4.0&   0.5&   1.9&  39.5&  25.1&   9.5&   0.0&   0.0&   0.0&   0.0 \\ 
 566& 142355.627+390732.82&  0.0975&   6.7&  0.18&  0.00&   1.1&   2.6&   0.8&   3.2&   0.0&  21.4&   0.7&  77.8&   0.0&   0.0&   0.0 \\ 
 567& 142455.692+264438.98&  0.2310&  60.4&  0.13&  0.00&   1.0&   1.1&   0.1&   0.7&   0.0&   0.7&   0.0&  46.9&  20.1&  32.2&   0.0 \\ 
 568& 142658.445+421615.53&  0.3455&  37.5&  0.20&  0.00&   2.2&   1.5&   0.8&   2.2&   0.0&   8.2&   0.0&  81.8&   9.9&   0.0&   0.0 \\ 
 569& 142736.686+430202.29&  0.0971&  13.2&  0.26&  0.01&   1.4&   1.5&  -0.3&   2.1&   0.4&   2.3&   0.0&  17.2&  49.2&  30.0&   0.0 \\ 
 570& 142808.419+062545.01&  0.1736&  51.3&  0.45&  0.01&   1.0&   1.8&   0.2&   2.1&   0.0&  11.8&   0.0&  88.2&   0.0&   0.0&   0.0 \\ 
 571& 142848.228+274149.66&  0.1099&  12.5&  0.10&  0.00&   0.7&   0.1&   0.2&   0.5&   0.1&   5.4&  20.5&  74.0&   0.0&   0.0&   0.0 \\ 
 572& 142926.477+552945.85&  0.1566&  31.2&  0.22&  0.00&   1.0&   1.9&  -0.0&   1.2&   0.2&  10.0&   0.4&  58.4&   0.0&  27.9&   0.0 \\ 
 573& 143055.824+000451.33&  0.1188&  10.9&  0.25&  0.09&   0.8&   1.1&   0.5&  -0.2&   0.0&  22.7&   0.0&  77.3&   0.0&   0.0&   0.0 \\ 
 574& 143057.521-013939.64&  0.0927&   7.5&  0.23&  0.10&   2.0&   1.1&  -0.2&   1.4&   0.0&   5.8&   0.6&  86.7&   6.8&   0.0&   0.0 \\ 
 575& 143101.510+580443.22&  0.2148&  59.1&  0.58&  0.01&   0.9&   0.7&   0.3&   0.4&   0.0&   8.5&   8.3&  39.5&   5.8&  36.3&   0.0 \\ 
 576& 143137.968+021942.27&  0.0654&   3.8&  0.31&  0.07&   0.2&   2.0&   1.3&   3.3&   0.5&  16.8&   0.6&  12.1&  47.2&   0.0&  22.3 \\ 
 577& 143140.270+030154.09&  0.1528&  21.1&  0.18&  0.05&   1.0&   1.0&   0.3&   1.3&   0.0&   3.6&  20.1&  40.4&   1.1&  22.8&  11.3 \\ 
 578& 143146.399+341719.01&  0.1235&  28.2&  0.39&  0.00&   2.0&   1.6&   0.1&   1.2&   0.0&  21.0&   1.0&  46.1&   2.0&  28.2&   0.0 \\ 
 579& 143224.026+512428.59&  0.2313&  48.7&  0.82&  0.00&   0.7&   3.6&  -0.2&   1.9&   0.0&   8.1&   2.5&  80.1&   7.2&   2.0&   0.0 \\ 
 580& 143241.832+374054.27&  0.1290&  23.7&  0.19&  0.00&   0.8&   0.7&   0.3&   1.0&   0.0&   9.0&   2.4&  63.8&  24.8&   0.0&   0.0 \\ 
 581& 143300.154+055525.45&  0.1565&  42.6&  0.08&  0.04&   4.9&   0.3&  -0.1&   0.3&   0.2&  11.8&   0.2&  24.7&   0.0&  53.5&   8.9 \\ 
 582& 143326.743+114728.86&  0.1579&  42.7&  0.33&  0.02&   2.0&   0.7&   0.3&   1.0&   0.0&   5.1&   0.4&  43.1&   3.0&   9.4&  38.7 \\ 
 583& 143347.899+230748.14&  0.1701&  69.7&  0.08&  0.08&   2.0&   0.5&  -0.3&   1.0&   0.1&  11.0&   1.2&  19.9&   6.1&  39.8&  21.9 \\ 
 584& 143350.006+233407.82&  0.1662&  95.4&  0.35&  0.08&   1.0&   3.3&   0.2&   2.2&   0.4&   2.2&   1.6&   2.3&  11.8&  25.0&  54.2 \\ 
 585& 143414.026+030140.28&  0.3019&  81.5&  0.32&  0.05&   1.7&   1.4&   0.3&   1.7&   0.0&   6.8&   1.3&  59.2&   4.8&  27.8&   0.0 \\ 
 586& 143454.804+080306.39&  0.2072&  41.3&  0.26&  0.01&   1.2&   1.6&   0.1&   0.9&   0.0&   6.4&   1.2&  44.6&   5.5&  40.2&   0.0 \\ 
 587& 143553.215+184719.78&  0.0458&   1.9&  0.00&  0.04&   0.8&   2.7&   1.1&   2.8&   0.2&  16.0&   8.8&  17.8&  46.4&  10.2&   0.0 \\ 
 588& 143614.866+334940.87&  0.0976&   9.6&  0.28&  0.00&   1.5&   0.8&   0.7&   1.1&   0.0&  19.7&   2.2&  31.8&  38.4&   7.9&   0.0 \\ 
 589& 143635.635+443351.52&  0.0893&  25.6&  0.14&  0.02&   5.5&   0.1&   0.3&   0.2&   0.1&  10.1&   2.5&  22.9&  23.3&  21.3&  19.7 \\ 
 590& 143827.098+144116.81&  0.1936&  29.1&  0.17&  0.00&   3.4&   0.5&   0.3&   0.7&   0.0&   5.5&   1.0&  93.5&   0.0&   0.0&   0.0 \\ 
 591& 143841.184+001025.26&  0.1051&  11.9&  0.14&  0.10&   2.1&   1.3&   0.5&   2.4&   0.2&   0.6&   6.1&  55.2&   7.9&   1.4&  27.9 \\ 
 592& 143854.007+253454.57&  0.0918&  11.9&  0.42&  0.03&   0.7&   2.3&   1.6&   2.6&   0.0&   0.0&   0.0&  18.8&  17.7&  63.1&   0.4 \\ 
 593& 144006.192+170020.17&  0.1070&  11.6&  0.39&  0.01&   1.6&   1.5&   0.4&   2.3&   0.3&  11.5&  20.0&  27.6&   7.4&   0.2&  32.9 \\ 
 594& 144021.259+034612.81&  0.0265&   0.2&  0.13&  0.07&   7.0&   0.1&  -0.3&   4.9&   0.3&  43.8&   1.2&  18.5&  35.3&   0.1&   0.0 \\ 
 595& 144058.145+124855.41&  0.1776&  24.4&  0.17&  0.00&   1.8&   0.4&  -0.2&   0.2&   0.0&  23.8&   0.1&  43.5&   5.8&  26.5&   0.0 \\ 
 596& 144108.110+120255.07&  0.2364&  86.6&  0.34&  0.01&   1.0&   2.4&   0.5&   2.0&   0.0&   0.9&   0.3&  31.6&   1.5&  23.6&  39.9 \\ 
 597& 144157.809+243649.25&  0.0413&   3.7&  0.56&  0.08&   1.2&   1.8&   0.5&   3.4&   0.1&   5.3&   5.4&  14.0&  50.6&   4.3&  20.2 \\ 
 598& 144200.211+495449.11&  0.1988&  87.5&  0.25&  0.05&   0.6&   1.4&   0.3&   1.1&   0.0&   0.9&   0.5&  36.8&   0.0&  61.5&   0.0 \\ 
 599& 144205.254+515153.25&  0.0891&  31.3&  0.99&  0.02&   0.5&   2.3&   1.0&   0.8&   0.0&   0.1&   0.2&   8.0&  33.0&  33.5&  25.2 \\ 
 600& 144206.475+254725.94&  0.2435& 126.9&  0.17&  0.04&   4.4&   0.3&  -0.1&  -0.4&   0.0&   1.9&   2.9&  13.8&  17.0&  61.1&   2.8 \\ 
 601& 144220.342+181900.04&  0.0878&  14.3&  0.32&  0.04&   1.9&   1.7&   0.8&   0.7&   0.0&   2.2&   1.8&  44.3&  51.7&   0.0&   0.0 \\ 
 602& 144229.851+222014.97&  0.0978&   5.1&  0.22&  0.07&   0.8&   0.8&  -0.1&   2.1&   0.5&  19.2&   7.1&  22.0&  24.5&  11.1&  13.6 \\ 
 603& 144315.468+115224.06&  0.1294&  39.8&  0.19&  0.01&   1.9&   1.6&   0.5&   0.9&   0.0&   0.7&   0.2&  44.3&  12.1&  32.5&   9.7 \\ 
 604& 144400.794+211850.53&  0.1878&  31.8&  0.11&  0.03&   0.9&   1.4&   0.1&  -0.0&   0.1&  11.1&   0.8&  33.9&  16.1&  31.3&   4.2 \\ 
 605& 144436.895+264137.41&  0.0900&   7.4&  0.20&  0.04&   1.1&   1.6&   0.6&   1.7&   0.0&  20.3&   2.9&  69.0&   7.7&   0.0&   0.0 \\ 
 606& 144446.735+635042.71&  0.1153&  15.3&  0.12&  0.02&   1.2&   1.5&   1.0&   3.1&   0.2&  12.5&   2.6&  18.6&  18.2&   0.0&  47.6 \\ 
 607& 144539.480+553651.07&  0.2896&  67.0&  0.00&  0.01&   1.3&   2.3&   0.2&   2.1&   0.0&   1.6&   0.0&  47.3&   0.0&  40.1&  10.1 \\ 
 608& 144721.562+051352.34&  0.1630&  33.5&  0.07&  0.13&   1.3&   0.6&   0.6&   0.3&   0.3&   5.8&   0.1&  93.7&   0.0&   0.0&   0.0 \\ 
 609& 144752.466+324111.73&  0.0984&   8.5&  0.12&  0.02&   0.7&   1.5&   0.7&   0.5&   0.0&   9.7&   1.2&  64.8&  17.3&   7.0&   0.0 \\ 
 610& 144816.049+173305.94&  0.0450&   8.9&  1.02&  0.04&   1.8&   2.4&  -0.3&   2.2&   0.1&   3.8&   0.5&   0.0&  63.9&  17.6&  13.9 \\ 
 611& 144854.276+313929.01&  0.0633&  11.6&  0.50&  0.00&   1.9&   1.7&   0.7&   1.2&   0.0&  10.9&   2.4&  48.5&  38.0&   0.1&   0.0 \\ 
 612& 145009.391+181937.35&  0.0791&   6.8&  0.27&  0.05&   1.4&   2.7&   0.5&   2.4&   0.0&   9.6&   2.5&  52.2&  35.7&   0.0&   0.0 \\ 
 613& 145035.138+162223.59&  0.2228&  28.8&  0.16&  0.00&   2.4&   0.5&   0.1&   1.5&   0.0&   6.7&   0.0&  93.3&   0.0&   0.0&   0.0 \\ 
 614& 145105.630+180735.43&  0.1213&   9.1&  0.30&  0.03&   1.9&   2.1&   1.9&   2.1&   0.1&   4.1&  15.8&  76.6&   3.3&   0.0&   0.0 \\ 
 615& 145119.735+395353.65&  0.2459&  96.2&  0.45&  0.00&   1.7&   2.0&   0.6&   0.4&   0.1&   2.3&   0.3&  26.0&  11.2&  19.2&  40.0 \\ 
 616& 145133.857+022658.62&  0.0969&   7.6&  0.04&  0.13&   1.0&   1.6&   0.5&   1.2&   0.0&  16.7&   3.6&  79.7&   0.0&   0.0&   0.0 \\ 
 617& 145208.652+165805.27&  0.0459&   2.9&  0.65&  0.03&   0.5&   3.4&  -0.8&   4.6&   0.1&   2.3&   0.0&   4.9&  33.9&  47.3&  11.5 \\ 
 618& 145220.189+154927.80&  0.1635&  41.2&  0.73&  0.02&   1.5&   1.6&   0.3&   1.9&   0.0&  14.5&   0.8&  32.6&   0.0&  10.4&  41.8 \\ 
 619& 145237.118+082226.86&  0.2779& 198.6&  0.48&  0.06&   0.8&   3.9&   0.4&   1.5&   0.4&   1.9&   1.8&  11.7&   4.0&  13.3&  65.8 \\ 
 620& 145245.468+025321.34&  0.2644&  45.5&  0.41&  0.13&   3.5&   0.4&   0.3&   1.1&   0.0&   7.4&   0.0&  92.6&   0.0&   0.0&   0.0 \\ 
 621& 145408.638+201241.79&  0.1767&  89.5&  0.38&  0.03&   1.5&   3.7&  -0.2&   3.5&   0.2&   5.7&   0.3&   5.9&   4.9&  42.5&  39.8 \\ 
 622& 145428.925+231936.44&  0.1654&  53.0&  0.52&  0.05&   0.7&   5.2&   0.1&   1.7&   0.1&  13.3&   0.0&  27.2&   0.0&  29.1&  29.9 \\ 
 623& 145440.678+203834.87&  0.1855&  54.7&  0.31&  0.06&   1.3&   4.6&   1.6&   3.6&   0.2&   9.1&   0.7&  20.1&   4.2&   0.0&  64.9 \\ 
 624& 145455.445+453126.60&  0.0366&   6.6&  0.10&  0.03&   1.2&   1.6&  -0.1&   0.1&   0.1&   6.4&   0.9&  22.9&  16.1&  50.6&   2.5 \\ 
 625& 145505.446+131651.64&  0.0827&  31.4&  0.62&  0.03&   1.5&   1.8&   0.2&   2.4&   0.0&   5.7&   1.3&  12.5&  66.9&   4.6&   8.8 \\ 
 626& 145511.364+190420.42&  0.0586&   2.7&  0.33&  0.06& -13.2&  -0.0&  -0.2&   1.8&   0.1&   4.3&   0.0&   7.9&  35.3&  52.4&   0.0 \\ 
 627& 145555.006+622307.12&  0.1470&  28.1&  0.59&  0.00&   1.6&   3.7&   1.4&   3.4&   0.3&   6.2&   2.3&  40.6&  36.5&   0.0&  13.6 \\ 
 628& 145934.022+371953.81&  0.2021&  50.0&  0.47&  0.03&   1.4&   1.5&  -0.2&   2.4&   0.0&  18.9&   2.1&  19.7&   8.8&   0.0&  49.9 \\ 
 629& 145939.811+021804.20&  0.0425&   0.8&  0.00&  0.12&   0.9&   1.6&   1.0&   0.7&   0.0&  43.8&   0.5&   6.3&  49.4&   0.0&   0.0 \\ 
 630& 150522.258+072334.96&  0.1198&  12.7&  0.30&  0.07&   2.5&   0.6&   0.3&   0.0&   0.0&  22.7&   0.0&  77.3&   0.0&   0.0&   0.0 \\ 
 631& 150546.274+245406.85&  0.3258& 103.0&  0.16&  0.11&   1.0&   1.0&   0.0&  -0.0&   0.1&   2.0&  10.1&  22.1&  26.9&  28.8&  10.0 \\ 
 632& 150604.202+300229.13&  0.2351& 119.7&  0.21&  0.02&   0.9&   1.1&  -0.1&   1.4&   0.0&   0.9&   1.2&  24.0&   0.0&  73.7&   0.0 \\ 
 633& 150635.563+321035.77&  0.1159&  20.7&  0.25&  0.03&   2.5&   0.4&   0.4&  -0.1&   0.3&   8.4&   8.5&  41.4&   0.0&   3.9&  36.7 \\ 
 634& 150724.302+413556.51&  0.2075&  53.7&  0.07&  0.03&   2.5&   0.7&   0.1&   0.1&   0.0&   2.9&   0.0&  70.3&   0.0&  26.4&   0.0 \\ 
 635& 150926.474+152132.04&  0.2022& 110.7&  0.17&  0.04&   1.9&   1.1&  -0.2&   0.8&   0.0&   1.9&   0.2&  16.1&   1.7&  42.9&  36.5 \\ 
 636& 151010.680+182242.74&  0.1497&  41.0&  0.59&  0.06&   0.9&   3.2&   0.3&   0.4&   0.2&   5.1&   1.7&  20.4&  24.4&  25.1&  22.6 \\ 
 637& 151025.534+092459.09&  0.1161&  24.6&  0.52&  0.05&   1.8&   1.1&   0.3&   0.4&   0.0&  12.3&   3.5&  84.2&   0.0&   0.0&   0.0 \\ 
 638& 151052.826+095534.44&  0.2029&  54.1&  0.55&  0.07&   1.3&   3.6&   0.3&   2.4&   0.0&  26.8&   0.0&  73.2&   0.0&   0.0&   0.0 \\ 
 639& 151105.964+550605.28&  0.3353&  40.7&  0.32&  0.01&   1.2&   3.2&   0.1&   1.7&   0.2&   5.7&  12.1&   2.9&   0.0&  67.0&   0.0 \\ 
 640& 151111.402+054027.02&  0.0684&   6.4&  0.23&  0.08&   1.0&   1.0&  -0.2&   2.0&   0.2&   8.5&   2.2&  18.0&  49.9&  14.4&   6.9 \\ 
 641& 151151.362+230903.77&  0.0521&  77.4&  0.39&  0.12&   1.3&   3.9&  -0.2&   2.3&   0.5&   0.6&   0.4&   0.0&  24.1&  13.9&  59.8 \\ 
 642& 151248.146+160001.69&  0.0975&   7.1&  0.36&  0.04&   0.6&   5.0&  -0.1&   0.1&   0.0&  17.0&   5.5&  11.2&  52.2&   0.0&  14.0 \\ 
 643& 151354.677+553302.44&  0.2261& 100.2&  0.25&  0.01&   1.9&   2.1&   0.6&   1.2&   0.0&   1.9&   1.1&  24.6&  20.2&  25.3&  26.9 \\ 
 644& 151433.674+025728.23&  0.1275&  23.1&  0.27&  0.06&   2.0&   1.4&   0.2&   1.3&   0.0&   1.9&   0.8&  97.0&   0.0&   0.0&   0.0 \\ 
 645& 151528.812+325813.42&  0.1002&  11.9&  0.17&  0.03&   2.6&   0.9&   0.6&   1.3&   0.0&   6.0&   7.1&  56.9&   0.0&  14.8&  14.8 \\ 
 646& 151550.506+060114.31&  0.1041&   4.8&  0.00&  0.07&   1.9&   1.8&   0.6&   1.2&   0.1&  17.9&  13.3&  68.5&   0.0&   0.1&   0.0 \\ 
 647& 151552.030+312322.50&  0.0719&   6.3&  0.13&  0.03&   1.4&   0.9&   0.6&  -0.4&   0.0&  18.3&   6.1&  42.2&  16.3&  16.7&   0.0 \\ 
 648& 151711.479+265804.35&  0.0719&   3.4&  0.15&  0.07&   1.2&   1.6&   0.8&   1.3&   0.0&   6.7&   0.0&  32.1&  61.2&   0.0&   0.0 \\ 
 649& 151742.415+484843.65&  0.0619&   8.1&  0.27&  0.03&   0.7&   4.1&   0.8&   3.2&   0.0&   6.6&   0.4&   2.6&  63.0&  11.6&  15.7 \\ 
 650& 151743.608+284654.25&  0.1722&  19.1&  0.28&  0.04&   1.3&   1.3&   0.6&   0.9&   0.2&   0.8&   0.0&  70.3&  22.6&   5.4&   0.0 \\ 
 651& 151845.850+233536.81&  0.2474&  39.6&  0.25&  0.15&   1.0&   0.9&   0.5&   0.4&   0.0&   1.1&   0.4&  97.8&   0.0&   0.1&   0.0 \\ 
 652& 151915.545+162415.88&  0.1514&  54.2&  0.35&  0.07&   0.7&   5.0&   0.1&   1.9&   0.8&   6.2&   3.4&  34.0&   0.0&  46.6&   6.3 \\ 
 653& 152038.333+215254.26&  0.0943&  13.1&  0.13&  0.18&   1.8&   1.1&   0.4&   2.3&   0.0&   1.7&   3.8&  34.0&  48.2&   7.8&   4.3 \\ 
 654& 152057.010+371520.39&  0.1573&  17.7&  0.22&  0.03&   1.3&   1.6&   0.4&   1.3&   0.0&  14.5&  16.2&  53.9&   0.0&   0.0&   0.0 \\ 
 655& 152058.913+421254.39&  0.1075&   7.2&  0.07&  0.03&   1.6&   1.1&   0.4&   1.2&   0.0&  13.9&  10.2&  75.9&   0.0&   0.0&   0.0 \\ 
 656& 152139.418+205923.22&  0.2466& 120.6&  0.46&  0.17&   0.7&   2.2&   0.7&   0.3&   0.0&   7.9&   0.5&  30.3&   0.0&   3.9&  57.3 \\ 
 657& 152159.186+021022.45&  0.0794&  18.7&  0.96&  0.10&   0.7&   5.4&   0.9&   4.2&   0.2&  13.0&   0.0&   0.1&  31.5&  12.5&  42.2 \\ 
 658& 152236.773-015035.89&  0.0916&   6.7&  0.08&  0.30&   3.2&   0.1&  -0.2&   0.9&   0.1&   3.4&   7.8&  50.6&   1.9&  36.2&   0.0 \\ 
 659& 152321.888+140922.96&  0.1745&  29.7&  0.18&  0.13&   1.3&   1.5&   0.3&   2.9&   0.2&   9.0&  15.9&  64.8&   8.0&   1.6&   0.0 \\ 
 660& 152351.432+084734.68&  0.0398&   0.6&  0.33&  0.06&   0.4&   4.0&   0.6&   2.8&   0.2&  24.1&   1.7&  22.5&  51.4&   0.0&   0.0 \\ 
 661& 152419.411+054415.06&  0.1296&   9.2&  0.36&  0.07&   2.4&   1.1&  -0.1&   1.0&   0.1&   2.7&   0.0&  90.3&   0.0&   0.0&   0.0 \\ 
 662& 152426.506+080908.04&  0.0876&  71.3&  0.54&  0.10&   2.2&   3.3&   0.6&   2.2&   0.7&   2.9&   5.8&   1.9&  54.5&  10.3&  19.7 \\ 
 663& 152507.925+213353.71&  0.0811&   5.1&  0.23&  0.17&   0.5&   3.3&   1.0&   1.9&   0.0&   3.4&  14.6&  27.1&  13.5&  41.4&   0.0 \\ 
 664& 152541.561+260225.17&  0.1881&  45.2&  0.49&  0.14&   1.5&   1.4&  -0.2&   0.6&   0.2&  14.9&   4.5&  35.4&   4.1&   0.0&  40.1 \\ 
 665& 152633.046+064053.43&  0.0357&   2.5&  0.14&  0.05&   1.1&   1.8&   1.8&   2.8&   0.4&   5.4&   8.0&  35.8&  12.9&  35.6&   1.7 \\ 
 666& 152847.789+032321.28&  0.2997& 232.4&  0.26&  0.10&   1.2&   1.3&   0.0&   0.9&   0.0&   2.0&   0.9&  13.8&  21.5&  36.8&  25.0 \\ 
 667& 152859.100+245646.77&  0.1537&  29.6&  0.20&  0.15&   0.9&   0.7&   0.3&  -0.9&   0.0&   7.3&   0.0&  39.8&   0.4&  35.0&  16.9 \\ 
 668& 152906.422+543337.66&  0.2214&  24.2&  0.10&  0.04&   1.6&   0.8&   0.1&   0.2&   0.0&  24.3&   0.0&  75.3&   0.0&   0.0&   0.0 \\ 
 669& 152929.902+271205.43&  0.0729&  23.3&  0.64&  0.12&   1.2&   3.5&   0.6&   1.6&   0.4&   7.8&   2.2&   4.1&  10.8&  12.4&  60.9 \\ 
 670& 153004.238+413203.25&  0.2148&  26.2&  0.16&  0.07&   0.9&   1.1&   0.3&   0.8&   0.0&  21.3&   0.0&  78.2&   0.0&   0.0&   0.0 \\ 
 671& 153016.063+373346.16&  0.0774&  12.6&  0.27&  0.05&   1.2&   6.3&   3.6&   2.4&   1.3&  14.3&   4.6&  77.1&   0.0&   0.0&   0.0 \\ 
 672& 153057.062+304324.72&  0.3787&  56.4&  0.13&  0.07&   0.6&   2.5&   1.1&   2.9&   0.2&   3.2&   0.0&  59.0&  14.2&   0.0&  23.4 \\ 
 673& 153144.602+064304.27&  0.1058&  19.3&  0.88&  0.10&   2.3&   1.9&   1.1&   0.6&   0.0&  41.7&   9.5&  48.7&   0.0&   0.0&   0.0 \\ 
 674& 153344.952+121557.16&  0.1825&  43.2&  0.30&  0.10&   2.0&   1.8&  -0.3&   1.2&   0.7&   1.6&   0.4&  16.0&   1.0&  38.3&  39.8 \\ 
 675& 153426.004+173747.13&  0.0587&  24.8&  0.09&  0.12&   0.7&   4.7&   0.3&   0.6&   1.1&   2.7&   4.7&   2.0&   2.1&  49.3&  37.6 \\ 
 676& 153507.114+202743.09&  0.1839&  71.5&  0.59&  0.18&   0.9&   5.3&   1.6&   2.0&   0.3&   0.7&   0.5&  20.6&   0.0&  12.7&  63.6 \\ 
 677& 153534.061+123410.18&  0.1108&  20.2&  0.27&  0.10&   1.7&   1.5&   0.3&   1.7&   0.0&  29.4&   1.2&  69.4&   0.0&   0.0&   0.0 \\ 
 678& 153703.367+135944.15&  0.0737&  33.0&  0.32&  0.12&   1.6&   4.1&   2.2&   2.1&   0.3&   2.8&  11.9&   7.9&  76.7&   0.0&   0.0 \\ 
 679& 153724.245-015317.93&  0.1533&  16.5&  0.26&  0.37&   2.1&   2.9&   0.1&   3.0&   0.0&  25.3&   7.2&  66.4&   0.0&   0.0&   0.0 \\ 
 680& 153852.301+253945.69&  0.2699&  60.4&  0.05&  0.16&   0.5&   0.5&   0.0&   0.3&   0.0&  16.0&   0.5&  83.6&   0.0&   0.0&   0.0 \\ 
 681& 153854.842+171259.05&  0.1317&  77.3&  0.73&  0.08&   1.3&   3.6&   0.1&   1.8&   0.1&   6.7&   4.2&   9.8&  32.4&   2.3&  44.1 \\ 
 682& 154012.458+072841.27&  0.1794& 106.5&  0.33&  0.09&   0.7&   1.0&  -0.3&   1.1&   0.2&   1.1&   0.7&  18.3&   7.1&  61.7&  10.3 \\ 
 683& 154128.740-014346.89&  0.1052&  12.6&  0.61&  0.35&   2.5&   1.9&   1.0&   2.1&   0.0&  20.7&   5.3&  74.0&   0.0&   0.0&   0.0 \\ 
 684& 154224.125+234053.94&  0.2956& 121.2&  0.37&  0.15&   1.2&   1.8&   0.2&   1.8&   0.0&   1.9&   0.1&  43.1&  24.1&   0.0&  30.6 \\ 
 685& 154228.282+431538.39&  0.1502&  31.7&  0.28&  0.06&   1.0&   5.3&   0.7&   2.4&   2.2&  10.2&   1.3&  39.9&   0.0&  29.6&  16.2 \\ 
 686& 154234.522+211120.67&  0.1341&  10.0&  0.04&  0.15&   1.3&   1.0&   1.2&   1.6&   0.0&   0.0&   0.0& 100.0&   0.0&   0.0&   0.0 \\ 
 687& 154322.404+331018.62&  0.1266&  22.0&  0.33&  0.06&   1.4&   1.9&   0.9&   2.4&   0.0&   5.6&   6.8&  29.6&  55.0&   0.0&   3.0 \\ 
 688& 154401.810+180805.27&  0.2283&  99.9&  0.11&  0.07&   1.0&   0.7&  -0.1&   0.6&   0.0&   0.8&   0.2&  21.0&  23.7&  45.6&   7.7 \\ 
 689& 154518.526+354220.10&  0.0686&   2.9&  0.40&  0.04&   0.7&   3.3&   0.5&   0.7&   0.0&  18.0&   0.0&  12.7&  60.8&   8.4&   0.0 \\ 
 690& 154520.782+345251.07&  0.2327&  42.6&  0.39&  0.06&   1.1&   1.6&  -0.1&   1.4&   0.1&  15.7&   0.0&  84.0&   0.0&   0.0&   0.0 \\ 
 691& 154715.816+443343.11&  0.0621&   3.3&  0.17&  0.04&   1.6&   0.7&   0.7&   3.0&   0.1&  22.3&   7.3&  33.9&  36.2&   0.0&   0.0 \\ 
 692& 154733.650+051753.28&  0.1967&  44.1&  0.36&  0.11&   1.5&   2.5&   0.6&   1.4&   0.4&   1.2&  12.4&  11.2&   2.9&   9.6&  56.2 \\ 
 693& 154806.173+142227.12&  0.0355&   0.7&  0.14&  0.05&   0.9&   1.7&   0.6&   0.4&   0.1&  24.1&   1.5&  23.6&  45.5&   4.6&   0.0 \\ 
 694& 154810.771+191229.34&  0.0999&   8.6&  0.04&  0.10&   2.2&   0.4&   0.6&  -1.3&   0.0&  29.0&   0.2&  70.8&   0.0&   0.0&   0.0 \\ 
 695& 154859.695+105950.90&  0.0721&   5.5&  0.29&  0.14&   0.8&   2.4&   0.5&   1.0&   0.0&  32.6&   0.1&  49.6&  17.7&   0.0&   0.0 \\ 
 696& 154917.702+470505.04&  0.1563&  38.2&  0.42&  0.07&   1.4&   0.7&  -0.3&   0.2&   0.0&   9.6&   0.1&  34.3&  13.7&   0.0&  41.9 \\ 
 697& 154919.351+572321.03&  0.2252&  39.4&  0.00&  0.00&   1.0&   1.5&   0.6&   0.5&   0.0&   9.8&   9.3&  80.3&   0.0&   0.0&   0.0 \\ 
 698& 154944.938+133437.51&  0.1897&  70.4&  0.03&  0.10&   4.5&   0.4&   0.2&   0.2&   0.0&   1.2&   0.5&  17.0&   7.6&  58.1&  15.2 \\ 
 699& 155004.610+303502.54&  0.1913&  31.8&  0.30&  0.08&   1.2&   2.8&   0.9&   3.5&   0.5&  12.1&   6.1&  15.0&   3.6&  42.1&  20.0 \\ 
 700& 155016.526+194923.99&  0.1478&  31.4&  0.17&  0.10&   1.4&   1.9&   0.7&   1.8&   0.0&   0.5&   1.1&  52.5&   0.0&  38.3&   7.4 \\ 
 701& 155054.050+422540.42&  0.0969&   9.7&  0.27&  0.07&   0.2&   0.6&   1.1&   2.2&   0.0&  23.1&   4.8&  42.3&  29.7&   0.0&   0.0 \\ 
 702& 155125.817+135031.73&  0.1680&  22.3&  0.25&  0.10&   1.1&   1.8&   0.5&   2.6&   0.0&  26.5&   0.0&  61.2&  11.3&   0.0&   0.8 \\ 
 703& 155159.849+004444.29&  0.1475&  26.6&  0.38&  0.33&   0.7&   4.5&  -0.1&   3.0&   0.0&   0.1&   0.0&  37.3&   6.3&  32.0&  24.3 \\ 
 704& 155353.419+141534.45&  0.1039&  18.1&  0.22&  0.11&   0.9&   0.4&   0.3&  -0.3&   0.0&   0.0&   3.4&  96.6&   0.0&   0.0&   0.0 \\ 
 705& 155406.770+444130.14&  0.1078&  18.9&  0.25&  0.07&   4.0&   0.3&   0.1&   0.8&   0.0&   8.6&   2.8&  26.8&  15.0&  23.9&  22.7 \\ 
 706& 155435.539+291319.92&  0.0943&  36.1&  0.33&  0.10&   2.4&   1.0&   0.0&   1.5&   0.1&  15.1&   4.0&  35.5&   0.1&  31.7&  13.2 \\ 
 707& 155523.753+023932.98&  0.2029&  54.5&  0.07&  0.28&   4.8&   0.4&   1.1&   0.5&   0.5&   5.9&   2.5&  14.3&  30.9&  22.9&  23.0 \\ 
 708& 155545.110+082439.95&  0.1029&  17.8&  0.37&  0.10&   1.3&   1.9&   0.4&   3.0&   0.0&   5.0&   0.2&  33.3&  37.6&  13.4&  10.2 \\ 
 709& 155555.582+214431.80&  0.0709&  14.0&  1.04&  0.11&   1.3&   4.3&   1.3&   3.1&   0.0&   0.0&   0.0&  23.1&  76.9&   0.0&   0.0 \\ 
 710& 155650.011+165925.23&  0.2321&  84.2&  0.40&  0.05&   1.3&   3.4&   0.3&   3.4&   0.7&   4.3&   0.6&  10.4&  11.9&  37.0&  29.7 \\ 
 711& 155728.906+472004.91&  0.1622&  40.0&  0.59&  0.05&   1.2&   1.8&   0.6&   3.1&   0.0&  12.0&   2.3&  12.6&  29.6&   0.0&  43.5 \\ 
 712& 155742.074+392655.56&  0.1014&  15.5&  0.15&  0.00&   1.2&   1.1&   0.5&   0.4&   0.0&  14.6&  18.9&  52.0&   0.1&  14.1&   0.0 \\ 
 713& 155815.722+180208.51&  0.0456&   1.7&  0.49&  0.06&   0.5&   4.9&  -0.0&   2.2&   0.3&  25.0&   2.3&   0.4&  57.7&   2.5&  11.6 \\ 
 714& 160014.062+050339.47&  0.2274&  40.1&  0.19&  0.17&   1.4&   1.8&   0.4&   2.1&   0.0&  10.6&   0.0&  89.4&   0.0&   0.0&   0.0 \\ 
 715& 160022.670+124527.99&  0.0344&   3.7&  0.16&  0.12&   2.0&   0.7&   0.9&   0.6&   0.0&  23.0&   8.6&  64.3&   4.0&   0.0&   0.0 \\ 
 716& 160051.494+150904.56&  0.0340&  10.1&  0.10&  0.07&   0.9&   1.7&  -0.3&   1.8&   0.2&   3.1&   0.8&  11.2&  16.8&  56.9&  10.3 \\ 
 717& 160151.384+042222.15&  0.1465&  23.7&  0.46&  0.20&   1.2&   3.7&   0.2&   2.2&   0.5&   0.4&   0.0&  53.1&   0.0&  17.8&  24.2 \\ 
 718& 160154.204+160016.80&  0.0383&   0.2&  0.15&  0.03&   1.8&  -0.2&   0.0&   0.0&   0.6&  82.1&  17.3&   0.0&   0.0&   0.0&   0.0 \\ 
 719& 160154.746+204410.08&  0.0828&   5.6&  0.18&  0.10&   1.5&   1.6&   0.7&   2.0&   0.1&  14.1&   1.2&  54.7&  29.3&   0.1&   0.0 \\ 
 720& 160156.700+122453.90&  0.0940&  11.5&  0.35&  0.11&   1.4&   2.9&   1.5&   2.4&   0.0&  13.8&   1.2&  65.3&  19.7&   0.0&   0.0 \\ 
 721& 160210.668+024505.15&  0.2441&  82.7&  0.43&  0.26&   2.6&   1.2&   0.2&   2.1&   0.0&   3.4&   1.1&  57.5&   0.0&  23.9&  12.8 \\ 
 722& 160229.244+335736.10&  0.0695&  10.5&  0.61&  0.06&   2.7&   1.5&   1.1&  -0.1&   0.0&   4.3&   6.7&  22.0&  28.6&   0.2&  38.1 \\ 
 723& 160303.636+214150.87&  0.0343&   2.1&  0.19&  0.14&   1.9&   0.3&   0.4&   0.4&   0.2&  19.8&   1.5&  29.6&  22.5&  26.2&   0.0 \\ 
 724& 160343.330+101958.38&  0.1913&  28.1&  0.14&  0.14&   0.7&   1.7&   0.6&   0.2&   0.0&   0.0&   0.0&  42.6&   0.0&  57.4&   0.0 \\ 
 725& 160417.304+155503.82&  0.0352&   0.7&  0.13&  0.05&   0.0&   0.6&   0.2&  -0.3&   0.0&   0.0&   0.0&  23.6&  35.8&  40.6&   0.0 \\ 
 726& 160448.737+170327.00&  0.1328&  16.3&  0.24&  0.05&   1.9&   1.4&   1.2&   1.2&   0.1&  22.5&   0.3&  62.7&  14.5&   0.0&   0.0 \\ 
 727& 160614.844+205011.37&  0.1839&  23.4&  0.04&  0.13&   3.0&   0.4&   0.2&   0.6&   0.0&  13.5&   2.7&  83.8&   0.0&   0.0&   0.0 \\ 
 728& 160630.118+183515.53&  0.0379&   1.8&  0.05&  0.04&   1.3&   0.9&   1.0&   2.4&   0.0&  15.0&   3.8&  45.2&  35.8&   0.0&   0.0 \\ 
 729& 160724.758+114154.41&  0.2068&  19.8&  0.23&  0.14&   0.9&   1.1&   0.2&   0.3&   0.1&  19.9&   0.0&  79.8&   0.2&   0.0&   0.0 \\ 
 730& 160740.301+203630.02&  0.1642&  20.4&  0.00&  0.08&   1.3&   0.4&   0.7&   0.2&   0.0&   6.0&   0.0&  43.9&  36.5&  13.5&   0.0 \\ 
 731& 160808.717+394755.92&  0.1909&  62.4&  0.22&  0.02&   1.3&   2.7&   0.1&   2.3&   0.1&   0.0&   4.0&  41.0&   0.0&  51.1&   0.0 \\ 
 732& 160812.264+155913.55&  0.2223&  32.8&  0.07&  0.05&   1.2&   0.6&  -0.1&   0.4&   0.1&   1.8&   0.0&  97.3&   0.0&   0.0&   0.0 \\ 
 733& 160813.092+362255.19&  0.0826&   7.0&  0.26&  0.03&   1.4&   1.6&   1.0&   2.0&   0.0&  20.5&   0.0&  49.8&  28.8&   0.0&   0.0 \\ 
 734& 161122.747+091558.05&  0.1545&  20.2&  0.38&  0.14&   1.5&   1.2&   0.5&   1.8&   0.0&   5.2&   0.2&  94.6&   0.0&   0.0&   0.0 \\ 
 735& 161129.184+331434.13&  0.3389&  47.2&  0.42&  0.02&   1.8&   3.4&   2.8&   2.2&   0.0&   3.0&   9.3&  36.0&  38.7&   0.0&   0.0 \\ 
 736& 161330.187+510335.57&  0.0336&   0.5&  0.41&  0.01&   0.4&   2.8&   0.5&   1.3&  19.5&  32.8&  22.3&   0.0&   0.0&   0.0&   0.0 \\ 
 737& 161446.824+085606.53&  0.1413&  15.9&  0.35&  0.17&   0.9&   1.1&  -0.6&  -0.0&   1.5&   4.5&   3.5&  41.9&   0.0&  47.6&   0.0 \\ 
 738& 161756.021+092035.67&  0.0836&   6.7&  0.26&  0.12&   2.3&   0.8&   0.2&  -0.2&   0.0&   8.5&   0.3&  51.9&  13.5&   0.0&  25.6 \\ 
 739& 161816.466+094506.37&  0.1307&  19.1&  0.17&  0.14&   0.7&   0.5&   0.2&   0.2&   0.0&  19.2&   6.7&  74.0&   0.0&   0.0&   0.0 \\ 
 740& 161925.980+215939.96&  0.1236&  12.8&  0.06&  0.12&   1.4&   5.6&   7.6&   2.5&   0.0&  21.5&   1.5&  43.7&   0.0&  32.2&   0.0 \\ 
 741& 162049.637+160944.45&  0.0832&   6.6&  0.30&  0.18&   0.7&   5.3&   0.7&   2.2&   0.0&   1.1&   0.0&  30.2&  68.7&   0.0&   0.0 \\ 
 742& 162100.811+211006.10&  0.0310&   8.1&  0.28&  0.14&   2.2&   1.0&   0.2&   2.7&   0.2&   7.2&   9.7&  16.2&  13.8&  52.5&   0.0 \\ 
 743& 162124.029+075947.78&  0.1264&  18.3&  0.40&  0.20&   1.4&   1.6&   0.3&   1.3&   0.1&  17.3&   7.1&  74.3&   0.0&   0.0&   0.0 \\ 
 744& 162200.283+235531.84&  0.0602&   5.0&  0.50&  0.11&   0.7&   3.6&  -0.2&   2.2&   0.1&  22.3&   1.3&   7.1&  15.8&   0.0&  53.4 \\ 
 745& 162205.705+185950.58&  0.1025&  10.4&  0.43&  0.16&   1.2&   3.7&   0.7&   4.2&   0.6&  11.9&  10.5&  28.8&  12.2&  34.5&   0.4 \\ 
 746& 162415.134+170105.53&  0.0346&   1.3&  0.50&  0.17&   0.4&   5.0&  -0.1&   2.5&   0.0&  12.5&   0.0&   3.8&  83.7&   0.0&   0.0 \\ 
 747& 162440.783+081727.79&  0.0993&   7.0&  0.34&  0.22&   2.1&   0.9&   0.6&   2.4&   0.4&  17.8&  17.3&  50.5&  13.7&   0.0&   0.0 \\ 
 748& 162503.350+070402.94&  0.0479&   3.8&  0.19&  0.24&   0.6&   4.7&   1.0&   5.4&   0.3&  12.7&   0.1&  14.6&  48.4&  23.6&   0.0 \\ 
 749& 162507.680+091714.28&  0.1984&  20.0&  0.68&  0.15&   0.7&   2.1&   0.1&   2.1&   0.2&  38.1&   0.0&  61.7&   0.0&   0.0&   0.0 \\ 
 750& 162702.561+432833.94&  0.0463&  34.3&  0.50&  0.02&   1.2&   1.9&  -0.1&   2.4&   0.0&   3.6&   0.6&   2.8&  23.8&  35.8&  33.2 \\ 
 751& 162718.799+255229.63&  0.1925&  32.0&  0.47&  0.09&   1.2&   2.1&   0.2&   1.9&   0.0&   9.3&   0.9&  60.5&   4.3&   8.9&  14.8 \\ 
 752& 162740.726+132634.53&  0.0900&  16.8&  0.71&  0.18&   1.0&   5.1&   1.0&   3.2&   0.1&   5.8&   0.2&  22.4&  44.4&   0.0&  27.0 \\ 
 753& 162755.956+480051.14&  0.1259&  13.3&  0.15&  0.02&   1.5&   1.1&  -0.1&   0.8&   0.4&   7.0&   4.1&  61.8&   0.0&  11.0&  15.6 \\ 
 754& 162800.151+413335.35&  0.2715& 175.5&  0.03&  0.00&  -3.4&  -0.2&   0.1&   0.0&   0.0&   1.1&   0.3&   9.9&   9.7&  56.2&  22.4 \\ 
 755& 162930.528+423447.31&  0.1158&  12.6&  0.23&  0.00&   2.3&   0.5&   0.1&   0.5&   0.0&  15.0&   6.2&  78.8&   0.0&   0.0&   0.0 \\ 
 756& 162938.266+302924.92&  0.0971&  36.3&  0.04&  0.02&   2.4&   0.8&   0.4&   1.2&   0.0&   1.9&   0.5&  25.0&  10.7&  27.9&  33.8 \\ 
 757& 163159.906+431754.46&  0.2251&  47.3&  0.10&  0.01&   1.1&   1.4&   0.5&   0.5&   0.0&   0.9&   0.1&  64.5&   0.0&  22.2&  12.3 \\ 
 758& 163214.198+241150.97&  0.0643&   3.9&  0.36&  0.12&   0.3&   2.3&   0.4&   2.1&   1.1&  13.7&   0.7&  12.7&  67.5&   0.0&   3.9 \\ 
 759& 163607.692+284408.39&  0.1426&  42.9&  0.71&  0.07&   1.4&   1.6&   0.7&   2.5&   0.0&   7.4&   0.4&  35.8&  30.2&   6.3&  19.8 \\ 
 760& 163658.750+173946.79&  0.1280&  70.5&  0.65&  0.30&   0.8&   4.4&   0.2&   2.5&   0.1&   5.7&   0.2&  16.8&  31.4&  21.9&  23.6 \\ 
 761& 163835.054+440349.43&  0.1122&  10.7&  0.46&  0.00&   1.8&   2.8&   0.8&   0.4&   0.0&  46.5&   0.0&  53.5&   0.0&   0.0&   0.0 \\ 
 762& 163859.402+250402.91&  0.2693&  57.9&  0.48&  0.10&   1.5&   4.0&   2.6&   2.0&   0.1&   0.0&   0.0&  45.0&  46.7&   0.0&   0.0 \\ 
 763& 163916.397+273333.90&  0.1111&  15.5&  0.19&  0.18&   1.7&   0.4&   0.2&   0.6&   0.1&   4.7&   2.5&  92.7&   0.0&   0.0&   0.0 \\ 
 764& 164255.162+415335.63&  0.0726&  20.7&  0.32&  0.00& -36.2&  -0.0&  -0.0&   0.1&   0.0&  12.7&   1.9&  31.3&  37.3&  16.8&   0.0 \\ 
 765& 164300.041+281944.61&  0.1750& 134.0&  0.92&  0.12&   0.9&   1.8&  -0.6&   2.1&   0.0&  10.3&   1.1&  29.7&   0.0&  54.3&   4.6 \\ 
 766& 164608.266+363705.21&  0.1366&  13.3&  0.22&  0.07&   1.1&   2.0&  -0.1&   0.9&   0.0&  10.1&   0.0&  89.9&   0.0&   0.0&   0.0 \\ 
 767& 164610.478+324258.73&  0.1377&  13.4&  0.00&  0.07&   2.5&   0.3&   0.3&   0.6&   0.0&  10.4&  15.5&  52.6&   0.0&  20.5&   0.0 \\ 
 768& 165030.946+295601.02&  0.1220&  22.1&  0.87&  0.12&   0.9&   1.8&  -0.3&   2.8&   0.1&  14.5&   0.3&  12.8&   2.4&  20.3&  49.6 \\ 
 769& 165437.337+295415.33&  0.0713&  22.7&  1.68&  0.16&   0.9&   3.7&   0.3&   1.2&   0.0&   0.0&   0.0&   0.0&  71.7&  28.3&   0.0 \\ 
 770& 165639.288+184021.69&  0.1671&  16.3&  0.65&  0.34&   0.8&   1.9&   0.3&   2.9&   0.0&  25.8&   0.0&  74.2&   0.0&   0.0&   0.0 \\ 
 771& 165648.641+314702.38&  0.0998&  14.5&  0.33&  0.09&   1.7&   2.0&   0.5&   2.7&   0.0&   7.0&   1.2&  91.5&   0.0&   0.0&   0.0 \\ 
 772& 165804.771+632608.97&  0.0975&  25.2&  0.20&  0.03&   1.7&   0.7&   0.2&   0.6&   0.4&   3.4&   0.2&  42.5&   0.1&  31.4&  20.6 \\ 
 773& 165820.664+245628.86&  0.1892&  59.5&  0.16&  0.18&   1.3&   2.3&   0.4&   1.6&   0.1&   1.1&   0.2&  34.5&   5.7&  18.1&  39.6 \\ 
 774& 165902.064+371514.36&  0.1123&   7.1&  0.21&  0.06&   3.0&   0.7&   0.4&   0.6&   0.1&  11.6&  20.2&  64.8&   0.0&   3.0&   0.0 \\ 
 775& 165958.032+213640.06&  0.1567&  54.5&  0.66&  0.27&   1.7&   3.1&   0.1&   2.4&   0.2&  18.9&   5.4&  14.5&  10.0&   4.0&  45.9 \\ 
 776& 170057.230+601924.84&  0.1490&  25.6&  0.46&  0.01&   1.0&   2.5&   0.6&   2.1&   0.0&   9.5&   1.0&  52.8&   1.2&  19.5&  15.9 \\ 
 777& 170128.190+190337.74&  0.2835&  46.4&  0.02&  0.34&   0.2&   0.5&  -0.0&   1.2&   0.0&   0.0&   0.0&  99.9&   0.0&   0.0&   0.0 \\ 
 778& 170252.474+630710.07&  0.1634&  37.1&  0.44&  0.02&   0.7&   5.1&   0.5&   2.2&   0.1&  13.1&   0.8&  27.8&   8.0&   0.0&  50.3 \\ 
 779& 170356.712+622848.28&  0.1453&  17.4&  0.33&  0.03&   0.9&   1.9&   0.8&   1.5&   0.5&  12.0&   2.5&  22.2&  11.6&  35.8&  14.4 \\ 
 780& 170557.425+630055.58&  0.1048&  12.3&  0.21&  0.06&   1.1&   1.1&   0.1&   0.8&   0.2&  12.6&   9.9&  73.5&   2.5&   0.0&   0.0 \\ 
 781& 170636.588+334720.44&  0.1245&  29.8&  0.47&  0.09&   1.2&   2.4&   0.1&   2.2&   0.2&  10.8&   5.3&  31.8&  38.1&  13.2&   0.0 \\ 
 782& 171430.331+321508.77&  0.1365&  18.1&  0.16&  0.17&   1.5&   1.3&   0.4&   2.0&   0.0&   8.8&   2.2&  88.4&   0.0&   0.0&   0.0 \\ 
 783& 171546.258+582255.47&  0.1271&  14.0&  0.26&  0.06&   0.4&   2.5&   0.6&   1.5&   0.0&  16.0&   0.3&  40.0&  12.9&   0.0&  30.6 \\ 
 784& 172010.834+274214.75&  0.1590&  52.6&  0.26&  0.16&   0.8&   5.3&  -0.1&   3.6&   0.2&   3.1&   0.0&  19.9&   5.8&  17.5&  52.4 \\ 
 785& 172036.091+631722.47&  0.1794&  23.4&  0.11&  0.10&   5.5&   0.2&  -1.3&  -0.3&   0.0&  22.1&   0.3&  31.5&  11.4&   0.0&  34.5 \\ 
 786& 173139.158+544631.48&  0.1368&  38.8&  0.55&  0.13&   0.8&   5.4&  -0.3&   2.1&   0.5&   8.6&   2.0&  22.4&   0.1&  24.5&  40.7 \\ 
 787& 174133.046+540325.42&  0.1136&  15.8&  0.49&  0.12&   0.7&   1.7&   0.4&   1.8&   0.0&  19.0&   2.7&  28.3&  35.8&   9.3&   4.3 \\ 
 788& 210443.855-073145.45&  0.3072& 189.0&  0.39&  0.23&   1.3&   1.9&   0.4&   1.9&   0.0&   0.3&   1.2&  29.0&   0.0&  37.3&  32.2 \\ 
 789& 211230.600-005022.42&  0.2146&  36.4&  0.59&  0.18&   1.0&   3.6&   0.9&   2.9&   0.4&  31.9&  12.1&  16.3&   9.3&  29.2&   0.0 \\ 
 790& 211348.163-063059.63&  0.1589&  29.4&  0.39&  0.38&   2.2&   1.1&  -0.2&   1.7&   0.0&   7.8&   1.8&  60.3&   0.3&   5.6&  24.2 \\ 
 791& 211948.178+004021.76&  0.0344&   1.2&  0.11&  0.24&   2.5&   0.5&   0.4&   4.9&   0.2&   9.0&   0.0&  17.4&  31.2&  42.1&   0.0 \\ 
 792& 212036.403-063722.61&  0.1191&  12.0&  0.14&  0.33&   0.7&   1.3&   0.6&   1.9&   0.0&   1.1&   0.2&  68.1&   0.0&  30.1&   0.0 \\ 
 793& 212233.367+010016.52&  0.1851&  77.4&  0.57&  0.19&   1.7&   2.0&   0.3&   1.9&   0.0&   3.2&   0.3&  15.2&   9.1&  26.0&  45.8 \\ 
 794& 213556.916+000328.71&  0.0856&   3.9&  0.15&  0.17&  -7.1&  -0.0&   1.2&   1.7&   0.2&  21.5&   6.4&  69.0&   3.0&   0.0&   0.0 \\ 
 795& 214307.529-080727.48&  0.2283&  82.9&  0.36&  0.09&   1.0&   1.8&   0.5&   1.0&   0.0&   7.2&   0.6&  25.7&   6.5&  24.0&  36.0 \\ 
 796& 214456.719-070708.13&  0.0857&  12.6&  0.58&  0.06&   1.6&   3.3&   0.3&   3.9&   0.3&  10.0&   1.1&   8.1&  70.3&   9.8&   0.0 \\ 
 797& 215735.446-005021.44&  0.2186&  39.8&  0.11&  0.33&   1.7&   1.0&   0.5&   1.6&   0.0&   1.7&   0.3&  97.9&   0.0&   0.0&   0.0 \\ 
 798& 220122.889+002516.09&  0.2230& 101.5&  0.27&  0.18&   3.3&   0.8&   0.5&   1.0&   0.0&   0.0&   0.9&  26.5&   0.0&  39.7&  32.9 \\ 
 799& 220545.533-092916.59&  0.1354&   9.9&  0.30&  0.07&   1.4&   1.2&   0.4&   1.8&   0.0&  15.5&   0.0&  84.5&   0.0&   0.0&   0.0 \\ 
 800& 223138.119-080652.61&  0.1917&  46.6&  0.06&  0.13&   1.9&   1.3&   0.5&   1.8&   0.0&   1.0&   0.4&   5.2&  38.3&   9.9&  44.4 \\ 
 801& 225348.322-084624.58&  0.1503&  35.2&  0.36&  0.10&   1.7&   1.3&  -0.1&   1.2&   0.4&  10.4&   0.0&  31.8&   0.6&  56.0&   0.0 \\ 
 802& 225506.799+005839.92&  0.0534&  34.4&  0.04&  0.20&   0.7&   2.5&  -0.1&   2.6&   0.3&   0.9&   0.2&   7.6&   4.1&  44.0&  42.4 \\ 
 803& 230128.246-083355.81&  0.1812&  36.8&  0.34&  0.08&   2.1&   1.2&   0.4&   1.8&   0.0&  24.8&   1.1&  26.6&   3.6&  17.1&  26.1 \\ 
 804& 231947.688+004316.07&  0.1186&   9.6&  0.23&  0.14&   1.7&   2.2&   0.3&   1.9&   0.1&  12.6&   5.9&  80.3&   0.1&   0.0&   0.0 \\ 
 805& 233712.763-105800.32&  0.0783&  16.1&  0.31&  0.07&   1.6&   1.4&   0.1&   0.9&   0.0&   7.1&   3.2&  89.7&   0.0&   0.0&   0.0 \\ 
 806& 234640.250-090754.15&  0.1919&  23.7&  0.00&  0.08&  -0.0&   0.6&   0.3&   0.4&   0.0&  12.4&   4.0&  60.0&  23.4&   0.0&   0.0 \\ 
 807& 234743.507-103447.41&  0.1470&  32.8&  0.37&  0.10&   2.2&   0.6&   0.3&   1.1&   0.0&  29.7&   0.0&  70.3&   0.0&   0.0&   0.0 \\ 
 808& 235355.800-102113.77&  0.0731&   1.8&  0.00&  0.09&   3.5&   1.2&   2.6&   2.1&   0.1&  28.1&   3.1&  59.9&   0.2&   8.6&   0.0 \\ 


==> seds.tex <==
#lista                 vname    _FX0    _FX1    _FX2    _FX3    _FX4    _FX5    _FX6    _FX7    _FX8    _FX9   _FX10   _FX11   _FX12   _FX13        _FX14
#
   1& 001027.392-104341.71&   0.00&  14.57&  21.91&  46.73&  49.51&  41.73&  35.40&   0.00&  21.21&  10.78&   7.50&   1.83&   0.93&   0.55&   0.39 \\ 
   2& 001551.253-102317.92&  17.01&  11.74&  13.21&  35.22&  38.24&  31.69&  26.42&   0.00&  16.41&  10.58&   5.92&   1.14&   0.49&   0.07&   0.00 \\ 
   3& 010823.370-094356.22&   0.00&   0.00&   8.33&  17.70&  24.44&  22.44&  19.46&   0.00&  12.44&  11.31&   5.15&   1.13&   0.44&   0.00&   0.19 \\ 
   4& 011942.227+010751.63&  16.51&  24.61&  25.91&  56.62&  57.04&  48.34&  42.05&   0.00&  32.57&  24.67&  11.38&   2.39&   0.81&   0.08&   0.00 \\ 
   5& 012015.683-095920.12&   0.00&  10.17&  12.92&  34.19&  37.75&  32.13&  27.35&   0.00&  22.10&  12.20&   3.63&   1.62&   0.60&   0.07&   0.24 \\ 
   6& 014327.340-011342.55&   3.69&   6.66&   7.75&  20.41&  28.80&  26.64&  22.75&  20.55&  16.15&  11.84&   7.26&   1.47&   0.64&   0.35&   0.37 \\ 
   7& 014838.633-093259.77&   3.90&   0.00&   9.12&  24.25&  32.38&  28.64&  24.63&   0.00&  16.19&  10.64&   6.16&   1.29&   0.49&   0.07&   0.00 \\ 
   8& 015107.018-005636.72&   1.49&   4.93&   9.69&  24.30&  31.78&  28.20&  24.74&  21.92&  18.45&  12.27&   6.95&   1.59&   0.65&   0.11&   0.00 \\ 
   9& 020505.984-004345.25&  23.26&  29.85&  27.71&  47.72&  46.78&  39.83&  31.64&  26.33&  19.83&   9.36&   5.98&   1.18&   0.44&   0.15&   0.00 \\ 
  10& 021007.624-095431.19& 227.70& 181.10&  79.85& 126.30& 105.20&  85.36&  62.76&   0.00&   0.00&   0.00&   0.00&   1.19&   0.39&   0.17&   0.11 \\ 
  11& 022427.085-093739.48&   0.00&   0.00&  17.99&  43.61&  45.43&  38.02&  32.09&   0.00&  21.41&  13.43&   8.54&   1.70&   0.58&   0.06&   0.00 \\ 
  12& 022743.211-001523.04&  42.02&  49.50&  40.48&  61.08&  68.95&  55.27&  44.83&  36.01&  28.69&  18.32&  10.30&   2.24&   0.90&   0.23&   0.21 \\ 
  13& 022957.373-005412.86&   0.00&  14.55&  16.25&  44.72&  49.32&  43.08&  35.69&   0.00&  23.34&  15.41&   8.26&   1.65&   0.61&   0.19&   0.10 \\ 
  14& 023446.381+003035.87&   0.00&   0.00&  14.39&  32.85&  35.45&  29.36&  25.06&  22.68&  18.56&  11.06&   6.23&   1.24&   0.46&   0.05&   0.00 \\ 
  15& 025203.278-081839.42&   0.00&  10.25&   0.00&  30.18&  42.56&  34.83&  30.05&   0.00&  16.28&  11.60&   7.15&   1.78&   0.66&   0.15&   0.11 \\ 
  16& 025559.311-010823.08&  21.72&  24.32&  28.88&  51.48&  58.25&  47.16&  35.07&  28.01&  21.49&  14.19&   7.25&   1.56&   0.62&   0.22&   0.00 \\ 
  17& 025850.526+003458.72&   0.00&  44.03&  39.37&  64.32&  67.95&  55.76&  46.98&  34.77&  28.67&  18.06&   9.99&   2.05&   0.81&   0.24&   0.00 \\ 
  18& 030228.430-005618.13&   0.00&  30.52&  41.22&  77.20&  78.65&  65.75&  53.80&   0.00&  28.82&  21.66&  11.97&   2.60&   1.05&   0.65&   0.29 \\ 
  19& 032033.650-002021.24&   0.00&   0.00&   7.05&  20.60&  19.16&  15.06&  12.03&  61.54&  46.49&  26.39&  20.27&   1.46&   0.54&   0.15&   0.00 \\ 
  20& 073214.273+390405.81&   0.00&   7.06&  20.71&  37.12&  43.19&  37.04&  32.04&   0.00&  19.70&  12.69&   7.89&   1.02&   0.30&   0.13&   0.00 \\ 
  21& 073420.839+314419.72&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&  15.99&  12.35&   0.00&   1.06&   0.31&   0.00&   0.00 \\ 
  22& 073537.325+393345.70&   0.00&  45.54&  45.05&  97.15&  89.04&  69.04&  54.14&   0.00&  36.41&  19.92&  12.37&   2.50&   0.90&   0.20&   0.00 \\ 
  23& 073724.079+382438.81&   0.00&  12.68&  16.87&  38.47&  42.37&  36.07&  30.64&   0.00&  19.39&  11.99&   5.57&   1.29&   0.45&   0.00&   0.00 \\ 
  24& 074541.458+220821.98&   0.00& 129.40&  48.14& 107.30&  97.43&  75.51&  57.99&  47.85&  36.57&  23.29&  12.18&   2.52&   0.90&   0.38&   0.00 \\ 
  25& 074630.900+333318.81&   0.00&  34.27&  32.32&  38.52&  47.96&  41.38&  39.08&   0.00&  18.76&  15.45&   8.65&   1.73&   0.64&   0.25&   0.00 \\ 
  26& 074650.321+224937.12&   0.00&  12.24&  30.59&  72.79&  74.73&  60.42&  49.22&  39.29&  32.14&  22.07&  11.64&   2.38&   0.84&   0.00&   0.00 \\ 
  27& 074820.234+175952.67&   0.00&  17.30&   9.18&  11.32&  10.79&   8.57&   9.36&   0.00&  10.42&   5.53&   0.00&   0.54&   0.10&   0.00&   0.00 \\ 
  28& 075056.918+480245.92&   0.00&   0.00&  46.08& 100.40&  98.18&  78.91&  67.08&   0.00&  43.34&  27.84&  15.26&   2.96&   0.96&   0.00&   0.00 \\ 
  29& 075246.207+382928.46&  46.60&  43.78&  48.34&  97.45&  92.65&  73.18&  60.44&   0.00&  34.29&  20.88&  13.23&   2.32&   0.82&   0.17&   0.00 \\ 
  30& 075255.994+384330.63&   0.00&   0.00&  14.57&  29.82&  32.66&   0.00&   0.00&   0.00&  16.55&  13.37&   6.71&   1.12&   0.37&   0.00&   0.00 \\ 
  31& 075318.070+450307.92&  51.06&  43.26&  32.21&  53.07&  51.55&  44.01&  31.35&   0.00&   0.00&   0.00&   0.00&   1.01&   0.30&   0.11&   0.00 \\ 
  32& 075323.098+243300.56&  37.58&  97.87&  77.15& 197.50& 190.90& 156.20& 128.00& 120.20&  96.44&  67.85&  31.83&   6.19&   2.02&   0.35&   0.00 \\ 
  33& 075339.602+301125.88&   0.00&   0.00&  11.33&  26.82&  35.15&  30.46&  25.82&   0.00&  15.41&  11.36&   5.29&   1.43&   0.62&   0.00&   0.00 \\ 
  34& 075423.026+375230.72&   0.00&  42.69&  29.99&  56.42&  58.78&  48.87&  39.83&   0.00&  25.03&  16.08&   9.61&   1.72&   0.72&   0.13&   0.00 \\ 
  35& 075440.183+124510.74&   0.00&  29.40&  26.77&  47.74&  57.17&  48.20&  41.04&   0.00&  21.12&  17.93&  13.42&   2.05&   0.82&   0.16&   0.00 \\ 
  36& 075528.968+213038.24&   0.00&   6.97&   7.00&  21.79&  33.94&  30.83&  25.38&  20.08&  15.05&  10.60&   6.75&   1.43&   0.61&   0.17&   0.14 \\ 
  37& 075658.898+362255.14&   0.00&  27.07&  28.85&  49.49&  51.43&  42.89&  34.57&   0.00&  21.92&  12.50&   8.62&   1.65&   0.66&   0.00&   0.00 \\ 
  38& 075710.942+142736.10&   0.00&   6.79&   8.18&  25.30&  33.22&  29.49&  24.17&   0.00&  17.86&   8.45&   6.39&   1.39&   0.56&   0.10&   0.00 \\ 
  39& 080037.058+261356.59&  23.73&  34.20&  23.49&  38.69&  40.47&  34.46&  28.80&   0.00&  19.05&  12.99&   7.01&   1.48&   0.55&   0.12&   0.00 \\ 
  40& 080103.761+344144.57&   0.00&  19.35&  30.32&  60.57&  68.04&  58.68&  49.48&   0.00&  27.78&  20.04&  11.35&   2.06&   0.77&   0.17&   0.00 \\ 
  41& 080127.970+321017.28&   0.00&  16.08&  25.56&  46.47&  49.49&  40.23&  30.78&   0.00&  19.69&  12.37&   6.85&   1.44&   0.56&   0.00&   0.00 \\ 
  42& 080218.394+323207.81&   0.00&  55.05& 119.40& 289.50& 281.90& 233.00& 190.50&   0.00& 139.30&  82.37&  45.51&   8.47&   2.58&   0.42&   0.14 \\ 
  43& 080246.610+085110.92&   0.00&  26.75&  33.99&  90.61& 101.30&  85.89&  72.46&   0.00&  45.02&  28.11&  14.31&   3.42&   1.17&   0.00&   0.00 \\ 
  44& 080330.523+310840.02&  41.99&  44.50&  48.02&  47.64&  52.90&  44.50&  45.62&   0.00&  17.92&  11.13&   8.55&   1.96&   0.72&   0.32&   0.00 \\ 
  45& 080346.450+291816.84&   0.00&   0.00&   8.92&  18.74&  26.55&  24.27&  21.34&  17.09&  13.45&  10.52&   5.60&   1.24&   0.56&   0.00&   0.00 \\ 
  46& 080446.742+104641.74&  95.42&   0.00&   0.00&   5.80&   2.35&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00 \\ 
  47& 080532.772+372801.05&   0.00&   5.40&  19.20&  34.71&  32.01&  26.91&  23.17&   0.00&  11.99&   0.00&   0.00&   0.63&   0.19&   0.00&   0.00 \\ 
  48& 080725.159+362222.68&   0.00&   0.00&  19.81&  36.85&  36.16&  28.50&  22.61&   0.00&   9.13&  10.15&   5.13&   0.96&   0.37&   0.00&   0.00 \\ 
  49& 080738.412+385625.57&   0.00&  41.75&  79.73& 165.20& 157.30& 129.20& 110.80&   0.00&  74.91&  48.65&  23.15&   4.91&   1.47&   0.44&   0.00 \\ 
  50& 080801.699+393145.96&   0.00&  32.03&  20.06&  39.77&  36.00&  29.02&  22.60&   0.00&  13.42&   5.36&   4.78&   1.01&   0.40&   0.12&   0.00 \\ 
  51& 080925.082+305652.85&  22.24&  46.81&  79.95& 189.10& 189.10& 157.80& 129.10&   0.00&  83.91&  50.99&  29.01&   6.56&   2.12&   0.35&   0.20 \\ 
  52& 081120.626+352147.40&   0.00&   0.00&  11.29&  21.07&  15.72&  12.01&   9.39&   0.00&  13.51&  10.00&   6.75&   6.30&   2.08&   0.41&   0.20 \\ 
  53& 081412.485+103744.38&   0.00&   0.00&  33.93&  67.56&  65.68&  53.95&  44.94&   0.00&  21.91&  14.81&   8.83&   1.63&   0.58&   0.35&   0.15 \\ 
  54& 081415.432+081359.90&   0.00&   9.39&  14.97&  33.76&  47.46&  40.90&  35.36&   0.00&  22.19&  12.67&   8.22&   1.69&   0.71&   0.23&   0.00 \\ 
  55& 081525.771+372025.85&  39.03&  78.14&  92.86& 139.90& 126.00& 101.10&  81.62&   0.00&  44.40&  27.57&  12.41&   3.43&   1.14&   0.52&   0.25 \\ 
  56& 081629.940+291559.34&   0.00&  51.16&  22.15&   0.00&   0.00&   0.00&   0.00&  31.80&  23.88&  14.71&   7.99&   1.81&   0.68&   0.08&   0.00 \\ 
  57& 081641.124+221847.78&   0.00&  50.72&  44.48&  69.63&  67.98&  53.82&  40.65&  33.46&  25.43&  16.67&   9.16&   1.88&   0.72&   0.42&   0.00 \\ 
  58& 081802.412+281232.23&  14.89&   0.00&  16.50&  40.09&  39.97&  33.83&  27.89&  23.28&  17.04&  12.47&   6.25&   1.38&   0.50&   0.10&   0.00 \\ 
  59& 081912.014+405856.41&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&  17.26&  11.39&   7.55&   1.67&   0.71&   0.24&   0.00 \\ 
  60& 081922.205+062523.11&   0.00&   6.13&  12.55&  36.63&  40.22&  33.27&  26.00&  20.85&  17.62&  11.92&   6.19&   1.25&   0.52&   0.13&   0.00 \\ 
  61& 081936.794+282405.62&  14.43&  25.37&  26.20&  54.02&  54.10&  42.33&  33.66&  24.38&  18.52&  12.25&   6.66&   1.51&   0.50&   0.15&   0.00 \\ 
  62& 081953.532+041409.22&  82.52& 115.80&  43.18&  46.55&  46.03&  32.01&  24.27&  22.26&  14.99&  10.44&   6.07&   1.68&   0.87&   0.34&   0.19 \\ 
  63& 082134.238+432301.03&   0.00&  37.49&  31.15&  59.76&  69.65&  57.29&  48.39&   0.00&  21.57&  11.91&   9.06&   2.00&   0.77&   0.43&   0.00 \\ 
  64& 082254.881+192128.22&   0.00&  23.36&  40.62&  60.60&  49.98&  38.10&  29.83&   0.00&  30.95&  18.82&   8.78&   1.89&   0.75&   0.63&   0.93 \\ 
  65& 082518.910+412039.78&   0.00&  10.86&  14.42&  29.98&  32.83&  27.08&  22.62&   0.00&  15.47&   8.44&   5.57&   1.03&   0.42&   0.00&   0.00 \\ 
  66& 082655.471+135059.51&   0.00&   0.00&   8.11&   6.17&  12.96&   9.82&   7.95&   0.00&   0.00&   0.00&   0.00&   0.39&   0.13&   0.00&   0.00 \\ 
  67& 082752.838+260502.48&  17.23&   0.00&  21.19&  49.23&  48.17&  40.72&  35.81&  26.79&  19.44&  13.33&   6.48&   1.40&   0.49&   0.15&   0.00 \\ 
  68& 082858.685+274101.33&  35.91&  31.56&  27.68&  56.46&  51.48&  42.49&  34.53&  28.29&  23.15&  15.90&   7.04&   1.73&   0.56&   0.14&   0.36 \\ 
  69& 082930.302+350216.51&   0.00&  18.36&  28.61&  52.01&  53.96&  46.10&  36.08&   0.00&  21.15&  12.71&   8.76&   1.69&   0.68&   0.30&   0.18 \\ 
  70& 083035.626+492719.22&  28.28&  31.28&  50.24& 106.80& 111.90&  91.81&  77.25&   0.00&  49.39&  30.56&  19.57&   4.01&   1.46&   0.17&   0.12 \\ 
  71& 083036.559+071347.61&   0.00&  12.61&  19.59&  37.05&  39.20&  31.64&  26.25&  19.57&  13.02&   9.00&   6.00&   1.15&   0.49&   0.00&   0.00 \\ 
  72& 083130.043+403729.62&  37.73&  36.65&  17.90&  33.52&  32.56&  26.33&  21.31&   0.00&  15.94&  10.21&   4.45&   1.07&   0.40&   0.08&   0.00 \\ 
  73& 083231.308+492440.69&   0.00&  28.52&  17.98&  40.64&  44.98&  37.25&  30.90&   0.00&  23.44&  11.51&   8.65&   1.67&   0.64&   0.12&   0.00 \\ 
  74& 083317.222+413533.32&  32.22&  24.60&  22.20&  51.88&  57.74&  62.56&  44.92&   0.00&  28.26&  24.46&  14.10&   2.48&   0.94&   0.23&   0.00 \\ 
  75& 083319.171+370436.93&   0.00&   0.00& 106.20& 188.00& 169.10& 135.10&  98.12&   0.00&  57.83&  38.82&  19.04&   3.86&   1.68&   2.27&   6.78 \\ 
  76& 083340.301+534258.55&   0.00&   0.00&   0.00& 117.70&  85.57&  52.94&  44.30&   0.00&  28.46&  21.45&   9.89&   2.36&   0.85&   0.10&   0.00 \\ 
  77& 083415.653+375157.09&   0.00&  42.18&  45.56&  95.39& 112.00&  93.42&  78.82&   0.00&  52.69&  35.23&  19.67&   3.90&   1.40&   0.17&   0.00 \\ 
  78& 083433.708+172046.34&   0.00&  63.50& 105.80& 274.50& 238.50& 184.20& 141.90&   0.00& 127.10&  86.27&  47.88&  10.91&   4.11&   3.61&   1.92 \\ 
  79& 083449.697+100049.52&   0.00&   0.00&  10.23&  24.50&  26.91&  22.55&  19.41&   0.00&  13.83&  10.51&   4.31&   1.06&   0.38&   0.00&   0.00 \\ 
  80& 083454.797+251258.51&  97.57&  81.98&  83.72& 171.70& 182.80& 153.30& 131.70& 103.80&  88.06&  59.34&  30.11&   5.72&   1.90&   0.18&   0.16 \\ 
  81& 083503.108+524039.26&   0.00&  15.84&  25.42&  44.60&  43.46&  35.28&  26.90&   0.00&  20.02&  12.29&   0.00&   1.10&   0.41&   0.07&   0.00 \\ 
  82& 083521.230+423936.03&   0.00&  31.01&  52.36& 117.20& 111.80&  90.07&  72.99&   0.00&  48.59&  31.02&  16.23&   3.26&   1.12&   0.18&   0.00 \\ 
  83& 083651.588+173207.98&   0.00&  41.03&  46.56&  84.48&  78.61&  64.63&  52.44&   0.00&  29.14&  22.09&  11.08&   2.03&   0.75&   0.19&   0.00 \\ 
  84& 083913.284+120350.42&   0.00&  14.57&  18.63&  34.37&  42.31&  33.89&  27.93&   0.00&  15.78&  12.99&   7.99&   1.50&   0.57&   0.11&   0.00 \\ 
  85& 083914.256+620825.00&   0.00&   0.00&  16.71&  40.05&  57.04&  54.58&  53.51&   0.00&  27.61&  16.91&  10.37&   2.30&   0.81&   0.14&   0.00 \\ 
  86& 083948.425+543450.70&  20.06&  24.20&  60.89& 127.90& 125.30& 103.40&  86.79&   0.00&  57.64&  29.92&  16.48&   3.37&   1.03&   0.34&   0.19 \\ 
  87& 084032.004+324747.40&   0.00&   8.87&  20.32&  35.47&  35.16&  29.27&  22.09&   0.00&  17.31&  13.64&   5.53&   1.39&   0.45&   0.09&   0.00 \\ 
  88& 084041.004+190343.79&   0.00&   3.64&  17.69&  40.89&  54.39&  49.17&  42.06&   0.00&  30.05&  19.10&  14.01&   2.52&   1.07&   0.13&   0.00 \\ 
  89& 084056.131+175731.14&  29.51&  42.30&  50.56&  99.67& 100.50&  84.17&  69.42&   0.00&  41.54&  26.10&  15.23&   2.96&   1.01&   0.12&   0.00 \\ 
  90& 084141.134+264239.20&   3.20&   9.16&  14.77&  43.84&  53.40&  42.44&  30.32&  23.72&  18.47&  13.38&   6.64&   1.38&   0.46&   0.00&   0.00 \\ 
  91& 084211.446+401040.79&   0.00&   4.64&  12.03&  27.90&  35.40&  32.48&  29.30&   0.00&  21.71&  11.78&   5.72&   1.49&   0.48&   0.00&   0.00 \\ 
  92& 084305.762+214200.91&   0.00&   0.00&  39.68&  77.35&  66.71&  51.13&  41.08&   0.00&  27.36&  18.30&   7.48&   1.87&   0.72&   0.11&   0.00 \\ 
  93& 084414.678+023426.77&   0.00&   0.00&  50.05&  54.50&  64.78&  50.14&  40.18&  28.45&  21.22&  17.11&   9.40&   2.03&   0.77&   0.22&   0.00 \\ 
  94& 084416.632+263303.35& 102.40&  99.68&  92.09& 142.20& 118.50& 111.00&  68.11&   0.00&  60.34&  43.29&  24.50&   4.65&   1.70&   1.09&   0.35 \\ 
  95& 084457.482+074510.86&   0.00&   0.00&  13.02&  27.94&  27.28&  22.43&  17.70&  14.62&  10.66&   7.55&   3.93&   0.72&   0.26&   0.00&   0.00 \\ 
  96& 084532.462+302339.75&  13.33&  28.75&  32.75&  63.33&  63.61&  51.99&  45.60&   0.00&  21.73&  16.50&   8.14&   1.57&   0.51&   0.09&   0.00 \\ 
  97& 084542.703+292932.81&   0.00&   0.00&  14.01&  23.97&  25.13&  19.96&  17.86&  11.60&   9.60&   6.82&   3.74&   0.83&   0.31&   0.08&   0.00 \\ 
  98& 084632.710+172445.96&   0.00&   8.26&  11.50&  25.62&  34.08&  30.01&  26.48&   0.00&  18.92&   9.95&   5.85&   1.43&   0.57&   0.00&   0.00 \\ 
  99& 084715.854+315510.88&  20.14&  16.30&  16.53&  31.67&  35.78&  31.19&  25.31&   0.00&  19.64&  11.89&   5.36&   1.88&   0.93&   0.28&   0.00 \\ 
 100& 084738.868+084446.31&  11.24&  17.42&  19.08&  38.70&  38.35&  30.19&  24.19&  17.52&  12.73&   8.90&   0.00&   0.90&   0.33&   0.00&   0.00 \\ 
 101& 084918.888+462252.58& 100.80&   0.00& 175.10& 352.90& 298.50& 233.60& 186.50&   0.00& 104.80&  72.01&  34.46&   6.41&   1.94&   0.56&   0.13 \\ 
 102& 085021.089+355705.80&   0.00&   0.00&  28.89&  52.30&  51.34&  43.51&  36.49&   0.00&  22.50&  14.44&   9.45&   1.58&   0.64&   0.27&   0.00 \\ 
 103& 085030.449+115410.58&  10.80&  14.76&  16.13&  32.78&  32.91&  25.41&  19.86&   0.00&  16.99&   0.00&   5.69&   1.11&   0.43&   0.00&   0.00 \\ 
 104& 085210.860+271031.44&   0.00&   5.41&   8.58&  19.45&  28.15&  24.66&  21.07&  15.44&  13.33&   9.26&   5.48&   1.19&   0.49&   0.00&   0.00 \\ 
 105& 085230.000+230223.79&   4.63&  10.78&  17.18&  39.01&  45.70&  39.79&  34.81&   0.00&  23.72&  13.75&   9.06&   1.84&   0.64&   0.00&   0.00 \\ 
 106& 085233.876+355124.37&   0.00&   0.00&  19.18&  47.70&  48.87&  41.33&  34.44&   0.00&  25.64&  16.26&   9.24&   1.59&   0.57&   0.09&   0.00 \\ 
 107& 085336.605+164311.67&  56.64&  50.00&  43.95&  80.57&  78.96&  64.99&  52.19&   0.00&  34.89&  21.96&  13.20&   2.41&   0.88&   0.34&   0.00 \\ 
 108& 085812.391+480829.41&   0.00&   0.00&  28.24&  52.49&  52.12&  40.69&  31.51&   0.00&  15.38&  12.35&   6.08&   1.27&   0.48&   0.22&   0.00 \\ 
 109& 085958.872+590832.95&   0.00&   3.31&   6.96&  20.59&  34.37&  31.82&  26.46&   0.00&  16.99&  14.58&   9.51&   1.76&   0.71&   0.11&   0.00 \\ 
 110& 090005.244+131707.45&   0.00&   6.13&   3.93&   6.60&  11.78&   8.58&   7.02&   0.00&   0.00&   0.00&   0.00&   0.59&   0.24&   0.00&   0.00 \\ 
 111& 090008.556+205039.80&   5.35&  14.74&  36.75&  79.12&  80.73&  69.02&  59.90&   0.00&  33.49&  23.78&  12.78&   2.75&   0.96&   0.26&   0.27 \\ 
 112& 090255.800+325546.56&   0.00&  14.60&  14.10&  38.94&  39.54&  33.23&  27.44&   0.00&  16.93&  14.35&   6.26&   1.37&   0.51&   0.37&   0.31 \\ 
 113& 090424.900+535614.06&   0.00&   3.45&  12.49&  31.01&  33.89&  28.15&  23.28&   0.00&  14.86&   7.26&   5.64&   1.29&   0.43&   0.27&   0.16 \\ 
 114& 090601.090+073423.79&   0.00&  23.36&  34.48&  68.14&  60.21&  46.73&  36.94&  34.14&  25.27&  16.80&   9.13&   1.94&   0.68&   0.09&   0.00 \\ 
 115& 090619.932+522150.00&   3.72&   6.78&  13.60&  29.54&  29.08&  22.68&  18.30&   0.00&  14.18&   7.39&   3.82&   0.85&   0.28&   0.00&   0.00 \\ 
 116& 090621.408+274319.04&   0.00&   6.29&  12.46&  29.29&  36.78&  32.09&  29.06&   0.00&  22.35&  12.43&   7.30&   1.63&   0.60&   0.00&   0.00 \\ 
 117& 090645.792+432817.31&   0.00&  15.22&  15.80&  35.56&  38.91&  31.93&  23.77&   0.00&  17.86&   9.25&   5.84&   1.28&   0.51&   0.07&   0.00 \\ 
 118& 090747.448+295159.44&   0.00&   2.35&   9.48&  24.33&  31.39&  27.65&  23.58&  19.66&  15.46&  10.74&   6.42&   1.26&   0.49&   0.00&   0.00 \\ 
 119& 090811.400+262658.69&  29.34&  74.26&  68.17& 131.20& 107.70&  81.94&  65.94&   0.00&  39.34&  24.57&  12.91&   2.83&   0.93&   0.45&   0.43 \\ 
 120& 091140.692+274111.15&   0.00&  41.00&  39.14&  83.23&  89.13&  74.82&  60.33&   0.00&  38.99&  25.59&  15.50&   3.04&   1.11&   0.17&   0.00 \\ 
 121& 091158.819+152433.52&   0.00&   7.56&   7.56&  17.89&  24.18&  21.89&  19.43&   0.00&  15.31&  10.96&   4.81&   1.07&   0.37&   0.00&   0.19 \\ 
 122& 091227.782+534222.95&   0.00&  37.87&  24.46&  49.37&  52.97&  41.19&  33.32&   0.00&  31.90&  18.30&  14.28&   2.12&   0.84&   0.18&   0.00 \\ 
 123& 091318.257+492556.36&  49.20&  80.86&  48.86&  46.36&  46.74&  33.31&  25.38&   0.00&  19.21&  13.45&   6.93&   1.76&   0.76&   0.32&   0.14 \\ 
 124& 091338.633+334627.93&   0.00&  22.15&  18.56&  32.80&  43.99&  34.27&  28.37&   0.00&  18.32&   9.70&   9.60&   1.68&   0.73&   0.30&   0.00 \\ 
 125& 091411.227+091136.07&   0.00&  11.68&  59.97&  70.59&  64.49&  53.80&  41.97&  35.84&  28.35&  18.59&   9.21&   1.95&   0.69&   0.08&   0.00 \\ 
 126& 091606.929+170000.77&   0.00&  10.32&  19.97&  41.72&  46.24&  37.10&  30.71&   0.00&  15.78&   5.92&   4.13&   1.35&   0.51&   0.08&   0.00 \\ 
 127& 091618.096+315807.69&   0.00&   0.00&  11.95&  35.90&  52.42&  43.01&  34.90&  25.34&  21.30&  13.85&   8.08&   1.87&   0.71&   0.16&   0.18 \\ 
 128& 092006.437+015807.65&   0.00& 393.20& 201.40& 355.00& 318.20& 249.40& 193.70& 144.90& 116.30&  75.46&  35.13&   7.38&   2.51&   1.16&   0.54 \\ 
 129& 092023.182+394039.10&   0.00&   2.88&  14.77&  35.25&  37.38&  32.53&  27.44&   0.00&  13.32&  11.01&   5.71&   1.20&   0.38&   0.10&   0.00 \\ 
 130& 092252.289+155754.77&   0.00&   0.00&  26.82&  53.52&  49.12&  37.82&  30.68&   0.00&  21.37&  13.12&   6.42&   1.42&   0.53&   0.00&   0.00 \\ 
 131& 092316.298+311429.66&  27.98&  40.87&  22.90&  26.07&  32.29&  23.52&  17.26&  21.15&  15.27&  10.06&   6.36&   1.86&   0.78&   0.08&   0.00 \\ 
 132& 092420.102+031454.70&   0.00&   0.00&  20.24&  51.61&  62.24&  54.22&  47.47&  41.35&  34.79&  23.63&   9.64&   3.50&   1.45&   0.91&   0.24 \\ 
 133& 092438.057+133134.95&  14.97&  14.88&  27.83&  47.44&  61.61&  55.21&  48.40&   0.00&  28.43&  22.26&  10.50&   2.55&   0.97&   0.35&   0.00 \\ 
 134& 092503.821+404602.82&   0.00&   0.00&   0.00&  26.11&  30.23&  22.92&   0.00&   0.00&  13.24&   6.70&   4.50&   0.79&   0.30&   0.00&   0.00 \\ 
 135& 092539.823+600729.85&   0.00&  11.00&  20.02&  41.63&  44.84&  37.11&  30.11&   0.00&  19.66&  13.54&   6.87&   1.46&   0.57&   0.12&   0.00 \\ 
 136& 092610.469+054710.10&   0.00&   0.00&   9.94&   8.70&  21.83&  20.63&  18.35&  13.66&  13.78&   8.57&   5.79&   1.52&   0.60&   0.12&   0.00 \\ 
 137& 092637.212+532550.96&   0.00&   0.00&  19.66&  40.50&  45.59&  40.09&  34.50&   0.00&  19.73&  11.62&   6.87&   1.53&   0.60&   0.19&   0.00 \\ 
 138& 092657.689+423136.63&  94.21& 140.10&  96.89& 150.70& 129.30& 103.20&  84.67&   0.00&  51.62&  37.04&  18.43&   3.50&   1.18&   0.31&   0.37 \\ 
 139& 092717.047+262344.70&   0.00&   0.00&  11.98&  20.29&  26.72&  23.30&  19.87&   0.00&  15.46&   5.12&   5.85&   1.21&   0.52&   0.15&   0.00 \\ 
 140& 092823.455+454806.45&   0.00&   0.00&  16.46&  27.20&  37.14&  31.62&  26.45&   0.00&  15.44&   9.62&   6.98&   1.47&   0.62&   0.00&   0.00 \\ 
 141& 092952.692+062528.69&  95.07&  79.41&  16.99&  24.89&  24.58&  16.33&  12.04&  19.34&  13.19&   7.56&   4.08&   1.16&   0.58&   0.30&   0.30 \\ 
 142& 093057.662+244822.79&   0.00&  12.94&  27.28&  60.94&  62.54&  51.45&  43.58&   0.00&  28.55&  20.31&  10.98&   2.14&   0.74&   0.17&   0.00 \\ 
 143& 093123.995+441857.32&   0.00&  13.85&  17.08&  36.75&  38.39&  31.41&  25.60&   0.00&  17.40&  12.81&   5.10&   1.51&   0.58&   0.19&   0.00 \\ 
 144& 093223.952+180303.80&   0.00&  30.31&  52.21& 112.10& 114.90&  94.88&  78.39&   0.00&  44.95&  27.25&  16.87&   3.67&   1.36&   0.60&   0.17 \\ 
 145& 093225.889+603346.86&   0.00&  36.58&  76.98& 171.40& 189.80& 162.70& 141.50&   0.00&  83.75&  53.23&  29.40&   6.24&   2.12&   0.41&   0.10 \\ 
 146& 093258.555+103152.14&   0.00&  16.09&  19.13&  45.05&  45.35&  36.91&  29.54&  23.92&  19.13&  10.63&   6.72&   1.28&   0.53&   0.09&   0.00 \\ 
 147& 093401.978+131236.15&   0.00&   0.00&   7.68&  22.96&  30.27&  25.60&  20.12&   0.00&  12.35&   9.34&   5.66&   0.95&   0.43&   0.18&   0.22 \\ 
 148& 093414.381+480456.26&   0.00&   9.84&   9.26&  28.74&  28.92&  23.87&  18.47&   0.00&  12.08&   9.09&   3.26&   0.77&   0.29&   0.00&   0.00 \\ 
 149& 093609.132+532855.40&   0.00&   6.77&  10.11&  31.82&  42.33&  36.90&  29.64&   0.00&  24.01&  14.81&   9.06&   1.51&   0.62&   0.14&   0.08 \\ 
 150& 093713.886+323453.77&  54.78&  56.37&  12.08&  68.14&  64.50&  53.21&  35.49&  35.73&  26.68&   9.22&   3.38&   2.47&   1.05&   1.11&   0.27 \\ 
 151& 093842.905+000148.68&  16.01&  26.91&  64.12& 142.70& 147.20& 125.10& 106.60&  86.51&  64.47&  44.38&  21.24&   4.40&   1.54&   0.45&   0.00 \\ 
 152& 093948.094+340556.40&   0.00&  21.70&  25.54&  48.23&  49.08&  39.09&  33.45&  22.26&  17.18&  11.64&   6.55&   1.32&   0.51&   0.13&   0.00 \\ 
 153& 093956.566+235922.67&   0.00&  85.41& 142.80& 315.60& 322.20& 270.10& 223.60&   0.00& 131.10&  89.38&  43.31&   8.21&   2.61&   0.72&   0.15 \\ 
 154& 094039.792+144551.47&   0.00&  12.25&  21.55&  43.44&  40.91&  32.57&  26.52&   0.00&  17.75&  14.12&   6.16&   1.25&   0.43&   0.00&   0.00 \\ 
 155& 094055.862+400715.19&   0.00&   0.00&  26.18&  44.03&  48.92&  35.32&  28.52&   0.00&  14.80&   9.94&   5.64&   1.40&   0.54&   0.16&   0.00 \\ 
 156& 094140.699+212102.49&   0.00&   0.00&   7.22&  21.52&  25.45&  21.47&  16.47&   0.00&  14.12&   7.04&   5.21&   1.07&   0.43&   0.08&   0.00 \\ 
 157& 094209.310+130553.84&   7.75&  17.72&  46.98& 133.40& 167.30& 152.70& 135.30&   0.00&  84.29&  54.42&  34.23&   5.77&   2.02&   0.22&   0.00 \\ 
 158& 094320.914+371132.22&   0.00&   3.79&   9.09&  23.20&  30.95&  27.71&  24.55&   0.00&  17.63&  10.72&   6.34&   1.38&   0.54&   0.12&   0.00 \\ 
 159& 094347.544+020557.95&   0.00&   0.00&  15.86&  30.02&  33.89&  29.38&  24.65&  21.87&  15.60&  11.31&   5.47&   1.47&   1.29&   0.79&   0.40 \\ 
 160& 094353.873+125512.47&   0.00&  12.60&   9.81&  17.75&  27.49&  24.43&  21.44&   0.00&  11.87&  11.40&   7.62&   1.63&   0.65&   0.23&   0.21 \\ 
 161& 094514.155+115124.29&   0.00&   0.00&  15.57&  36.08&  44.71&  38.30&  32.23&   0.00&  22.03&  17.19&   8.42&   1.72&   0.61&   0.00&   0.00 \\ 
 162& 094555.742+104542.90&   0.00&   3.89&  13.85&  31.09&  37.37&  32.82&  29.56&  26.46&  20.99&  13.74&   7.28&   1.56&   0.54&   0.00&   0.00 \\ 
 163& 094604.426+185641.15&   0.00& 159.60& 206.70& 406.60& 359.70& 290.50& 230.80&   0.00& 147.70&  94.44&  56.33&  11.59&   4.83&   5.01&   6.75 \\ 
 164& 094659.530+225207.47&   0.00&   0.00&   7.81&  17.76&  26.39&  24.10&  20.50&   0.00&  13.13&   7.16&   6.39&   1.20&   0.50&   0.10&   0.00 \\ 
 165& 094701.490+600720.12&  45.39&  35.63&  30.66&  57.50&  52.23&  41.83&  32.23&   0.00&  12.63&  12.07&   6.82&   1.40&   0.50&   0.30&   0.17 \\ 
 166& 094704.462+543044.40&   0.00&   0.00&   7.88&  19.65&  22.88&  21.56&  19.87&   0.00&  11.13&  10.08&   0.00&   0.63&   0.16&   0.00&   0.00 \\ 
 167& 094744.465+405914.72&   0.00&  31.91&  32.82&  58.87&  64.01&  53.73&  42.39&   0.00&  20.52&  13.01&   9.78&   1.70&   0.63&   0.22&   0.00 \\ 
 168& 094818.677+023004.16&   0.00&  13.06&  38.61&  94.85& 103.70&  89.77&  77.55&  65.29&  53.42&  36.56&  17.12&   3.73&   1.37&   0.74&   0.87 \\ 
 169& 094915.845+204412.77&  16.86&  36.58&  63.99& 146.30& 153.10& 132.80& 110.10&   0.00&  73.77&  47.83&  27.43&   3.40&   1.05&   0.00&   0.00 \\ 
 170& 094952.824-002104.82&   0.00&   3.74&   8.25&  20.04&  28.45&  24.98&  21.51&  17.21&  14.04&  10.87&   6.24&   1.20&   0.46&   0.00&   0.00 \\ 
 171& 095006.482+163106.02&   0.00&   0.00&   0.00&   0.00&  22.18&  19.31&   0.00&   0.00&  15.58&  10.15&   7.05&   1.19&   0.51&   0.00&   0.00 \\ 
 172& 095053.155+091931.49&   0.00&  12.37&  14.12&  29.50&  32.56&  26.95&  23.60&  18.32&  13.79&   8.53&   5.04&   1.04&   0.42&   0.09&   0.00 \\ 
 173& 095136.689+284458.12&   0.00&   2.96&  10.54&  29.20&  33.13&  27.99&  22.46&   0.00&  16.87&  11.17&   6.73&   1.37&   0.50&   0.09&   0.00 \\ 
 174& 095224.634+641657.66& 142.20& 101.70&  38.84&  68.54&  70.59&  55.28&  39.69&   0.00&   0.00&   0.00&   0.00&   0.80&   0.30&   0.20&   0.00 \\ 
 175& 095336.144+292543.28&  18.02&  30.64&  23.78&  41.23&  38.30&  29.39&  23.17&   0.00&  14.09&   8.34&   5.04&   1.17&   0.45&   0.12&   0.00 \\ 
 176& 095531.781+445733.97&   0.00&  11.16&  18.11&  36.97&  43.97&  37.17&  29.09&   0.00&  17.96&  12.57&   8.52&   1.52&   0.61&   0.18&   0.00 \\ 
 177& 095636.199+543220.94&   0.00&   0.00&  14.52&  19.81&  30.06&  22.48&  16.85&   0.00&   9.93&   7.96&   5.15&   0.99&   0.34&   0.00&   0.00 \\ 
 178& 095729.906+024942.07&   1.96&   6.61&   9.35&  24.14&  32.15&  27.80&  23.96&  18.34&  15.35&   9.77&   6.54&   1.35&   0.55&   0.00&   0.00 \\ 
 179& 095824.622+003203.16&  19.76&   0.00&  21.53&  46.81&  44.17&  36.30&  29.37&  23.87&  18.08&  13.81&   6.12&   1.43&   0.46&   0.08&   0.00 \\ 
 180& 095842.643+631845.50&   0.00&  19.61&  21.12&  48.97&  58.80&  48.91&  38.72&   0.00&  22.21&  14.88&   8.70&   1.93&   0.81&   0.00&   0.00 \\ 
 181& 095851.290+075910.25&   0.00&   1.65&   5.36&  14.39&  23.37&  20.81&  18.56&  15.09&  12.15&  10.29&   5.33&   1.15&   0.42&   0.00&   0.00 \\ 
 182& 100027.310+104928.02&   0.00&   0.00&  15.19&  33.71&  43.67&  37.44&  32.51&   0.00&  21.33&  14.79&   7.96&   1.56&   0.54&   0.00&   0.00 \\ 
 183& 100031.169+375759.06&   0.00&   8.39&  14.88&  36.47&  47.24&  40.83&  33.69&   0.00&  22.68&  16.42&   8.01&   2.06&   0.84&   0.25&   0.00 \\ 
 184& 100111.930+192933.52&   0.00&   0.00&  10.41&  28.81&  41.46&  36.97&  30.22&   0.00&  19.69&  15.80&   7.55&   1.75&   0.68&   0.00&   0.00 \\ 
 185& 100113.642+092859.67&   0.00&   0.00&   9.95&  19.45&  22.12&  18.32&  16.60&  11.70&   0.00&   6.58&   3.49&   0.49&   0.16&   0.00&   0.00 \\ 
 186& 100402.383+550647.40&   0.00&   6.86&  14.01&  34.97&  35.87&  29.46&  23.94&   0.00&  12.24&  10.28&   5.50&   1.10&   0.38&   0.10&   0.00 \\ 
 187& 100409.672+355646.11&   0.00&   4.15&   7.86&  19.86&  24.98&  22.44&  19.99&   0.00&  12.80&   8.15&   4.30&   0.94&   0.35&   0.00&   0.00 \\ 
 188& 100522.452+072728.30&   0.00&  14.58&  31.99&  85.82& 104.20&  82.65&   0.00&  46.52&  27.76&  20.33&   7.92&   1.71&   0.54&   0.00&   0.00 \\ 
 189& 100529.796+291645.33&   0.00&   7.17&   7.88&  19.63&  25.04&  23.16&  20.48&   0.00&  14.08&   6.52&   5.14&   1.00&   0.32&   0.08&   0.00 \\ 
 190& 100618.310+194131.66&   0.00&   5.27&  10.23&  24.13&  28.16&  23.31&  19.89&   0.00&  13.02&   7.48&   4.33&   0.99&   0.41&   0.00&   0.00 \\ 
 191& 100626.726+520906.04&   0.00&  26.03&  19.02&  38.33&  35.65&  29.51&  22.08&   0.00&  15.84&   9.82&   6.06&   0.99&   0.39&   0.30&   0.31 \\ 
 192& 100650.868+014133.99&   0.00&   4.51&  23.10&  46.12&  46.52&  40.24&  34.30&  25.75&  20.40&  14.48&   6.01&   1.76&   0.61&   0.00&   0.00 \\ 
 193& 100743.618+554934.54&   0.00&  41.47&  80.32& 192.20& 189.40& 160.90& 131.20&   0.00&  78.14&  51.97&  27.59&   5.42&   1.61&   0.23&   0.11 \\ 
 194& 100752.675+291104.78&   0.00&   0.00&   6.88&  10.71&  18.84&  14.54&  11.94&   0.00&   0.00&   0.00&   0.00&   0.70&   0.30&   0.14&   0.00 \\ 
 195& 100755.092+392139.13&   0.00&   0.00&   5.74&  24.93&  36.93&  31.77&  26.54&   0.00&  18.37&  11.71&   8.54&   1.49&   0.62&   0.07&   0.00 \\ 
 196& 100907.284-000157.86&   0.00&   0.00&  22.67&  48.39&  47.71&  43.29&  35.49&  27.47&  21.83&  16.07&   7.74&   1.64&   0.55&   0.26&   0.00 \\ 
 197& 100918.542+374228.31&   0.00&   4.25&   7.74&  24.40&  37.98&  34.64&  32.75&   0.00&  22.73&  13.56&  11.12&   1.64&   0.69&   0.11&   0.00 \\ 
 198& 101004.738+183613.74&   0.00&  17.21&  20.10&  53.35&  58.30&  47.01&  37.97&   0.00&  27.22&  16.04&   8.87&   1.96&   0.73&   0.07&   0.00 \\ 
 199& 101009.833+145732.15&   0.00&   6.17&   6.39&  18.65&  23.21&  19.69&  16.30&   0.00&  14.50&  10.49&   7.00&   1.07&   0.43&   0.11&   0.00 \\ 
 200& 101108.878+614156.53&   0.00&  10.31&  12.33&  30.89&  32.28&  27.37&  20.47&   0.00&  12.78&   9.32&   4.72&   1.05&   0.42&   0.15&   0.00 \\ 
 201& 101241.698+641102.30&  63.03&  27.73&  25.48&  50.10&  48.79&  40.96&  32.37&   0.00&  19.64&  13.26&   8.51&   1.53&   0.54&   0.11&   0.00 \\ 
 202& 101342.775+125135.28&   0.00&   0.00&  40.03&  88.15&  85.44&  69.62&  57.25&  47.93&  37.23&  20.60&  14.07&   3.00&   1.42&   0.88&   0.96 \\ 
 203& 101437.649+010926.79&   0.00&   7.20&  18.58&  48.44&  55.22&  48.11&  41.64&  35.07&  27.09&  19.60&  10.34&   2.27&   0.87&   0.00&   0.00 \\ 
 204& 101519.687+010341.63&   0.00&  24.93&  23.89&  41.59&  49.25&  40.88&  32.45&  27.66&  15.77&  14.83&   8.47&   1.76&   0.65&   0.00&   0.00 \\ 
 205& 101624.362+580136.72&   0.00&  29.31&  32.97&  63.97&  70.90&  59.90&  48.46&   0.00&  25.02&  16.96&  10.55&   2.28&   0.96&   0.47&   0.00 \\ 
 206& 101629.210-000137.12&   0.00&   0.00&  25.51&  49.19&  43.69&  36.60&  28.76&  25.30&  19.83&  13.89&   7.31&   1.49&   0.52&   0.59&   0.21 \\ 
 207& 101658.481+282425.47&   0.00&   0.00&  15.28&  37.50&  45.30&  39.34&  34.45&   0.00&  24.92&  15.28&   9.63&   1.71&   0.60&   0.11&   0.00 \\ 
 208& 101906.120+192100.31&   0.00&   0.00&  11.25&  27.07&  23.30&  19.17&  11.15&   0.00&   0.00&   0.00&   0.00&   0.51&   0.11&   0.00&   0.00 \\ 
 209& 102000.211+081333.81&   0.00& 125.40& 136.00& 287.90& 258.30& 216.50& 170.80& 129.70&  91.53&  62.36&  28.41&   6.11&   2.50&   3.87&  12.96 \\ 
 210& 102054.334+100624.00&  28.11&  28.56&  38.12&  82.87&  90.27&  78.59&  67.47&  47.78&  38.00&  27.16&  17.94&   3.45&   1.19&   0.28&   0.15 \\ 
 211& 102103.542+304108.90& 144.80& 131.80&  65.73&  89.54&  77.14&  57.01&  42.97&   0.00&  28.43&  16.50&  11.29&   1.99&   0.73&   0.22&   0.00 \\ 
 212& 102200.787+220947.44&  95.29& 126.20& 116.90& 230.70& 206.70& 162.90& 130.30&   0.00&  79.39&  53.38&  29.59&   6.12&   2.20&   1.14&   0.43 \\ 
 213& 102206.982+201009.31&   0.00&   0.00&  15.78&  36.84&  36.92&  29.78&  23.73&   0.00&  13.30&  12.47&   5.83&   1.15&   0.39&   0.08&   0.00 \\ 
 214& 102518.962+131918.06&   0.00&   9.13&  11.78&  27.71&  28.20&  23.59&  20.28&  16.29&  11.95&   8.51&   4.02&   0.96&   0.33&   0.00&   0.00 \\ 
 215& 102544.676+025824.45&   0.00&  36.74&  18.58&  29.77&  33.37&  28.88&  25.21&  18.94&  16.88&  11.14&   6.29&   1.30&   0.57&   0.23&   0.00 \\ 
 216& 102552.646+043949.59&  30.60&  58.69&  47.70&  93.73&  90.32&  72.76&  57.95&  45.82&  35.64&  24.80&  12.45&   2.88&   1.17&   0.33&   0.00 \\ 
 217& 102607.469+562330.00&   0.00&  12.55&  22.00&  44.69&  45.78&  37.10&  28.58&   0.00&  16.39&   8.59&   6.32&   1.29&   0.52&   0.12&   0.00 \\ 
 218& 102724.199+370421.02&   0.00&   0.00&  34.30&  61.42&  50.61&  39.52&  31.79&   0.00&  14.67&   8.67&   3.27&   1.07&   0.36&   0.34&   0.00 \\ 
 219& 102808.544+294933.32&   0.00&  10.48&  18.23&  41.29&  40.21&  33.02&  27.47&   0.00&  15.03&   9.09&   5.04&   1.10&   0.37&   0.10&   0.12 \\ 
 220& 102812.180+121501.90&  63.35&  42.08&  33.73&  77.15&  86.98&  73.16&  55.32&   0.00&  38.16&  23.18&  12.21&   2.46&   0.96&   0.24&   0.00 \\ 
 221& 102842.110+031129.41&   0.00&   6.54&   7.73&  19.32&  28.24&  23.95&  19.79&  14.90&  12.52&   8.74&   5.70&   1.25&   0.49&   0.00&   0.00 \\ 
 222& 102856.978+450910.94&   0.00&   0.00&  10.63&  25.20&  27.86&  23.39&  19.74&   0.00&  14.99&   6.88&   4.86&   1.08&   0.46&   0.11&   0.00 \\ 
 223& 102925.404+122244.89&   0.00&   8.55&   8.73&  19.86&  25.18&  21.45&  19.12&  14.58&  12.25&   8.27&   4.87&   0.95&   0.34&   0.09&   0.00 \\ 
 224& 103000.478+205517.53&   0.00&  12.46&  24.91&  52.43&  56.84&  49.13&  42.84&   0.00&  29.83&  15.95&   8.47&   1.94&   0.71&   0.11&   0.00 \\ 
 225& 103138.582+112816.84&   0.00&   0.00&  43.09&  51.57&  58.34&  49.60&  44.13&  37.38&  33.07&  23.99&  13.26&   2.89&   1.14&   0.32&   0.00 \\ 
 226& 103320.513+243559.14&   0.00&   9.39&  11.24&  25.73&  33.32&  26.99&  21.00&   0.00&  15.13&   8.19&   5.06&   1.18&   0.48&   0.10&   0.00 \\ 
 227& 103618.626+054409.41&   2.98&   5.84&   7.75&  19.01&  27.25&  24.25&  20.27&  17.88&  15.08&  11.58&   6.33&   1.39&   0.58&   0.00&   0.00 \\ 
 228& 103748.274+115342.67&   0.00&   8.46&  23.45&  56.48&  57.05&  46.97&  39.01&  31.12&  25.19&  17.67&   8.28&   1.97&   0.70&   0.16&   0.00 \\ 
 229& 103811.402+153514.61&   2.64&   7.59&  10.38&  27.78&  30.01&  24.56&  21.73&   0.00&  11.63&   9.69&   5.54&   1.01&   0.38&   0.00&   0.00 \\ 
 230& 103826.587+182331.09&  12.27&  36.15&  76.22& 167.10& 157.50& 130.50& 110.20&   0.00&  71.30&  43.30&  21.81&   4.70&   1.52&   0.27&   0.26 \\ 
 231& 103928.058+011242.06&   0.00&   5.98&   8.58&  21.95&  23.45&  19.35&  15.49&  18.17&  14.10&   9.71&   4.30&   1.43&   0.49&   0.00&   0.00 \\ 
 232& 103934.512+060425.00&   0.00&   0.00&  15.25&  38.92&  45.36&  37.95&  31.74&  25.21&  21.03&  15.15&   8.02&   1.88&   0.75&   0.10&   0.00 \\ 
 233& 104033.662+373627.14&   0.00&   0.00&  13.73&  41.16&  51.23&  44.43&  35.11&   0.00&  22.95&  12.75&   9.01&   1.92&   0.77&   0.08&   0.00 \\ 
 234& 104128.630+371545.82&   0.00&  45.52&  74.06& 134.80& 127.00& 103.00&  81.90&   0.00&  28.21&  15.17&   8.02&   1.80&   0.57&   0.21&   0.00 \\ 
 235& 104144.486+191405.27&   0.00&  29.05&  22.72&  40.39&  40.24&  31.35&  24.44&   0.00&  15.47&   8.30&   6.09&   1.18&   0.46&   0.00&   0.00 \\ 
 236& 104152.382+522444.82&   0.00&   5.94&   4.07&  17.95&  29.55&  25.11&  21.30&   0.00&  11.88&   8.85&   6.79&   0.00&   0.00&   0.00&   0.00 \\ 
 237& 104204.135+293323.41&   0.00&  19.75&  65.47& 157.40& 155.70& 130.00& 110.00&   0.00&  71.12&  47.77&  23.67&   4.92&   1.49&   0.20&   0.00 \\ 
 238& 104215.170+140636.31&   0.00&  48.99&  73.68& 151.00& 136.70& 110.80&  90.70&  72.80&  54.54&  39.56&  17.43&   3.60&   1.18&   0.18&   0.00 \\ 
 239& 104218.238+370756.34&   0.00&  41.03&  36.88&  65.71&  66.74&  55.43&  49.70&   0.00&  35.87&  21.61&  14.81&   2.85&   1.15&   0.52&   0.13 \\ 
 240& 104220.143+564855.80&  24.86&  61.08&  80.99& 204.20& 218.30& 187.10& 151.00&   0.00& 106.20&  62.86&  37.71&   6.91&   2.25&   0.49&   0.18 \\ 
 241& 104230.550+003442.00&   0.00&  16.71&  35.21&  84.01&  78.84&  64.87&  52.76&  41.88&  32.37&  22.64&  11.66&   2.61&   0.95&   0.43&   0.36 \\ 
 242& 104349.877+420923.41&   0.00&  28.44&  25.12&  45.17&  53.61&  42.49&  32.85&   0.00&  24.13&  15.00&   8.69&   1.96&   0.77&   0.08&   0.00 \\ 
 243& 104410.435+394908.57&   0.00&  23.42&  26.66&  58.42&  53.88&  42.02&  34.93&   0.00&  22.48&  10.36&   6.17&   1.34&   0.48&   0.00&   0.00 \\ 
 244& 104619.330+071452.32&   0.00&  38.30&  20.31&  34.39&  35.59&  29.48&  23.21&  19.63&  16.18&  11.75&   6.90&   1.37&   0.46&   0.00&   0.00 \\ 
 245& 104655.553+150742.25&   0.00&   7.48&  14.51&  34.64&  35.27&  29.09&  21.79&  18.97&  14.12&   9.40&   4.45&   1.09&   0.38&   0.00&   0.00 \\ 
 246& 104710.562+180217.20&   0.00&  18.40&  19.33&  45.21&  47.06&  39.95&  34.25&   0.00&  22.74&  16.18&   8.29&   1.70&   0.56&   0.15&   0.16 \\ 
 247& 104902.102+443556.87&  58.63&  55.54&  40.98&  61.10&  50.14&  39.49&  30.56&   0.00&  15.88&  11.03&   2.84&   1.12&   0.36&   0.26&   0.00 \\ 
 248& 104933.866+323911.15&  40.61&  28.35&  25.57&  44.61&  41.69&  34.28&  29.69&   0.00&  19.71&  10.27&   6.96&   1.34&   0.46&   0.07&   0.00 \\ 
 249& 104935.983+132235.39&   0.00&  27.89&  45.20&  59.66&  60.06&  44.54&  34.18&  25.52&  19.77&  12.94&   6.94&   1.52&   0.65&   0.37&   0.00 \\ 
 250& 104953.318+564551.33&   4.52&   9.30&   8.59&  26.85&  32.12&  28.29&  24.50&   0.00&  16.15&   8.94&   8.73&   1.26&   0.53&   0.11&   0.00 \\ 
 251& 105220.450+054941.59&  37.79&  65.89& 110.00& 254.80& 260.00& 219.60& 175.80& 216.20& 128.60& 118.00&  37.05&   8.62&   2.57&   0.45&   0.40 \\ 
 252& 105228.742+574213.74&  17.28&  21.60&  23.82&  46.06&  51.46&  39.83&  30.29&   0.00&  21.46&   9.02&   6.08&   1.36&   0.54&   0.09&   0.00 \\ 
 253& 105302.563+345739.24&   0.00&  10.01&  17.28&  46.12&  59.79&  52.34&  41.82&   0.00&  24.70&  16.65&  10.95&   2.58&   1.05&   0.13&   0.00 \\ 
 254& 105411.851+082006.31&   0.00&  25.94&   0.00&   0.00&   0.00&   0.00&   0.00&   8.10&  12.32&   3.65&   3.74&   0.53&   0.19&   0.10&   0.00 \\ 
 255& 105435.515+555738.18&   0.00&   0.00&   7.25&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.65&   0.19&   0.00&   0.00 \\ 
 256& 105532.426+135220.27&   0.00&   3.84&   9.88&  21.60&  24.35&  21.00&  18.09&  15.47&  11.28&   8.05&   4.18&   0.93&   0.32&   0.00&   0.00 \\ 
 257& 105555.291+440326.92&   0.00&   0.00&  16.51&  40.13&  39.02&  21.56&  16.34&   0.00&   0.00&   0.00&   0.00&   0.38&   0.09&   0.00&   0.00 \\ 
 258& 105743.939+123539.91&  35.43&  70.45&  80.13& 170.30& 151.00& 114.20&  90.12&  73.98&  56.19&  36.71&  18.67&   4.36&   1.53&   0.13&   0.00 \\ 
 259& 105755.265+334041.54&   0.00&   9.40&  22.07&  53.15&  51.95&  43.53&  34.04&   0.00&  22.72&  14.45&   5.92&   1.48&   0.50&   0.19&   0.11 \\ 
 260& 110100.307+395525.95&   0.00&   0.00&  22.57&  37.26&  46.85&  45.53&  42.00&   0.00&  26.23&  15.47&  10.84&   2.53&   0.97&   0.33&   0.00 \\ 
 261& 110106.809+061552.90&   0.00&   0.00&  15.14&  35.35&  44.69&  38.72&  34.40&  24.39&  19.22&  14.46&   7.81&   1.63&   0.63&   0.15&   0.00 \\ 
 262& 110320.189+544848.12&   0.00&   0.00&  22.67&  42.21&  40.01&  32.27&  23.77&   0.00&  14.34&   5.65&   3.65&   0.91&   0.36&   0.13&   0.00 \\ 
 263& 110322.090+360210.18&   0.00&  12.78&  28.41&  65.37&  76.12&  65.74&  55.99&   0.00&  30.77&  21.11&  12.40&   2.64&   1.01&   0.12&   0.00 \\ 
 264& 110334.481+024220.00&   0.00&  14.49&  16.01&  33.13&  33.27&  27.08&  23.12&  16.69&  13.82&   9.88&   5.00&   1.05&   0.40&   0.00&   0.00 \\ 
 265& 110409.655+441535.77&   0.00&   9.82&   8.30&  21.78&  33.25&  30.84&  23.94&   0.00&  23.12&  12.21&   7.22&   1.57&   0.69&   0.11&   0.00 \\ 
 266& 110520.364+301719.55&   0.00&  62.84&  34.83&  59.59&  54.34&  46.29&  38.18&   0.00&  20.09&  13.44&   6.45&   1.54&   0.56&   0.30&   0.00 \\ 
 267& 110540.706+055954.26&   0.00&  37.69&  86.21& 226.00& 219.20& 181.10& 145.00& 131.50&  95.89&  64.22&  27.09&   7.85&   2.73&   1.25&   0.69 \\ 
 268& 110618.312+493538.77&   0.00&  30.55&  43.41& 116.30& 122.70& 107.30&  92.60&   0.00&  54.92&  34.28&  19.64&   3.56&   1.15&   0.35&   0.00 \\ 
 269& 110618.382+032641.58&   8.83&  13.84&  13.96&  29.64&  33.40&  28.71&  26.13&  17.71&  14.38&   9.90&   5.62&   1.38&   0.59&   0.15&   0.17 \\ 
 270& 110653.736+405736.41&   0.00&  32.08&  40.95&  69.25&  60.06&  46.52&  35.64&   0.00&  20.77&  13.50&   5.28&   1.33&   0.48&   0.11&   0.00 \\ 
 271& 110724.391+361222.55&   0.00&  13.61&  39.98&  97.31&  97.69&  83.26&  69.44&   0.00&  45.20&  31.29&  15.65&   3.32&   1.08&   0.23&   0.00 \\ 
 272& 110752.838+442144.83&   0.00&   4.28&   9.85&  22.02&  23.40&  20.12&  16.57&   0.00&  10.01&   0.00&   0.00&   0.56&   0.20&   0.00&   0.00 \\ 
 273& 110905.542+190615.10&   0.00&  44.33&  69.81& 130.90& 114.60&  90.79&  72.44&   0.00&  42.60&  24.98&  14.17&   3.17&   1.14&   0.29&   0.22 \\ 
 274& 110933.732+221155.81&   0.00&   4.29&  16.54&  40.16&  43.69&  39.09&  32.88&   0.00&  18.95&  10.47&   5.02&   1.36&   0.49&   0.00&   0.00 \\ 
 275& 111002.215+023527.17&   0.00&  67.06&  68.45& 131.80& 112.80&  85.41&  63.92&  43.29&  31.86&  21.41&   9.88&   2.20&   0.76&   0.34&   0.25 \\ 
 276& 111028.634+293239.51&   0.00&   0.00&  12.03&  28.47&  37.20&  32.08&  25.69&   0.00&  15.82&  10.92&   7.91&   1.33&   0.54&   0.08&   0.00 \\ 
 277& 111050.945+005531.00&  41.26&  48.62&  50.97&  83.69&  81.32&  66.76&  56.62&  40.23&  30.33&  20.59&  10.81&   2.27&   0.82&   0.33&   0.16 \\ 
 278& 111053.676+315759.88&   0.00&   0.00&   7.16&  21.39&  25.57&  22.21&  19.88&   0.00&  12.85&   7.79&   0.00&   1.01&   0.37&   0.07&   0.00 \\ 
 279& 111108.081+004048.79&   0.00&  33.24&  33.69&  54.37&  53.44&  41.77&  32.03&  20.65&  16.21&  11.29&   5.73&   0.98&   0.35&   0.07&   0.00 \\ 
 280& 111109.778+044035.33&   0.00&  77.58&  24.78&  86.02&  80.62&  70.99&  54.99&  33.71&  23.36&  17.05&   7.74&   1.29&   0.44&   0.16&   0.00 \\ 
 281& 111155.709+281858.11&   0.00&   5.84&  19.67&  29.21&  26.88&  21.69&  15.42&   0.00&   0.00&   6.59&   0.00&   0.44&   0.17&   0.00&   0.00 \\ 
 282& 111212.624-003628.39&   0.00&  45.17&  44.73&  93.51&  94.71&  79.06&  66.59&  53.16&  39.81&  28.09&  14.25&   3.10&   1.11&   0.25&   0.15 \\ 
 283& 111314.093+322115.41&  87.34&  84.36& 100.00& 160.00& 144.60& 117.40&  92.55&   0.00&  54.24&  29.76&  18.76&   3.93&   1.46&   1.04&   0.32 \\ 
 284& 111327.958-005409.53&   0.00&   8.18&  23.49&  52.69&  53.02&  45.87&  39.74&  33.08&  23.90&  15.86&   7.35&   1.40&   0.35&   0.00&   0.00 \\ 
 285& 111333.060+005001.37&   0.00&   3.46&   8.91&  21.62&  26.15&  22.80&  19.22&  17.04&  13.25&   9.30&   4.85&   1.14&   0.42&   0.00&   0.00 \\ 
 286& 111403.134+533652.86&   0.00&   7.65&  13.11&  26.09&  31.64&  27.43&  23.48&   0.00&  15.50&  10.52&   4.61&   1.30&   0.54&   0.15&   0.10 \\ 
 287& 111441.611+593029.94& 182.50& 182.00&  78.85& 124.80&  98.92&  72.75&  55.57&   0.00&  34.48&  17.42&  13.07&   2.28&   0.84&   0.32&   0.30 \\ 
 288& 111531.320+540946.33&   0.00&   0.00&  14.23&  31.39&  30.53&  24.61&  19.99&   0.00&  13.92&   7.95&   6.51&   0.85&   0.30&   0.09&   0.00 \\ 
 289& 111536.701+302522.15& 204.00& 142.00& 107.40& 160.30& 145.40& 119.90&  80.17&   0.00&  28.27&  16.94&   9.19&   1.56&   0.53&   0.22&   0.00 \\ 
 290& 111658.824+413955.28&  43.06&  30.76&  34.50&  64.84&  64.31&  53.99&  39.64&   0.00&  20.68&  14.65&   7.11&   1.55&   0.53&   0.12&   0.00 \\ 
 291& 111731.195+370239.52&   0.00&  12.82&  30.79&  54.46&  56.73&  47.70&  43.50&   0.00&  24.26&  15.07&   7.97&   1.59&   0.61&   0.00&   0.00 \\ 
 292& 111806.742+183856.35&   6.80&   7.08&  10.94&  25.02&  23.78&  19.99&  17.50&   0.00&  10.31&   5.04&   4.54&   0.77&   0.22&   0.00&   0.00 \\ 
 293& 111849.922+195424.30&  23.13&  22.55&  23.96&  47.14&  52.85&  42.44&  33.93&   0.00&  19.64&  12.40&   8.53&   2.11&   1.10&   0.32&   0.21 \\ 
 294& 111946.435+351803.48&  40.04&  25.57&  28.61&  48.71&  51.10&  42.33&  38.03&   0.00&  24.23&  14.99&   7.70&   1.37&   0.48&   0.07&   0.00 \\ 
 295& 112021.691+353553.94&  55.79&  54.77&  47.03&  81.54&  75.78&  61.40&  50.64&   0.00&  30.06&  16.19&   9.60&   1.91&   0.63&   0.10&   0.00 \\ 
 296& 112202.470+070632.18&  10.71&  25.46&  19.81&  38.43&  48.00&  39.41&  31.97&  22.86&  18.50&  13.72&   7.96&   1.70&   0.65&   0.11&   0.00 \\ 
 297& 112208.234+193236.20&   0.00&  36.24&  84.30& 205.70& 222.70& 193.40& 167.20&   0.00& 131.50&  77.89&  48.13&   8.35&   2.80&   0.35&   0.00 \\ 
 298& 112222.990+484047.58&   0.00&  43.15&  56.16& 124.20& 114.20&  93.13&  75.99&   0.00&  51.88&  31.68&  17.61&   3.40&   1.11&   0.29&   0.17 \\ 
 299& 112223.246+242330.91&   0.00&   0.00&  24.83&  23.86&  40.65&  33.06&  28.81&   0.00&  14.08&   7.95&   8.05&   1.74&   0.72&   0.17&   0.00 \\ 
 300& 112253.614+512030.28&   0.00&  15.21&  42.32&  95.37& 100.10&  86.85&  74.59&   0.00&  47.95&  28.72&  16.18&   2.92&   1.80&   1.82&   1.50 \\ 
 301& 112306.144+020254.77&   8.39&  18.70&  27.64&  62.92&  63.08&  51.17&  41.38&  33.94&  25.13&  16.62&   8.87&   1.83&   0.65&   0.00&   0.19 \\ 
 302& 112333.962+010735.58&   4.02&   3.40&  11.83&  24.72&  28.44&  24.57&  18.09&   0.00&  10.52&   7.27&   3.89&   0.85&   0.24&   0.00&   0.00 \\ 
 303& 112342.204+193816.42&   0.00&  55.25&  90.27& 164.00& 149.90& 120.10&  92.19&   0.00&  52.06&  30.70&  18.34&   4.06&   1.46&   1.14&   0.49 \\ 
 304& 112405.489+140053.82&   0.00&   0.00&  34.25&  41.08&  48.25&  39.20&  33.85&  17.73&  12.98&  11.65&   6.59&   1.45&   0.67&   0.27&   0.00 \\ 
 305& 112415.972+250235.71&   0.00&   0.00&  10.66&  24.63&  30.83&  27.47&  22.82&   0.00&  16.24&   7.61&   6.69&   1.26&   0.52&   0.10&   0.00 \\ 
 306& 112442.454+385909.32&   0.00&  22.30&  29.93&  69.77&  77.36&  65.85&  53.12&   0.00&  34.32&  17.01&  12.15&   2.54&   0.91&   0.12&   0.11 \\ 
 307& 112555.174+004958.76&   4.65&  12.15&  18.19&  39.65&  42.76&  35.31&  26.93&  23.93&  17.06&  11.39&   6.41&   1.51&   0.67&   0.25&   0.00 \\ 
 308& 112611.611+351753.12&  33.33&  65.47&  58.16& 111.30&  98.39&  81.76&  67.26&   0.00&  47.38&  32.15&  15.16&   3.48&   1.15&   1.76&   1.91 \\ 
 309& 112617.110+520457.25&   0.00&  31.16&  34.61&  54.43&  48.09&  39.42&  30.18&   0.00&  19.33&  10.54&   5.14&   1.13&   0.37&   0.23&   0.15 \\ 
 310& 112702.311+083615.05&   0.00&   0.00&   9.15&  21.18&  25.96&  22.84&  19.51&  16.22&  13.26&   9.13&   4.80&   0.96&   0.36&   0.00&   0.00 \\ 
 311& 112737.846+443444.22&   0.00&   0.00&   7.87&  24.57&  27.52&  20.72&  18.35&   0.00&  16.19&   9.24&   6.80&   1.31&   0.56&   0.29&   0.00 \\ 
 312& 112750.220+245202.15&  31.14&   0.00&  96.67& 136.70& 123.50&  96.93&  74.38&   0.00&  51.00&  28.89&  15.77&   3.59&   1.17&   0.26&   0.00 \\ 
 313& 112814.059+575034.54&   0.00&  17.70&  35.41&  83.05&  86.67&  73.69&  64.36&   0.00&  36.50&  24.19&  10.10&   2.53&   0.92&   0.27&   0.00 \\ 
 314& 112844.189+234053.38&   0.00&  32.11&  41.65& 123.60& 119.70&  99.71&  82.15&   0.00&  36.53&  23.34&  13.21&   3.02&   1.15&   0.58&   0.13 \\ 
 315& 112856.294-011722.24&   6.33&   8.31&  11.13&  25.65&  27.67&  23.42&  20.64&  14.31&  12.32&   8.56&   4.36&   0.89&   0.33&   0.00&   0.00 \\ 
 316& 112857.187+475300.95&   0.00&   6.78&  20.01&  49.42&  49.85&  40.88&  33.91&   0.00&  24.41&  14.37&   9.46&   1.69&   0.58&   0.00&   0.00 \\ 
 317& 112911.326+621331.19&   0.00&   0.00&  19.73&  33.96&  43.69&  40.25&  32.99&   0.00&  25.17&  17.49&  11.76&   2.08&   0.81&   0.26&   0.00 \\ 
 318& 112916.368+602853.14&   0.00&  20.93&  56.33& 127.40& 129.10& 104.20&  82.50&   0.00&  51.35&  27.21&  17.26&   3.48&   1.17&   0.33&   0.00 \\ 
 319& 113040.846+562910.04&  24.28&  54.96& 106.20& 245.00& 233.10& 191.30& 157.10&   0.00& 103.50&  65.34&  39.03&   6.94&   2.18&   0.51&   0.32 \\ 
 320& 113042.686+153846.38&   0.00&   9.92&  10.35&  20.66&  34.34&  30.19&  25.67&  22.32&  17.36&  13.54&   8.27&   1.85&   0.69&   0.00&   0.00 \\ 
 321& 113043.870+452939.20&   0.00&  16.12&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00& 118.20&  60.09&  23.86&   5.09&   1.45&   0.13&   0.00 \\ 
 322& 113053.258+111440.79&   0.00&   0.00&   0.00&   4.06&   9.11&   8.54&   7.40&   6.34&   4.53&   4.19&   2.38&   0.55&   0.19&   0.00&   0.00 \\ 
 323& 113104.411+552455.15&   0.00&  12.15&  22.62&  47.82&  44.85&  36.03&  28.87&   0.00&  21.44&  12.84&   6.92&   1.24&   0.43&   0.09&   0.00 \\ 
 324& 113209.343-023551.87&   0.00&   0.00&  36.90&  47.91&  51.54&  45.96&  41.88&   0.00&   0.00&  19.66&  11.02&   1.99&   0.71&   0.25&   0.00 \\ 
 325& 113233.089+142615.93&   0.00&   9.11&  23.75&  48.52&  48.01&  38.63&  30.89&  26.33&  18.23&  12.60&   5.91&   1.22&   0.39&   0.11&   0.00 \\ 
 326& 113338.642+041146.22&   0.00&  19.24&  13.12&  19.29&  29.84&  22.44&  17.50&  12.82&   9.06&   7.33&   4.22&   1.05&   0.35&   0.00&   0.00 \\ 
 327& 113340.646+062001.73&   0.00&   7.04&   0.00&   3.57&   8.47&   7.07&   6.06&   4.43&   3.66&   2.41&   1.59&   0.41&   0.13&   0.00&   0.00 \\ 
 328& 113349.613+020514.98&  17.75&  20.92&  18.04&  39.19&  39.55&  31.17&  25.72&  20.18&  15.23&  10.55&   3.98&   1.26&   0.49&   0.12&   0.00 \\ 
 329& 113351.934+572715.75&   0.00&   5.69&  10.60&  26.26&  30.87&  26.55&  23.16&   0.00&  16.24&   9.35&   6.05&   1.25&   0.49&   0.00&   0.00 \\ 
 330& 113437.522+250301.86&   0.00&   9.86&  19.49&  41.38&  41.44&  33.77&  27.14&   0.00&  17.25&  10.48&   5.24&   1.37&   0.52&   0.11&   0.13 \\ 
 331& 113509.103+360935.21&   0.00&   5.74&   9.93&  22.29&  31.53&  28.49&  25.49&   0.00&  13.82&   9.42&   6.75&   1.28&   0.50&   0.06&   0.00 \\ 
 332& 113753.921+392157.84&  15.30&  13.16&  35.46&  70.59&  78.97&  68.72&  62.36&   0.00&  32.19&  23.50&  14.10&   2.60&   0.94&   0.09&   0.00 \\ 
 333& 113800.526+335556.51&   0.00&   5.33&  12.12&  23.94&  34.80&  30.53&  25.99&   0.00&  21.78&  13.76&   7.66&   1.67&   0.66&   0.00&   0.00 \\ 
 334& 113929.244+235325.53&   0.00&   0.00&  29.90&  58.24&  63.48&  56.31&  48.95&   0.00&  25.38&  15.56&  10.91&   1.79&   0.59&   0.07&   0.00 \\ 
 335& 113941.926+360915.87&   0.00&   0.00&  15.23&  33.19&  35.29&  30.90&  25.45&   0.00&  15.76&  10.45&   7.92&   1.28&   0.48&   0.15&   0.11 \\ 
 336& 114039.694+034534.13&   0.00&   0.00&   4.57&  16.87&  24.09&  21.54&  19.66&  15.32&  11.74&   8.72&   4.83&   1.17&   0.38&   0.00&   0.00 \\ 
 337& 114043.404+265201.48&   0.00&   5.45&  12.24&  28.54&  42.51&  39.22&  34.44&   0.00&  21.16&  14.79&   9.64&   1.99&   0.78&   0.08&   0.00 \\ 
 338& 114056.146+140212.39&   0.00&  14.97&  21.69&  46.75&  44.72&  35.99&  30.26&  25.42&  19.52&  13.27&   6.84&   1.35&   0.45&   0.15&   0.00 \\ 
 339& 114146.169+354628.83&   0.00&   5.52&  16.32&  38.44&  46.13&  40.40&  35.74&   0.00&  25.58&  17.77&  11.02&   2.13&   0.77&   0.10&   0.00 \\ 
 340& 114159.400+265700.06&  25.63&  60.47& 171.70& 382.70& 375.30& 313.90& 262.10&   0.00& 166.90& 109.10&  53.65&   9.75&   3.05&   0.48&   0.20 \\ 
 341& 114315.900+095305.77&   0.00&   8.30&  19.85&  47.37&  49.65&  42.76&  34.55&  25.64&  21.07&  12.32&   7.59&   1.34&   0.50&   0.07&   0.00 \\ 
 342& 114318.211+082127.19&   0.00&   6.41&   9.73&  21.57&  26.13&  22.10&  17.94&  14.89&  12.84&   9.03&   5.23&   1.09&   0.50&   0.00&   0.00 \\ 
 343& 114342.730+511937.87&   0.00&  77.55&  68.68& 133.90& 113.70&  88.44&  65.83&   0.00&  38.46&  21.68&  14.23&   3.01&   1.24&   1.02&   0.33 \\ 
 344& 114407.430+264717.72&   0.00&   0.00&  12.53&  33.86&  38.23&  32.03&  25.80&   0.00&  23.26&  13.37&   6.84&   1.44&   0.48&   0.00&   0.00 \\ 
 345& 114411.018+053735.62&   0.00&   0.00&  22.25&  39.55&  43.38&  36.83&  30.75&  21.40&  17.78&  12.72&   7.80&   1.42&   0.54&   0.16&   0.00 \\ 
 346& 114627.895+201258.75&   0.00&   0.00&  25.69&  65.56&  68.28&  57.48&  46.08&   0.00&  30.11&  18.07&   8.33&   2.17&   0.79&   0.28&   0.13 \\ 
 347& 114657.358+323914.31&   0.00&  35.57&  53.90& 113.00& 102.10&  84.30&  69.51&   0.00&  40.93&  23.84&  12.81&   2.48&   0.80&   0.08&   0.00 \\ 
 348& 114741.110+375938.16&   0.00&  19.38&  19.65&  42.10&  42.44&  35.68&  26.91&   0.00&  16.46&   9.23&   6.37&   1.14&   0.44&   0.16&   0.00 \\ 
 349& 114903.382+245842.99&   0.00&  33.95&  27.85&  56.66&  60.14&  49.28&  41.82&   0.00&  23.64&  16.33&  10.89&   1.95&   0.81&   0.40&   0.00 \\ 
 350& 115037.526+013000.57&   0.00&   0.00&  47.61& 121.40& 115.30&  93.41&  74.90&  63.03&  47.19&  31.72&  15.42&   3.38&   1.21&   0.42&   0.29 \\ 
 351& 115052.982+460448.19&   0.00&   0.00&   9.46&  25.00&  43.40&  41.64&  34.59&   0.00&  20.47&   9.91&  10.70&   2.22&   0.90&   0.05&   0.00 \\ 
 352& 115208.570+481658.37&  16.15&  22.54&  25.59&  51.53&  44.85&  36.14&  28.42&   0.00&  15.58&   6.77&   3.25&   1.15&   0.34&   0.10&   0.10 \\ 
 353& 115225.538-011602.85&   0.00&  39.70&  45.84& 107.90&  98.31&  80.30&  65.59&   0.00&  44.43&  28.46&  16.12&   3.62&   1.34&   0.89&   0.75 \\ 
 354& 115311.890+005030.74&   9.44&   7.44&   6.44&  17.88&  29.44&  27.25&  22.38&   0.00&  15.46&  11.42&   6.74&   1.57&   0.60&   0.11&   0.00 \\ 
 355& 115355.538-031035.27&   0.00&  18.91&  25.12&  51.69&  48.75&  39.02&  30.74&   0.00&  23.80&  11.31&   5.60&   1.27&   0.44&   0.22&   0.00 \\ 
 356& 115431.471+312024.15&   8.01&  15.40&  21.78&  51.17&  56.75&  47.78&  39.12&   0.00&  24.16&  18.61&   9.24&   2.08&   0.77&   0.09&   0.00 \\ 
 357& 115446.094+300830.45&   0.00&   7.97&  11.56&  28.89&  33.52&  28.33&  23.43&   0.00&  17.23&   8.19&   8.68&   1.36&   0.54&   0.19&   0.00 \\ 
 358& 115640.214+583031.94&   0.00&   0.00&  10.14&  32.25&  40.53&  35.13&  28.82&   0.00&  15.69&  11.23&   9.72&   1.64&   0.76&   0.41&   0.30 \\ 
 359& 115730.590+210925.93&   0.00&   6.18&   8.66&  27.46&  30.77&  27.67&  22.67&   0.00&   0.00&   0.00&   0.00&   0.87&   0.30&   0.00&   0.00 \\ 
 360& 115821.650+363820.46&  15.64&  96.83& 153.30& 347.10& 337.30& 283.90& 234.60&   0.00& 147.20&  96.04&  49.71&   9.05&   2.85&   0.41&   0.16 \\ 
 361& 115837.723-021710.95&  34.49&  42.24&  86.21& 180.40& 183.30& 153.80& 133.60&   0.00&  79.30&  54.78&  27.96&   5.26&   1.74&   0.29&   0.19 \\ 
 362& 115931.855+430842.78&   0.00&  11.45&  10.07&  21.15&  33.20&  26.56&  20.01&   0.00&  17.12&  11.85&   6.88&   1.58&   0.61&   0.06&   0.00 \\ 
 363& 115950.669+191523.45&   0.00&   0.00&  15.26&  24.39&  34.19&  31.05&  26.86&   0.00&  13.92&  10.74&   6.75&   1.47&   0.60&   0.14&   0.00 \\ 
 364& 120144.575+375612.04&   0.00&   0.00&  13.40&  21.70&  24.72&  21.74&  18.11&   0.00&  10.19&   0.00&   0.00&   0.75&   0.25&   0.00&   0.00 \\ 
 365& 120222.212+243419.19&   0.00&   0.00&  28.31&  50.01&  50.17&  42.36&  35.34&   0.00&  20.65&  10.38&   6.80&   1.26&   0.41&   0.13&   0.00 \\ 
 366& 120251.859+402448.09&   0.00&  11.71&  26.31&  61.58&  68.90&  57.18&  45.96&   0.00&  28.44&  18.50&  11.03&   2.30&   0.90&   0.15&   0.00 \\ 
 367& 120336.979+604812.24& 163.30&   0.00&   9.90&  35.68&  34.86&  29.60&  21.51&   0.00&  12.61&   6.54&   0.00&   0.85&   0.28&   0.06&   0.00 \\ 
 368& 120353.909+064554.65&   0.00&   0.00&  15.28&  30.82&  29.78&  23.64&  19.21&  14.80&  12.00&   8.20&   4.44&   1.11&   0.46&   0.10&   0.16 \\ 
 369& 120419.075-001855.82&  62.31& 113.30&  86.90& 192.40& 165.80& 122.90&  98.05&   0.00&  77.11&  64.81&  34.30&   6.78&   2.13&   0.31&   0.19 \\ 
 370& 120454.713+001840.08&  92.75& 112.90&  56.05&  96.47&  94.65&  83.88&  55.73&  49.67&  36.88&  25.09&  12.45&   1.47&   0.45&   0.34&   0.00 \\ 
 371& 120541.890+184154.48&   0.00&  15.80&  10.12&  34.97&  37.65&  34.57&  17.73&   0.00&  16.70&  11.56&   4.46&   1.13&   0.46&   0.23&   0.00 \\ 
 372& 120543.690+513741.13&   0.00&   0.00&  19.12&   0.00&  62.46&   0.00&   0.00&   0.00&  22.91&  12.77&   7.53&   1.13&   0.46&   0.31&   0.00 \\ 
 373& 120620.518+245619.89&   0.00&   0.00&  16.08&  34.96&  36.76&  30.37&  26.73&   0.00&  18.58&  11.44&   6.15&   1.19&   0.45&   0.19&   0.23 \\ 
 374& 120627.955+253423.64&   0.00&  62.97&  80.45& 153.10& 140.10& 110.50&  88.04&   0.00&  44.09&  29.94&  14.95&   3.32&   1.18&   0.30&   0.00 \\ 
 375& 120630.811+091855.15&   0.00&   8.98&  13.88&  27.52&  30.62&  24.62&  19.79&  13.63&  11.14&   7.40&   4.31&   0.93&   0.34&   0.00&   0.00 \\ 
 376& 120708.652+065244.84&   0.00&  48.70&  54.23& 102.00& 106.30&  88.14&  70.11&  55.17&  43.68&  29.32&  16.32&   3.51&   1.38&   0.44&   0.17 \\ 
 377& 120811.275+402151.24&   0.00&  14.58&  28.15&  82.98&  93.17&  77.47&  64.80&   0.00&  52.64&  31.23&  20.30&   3.60&   1.21&   0.10&   0.00 \\ 
 378& 121117.789+400715.89&   0.00&  36.66&  20.75&  40.79&  43.23&  34.36&  26.08&   0.00&  15.93&  11.07&   6.97&   1.42&   0.54&   0.14&   0.00 \\ 
 379& 121136.034+142023.25&   0.00&   0.00&  15.83&  26.67&  29.66&  25.09&  20.33&   0.00&  10.47&   6.80&   3.71&   0.78&   0.26&   0.00&   0.00 \\ 
 380& 121258.150+121753.46&   0.00&   0.00&   6.12&  17.93&  24.11&  22.08&  18.55&  15.55&  12.31&   8.20&   5.32&   1.04&   0.40&   0.09&   0.00 \\ 
 381& 121333.026+142900.10&   0.00&   0.00& 277.90& 350.10& 241.80& 179.60& 111.90&  49.57&  38.48&  33.67&  10.65&   1.42&   0.44&   0.16&   0.00 \\ 
 382& 121658.049+262829.45&   0.00&   0.00&  25.76&  58.34&  62.94&  52.15&  46.66&   0.00&  22.82&  17.15&   8.36&   1.85&   0.69&   0.30&   0.14 \\ 
 383& 121702.429+390437.33&   0.00&  32.78&  34.99&  66.79&  61.20&  49.86&  40.06&   0.00&  26.10&  14.94&   6.51&   1.69&   0.59&   0.60&   1.23 \\ 
 384& 121744.033+284912.46&   0.00&  16.93&  21.04&  44.22&  40.85&  32.03&  25.91&   0.00&  17.74&  11.01&   5.13&   1.08&   0.36&   0.14&   0.00 \\ 
 385& 121937.704+435924.54&   0.00&  22.23&  14.32&  33.44&  35.48&  29.98&  25.81&   0.00&  17.70&  14.18&   5.82&   1.26&   0.45&   0.15&   0.00 \\ 
 386& 121937.906+380245.18&   9.14&   0.00&  17.39&  42.08&  40.11&  32.05&  25.83&   0.00&  17.25&  12.37&   3.86&   0.00&   0.00&   0.00&   0.00 \\ 
 387& 122156.458+000948.22&   0.00&  42.15&  52.28& 127.10& 113.80&  88.17&  67.39&  54.21&  40.91&  26.38&  12.90&   3.01&   1.01&   0.51&   0.30 \\ 
 388& 122206.689+113156.10&   4.33&  12.24&  22.51&  53.41&  55.91&  45.73&  37.14&  29.47&  23.45&  17.05&   9.05&   1.98&   0.75&   0.17&   0.00 \\ 
 389& 122240.466+150205.49&  60.81&   0.00&  14.39&  21.33&  16.66&  13.41&  10.00&  10.64&   5.86&   4.41&   2.05&   0.47&   0.17&   0.00&   0.00 \\ 
 390& 122256.134-011247.99&  73.98&  49.80&  13.08&  42.91&  44.08&  41.44&  25.11&  22.53&  15.24&  12.89&   6.57&   1.22&   0.46&   0.20&   0.15 \\ 
 391& 122422.781+213352.28& 194.60& 189.90& 120.10& 234.00& 206.10& 167.40& 129.40&   0.00&  72.82&  41.44&  24.12&   4.88&   1.59&   0.76&   0.16 \\ 
 392& 122424.122+533442.54&   0.00&  11.68&  19.35&  40.00&  48.70&  41.62&  35.62&   0.00&  23.29&  16.96&   9.67&   1.77&   0.73&   0.14&   0.00 \\ 
 393& 122636.197+225953.55&  12.59&  16.56&  19.56&  35.29&  33.51&  27.66&  22.62&   0.00&  16.75&   9.70&   4.51&   1.00&   0.32&   0.00&   0.00 \\ 
 394& 122700.286+295058.69&   1.92&   4.38&   9.74&  22.12&  32.18&  29.27&  25.49&   0.00&  20.81&  12.36&   6.65&   1.63&   0.67&   0.06&   0.00 \\ 
 395& 122718.550-002428.53&   0.00&   0.00&  15.62&  38.92&  42.29&  36.20&  30.98&  26.17&  21.92&  14.58&   7.55&   1.67&   0.57&   0.11&   0.00 \\ 
 396& 122909.250+100435.36&   0.00&   5.12&  14.13&  30.04&  33.02&  28.44&  24.45&  17.98&  15.38&  10.29&   5.41&   1.13&   0.41&   0.00&   0.00 \\ 
 397& 123015.010+021457.70&   3.50&   8.02&  21.07&  52.38&  59.15&  50.97&  45.09&  36.91&  28.31&  20.73&  10.36&   2.12&   0.76&   0.13&   0.00 \\ 
 398& 123032.861+215848.31&   0.00&  13.93&  12.81&  28.21&  35.56&  29.30&  23.82&   0.00&  16.12&  12.78&   7.88&   1.33&   0.49&   0.00&   0.00 \\ 
 399& 123054.458+103831.59&   0.00&   3.83&   8.66&  19.21&  25.99&  22.40&  18.92&  15.16&  13.16&   8.87&   5.50&   1.16&   0.44&   0.00&   0.00 \\ 
 400& 123114.863+412840.63&   2.13&   1.28&   6.46&  14.94&  25.98&  26.05&  23.83&   0.00&  16.89&  10.83&   8.02&   1.62&   0.60&   0.00&   0.00 \\ 
 401& 123126.964+032744.64&   0.00&  91.77&   0.00&   0.00&   0.65&   1.22&   1.31&  38.01&  28.91&  19.90&  10.02&   2.22&   0.84&   0.33&   0.14 \\ 
 402& 123305.035+480000.32&   0.00&  11.11&  17.10&  26.73&  30.93&  26.35&  21.70&   0.00&  16.23&   7.30&   5.42&   1.00&   0.41&   0.00&   0.00 \\ 
 403& 123339.146+270817.64&   0.00&  17.45&  20.20&  39.47&  41.92&  32.87&  25.59&   0.00&  15.32&   8.83&   7.25&   1.27&   0.58&   0.13&   0.00 \\ 
 404& 123443.783+612453.67&   0.00&  11.79&  40.88&  99.66& 106.70&  90.59&  76.88&   0.00&  51.32&  33.20&  19.49&   4.20&   1.46&   0.21&   0.00 \\ 
 405& 123614.983+015809.80&   0.00&  20.95&  15.70&  40.83&  40.01&  31.58&  25.49&  20.55&  15.41&  11.08&   5.92&   1.27&   0.50&   0.27&   0.00 \\ 
 406& 123820.722+482220.99&   0.00&  17.66&  11.81&  38.73&  45.62&  39.27&  35.43&   0.00&  21.01&  11.05&   6.65&   1.55&   0.60&   0.18&   0.00 \\ 
 407& 123822.282+473301.46&   0.00&   8.16&  18.39&  29.25&  39.21&  33.56&  25.92&   0.00&  15.80&  15.16&   7.43&   1.40&   0.58&   0.14&   0.00 \\ 
 408& 123827.545+603019.77&  55.54&  44.55&  32.62&  61.79&  56.98&  45.62&  36.13&   0.00&  24.82&  12.84&   6.99&   1.65&   0.59&   0.14&   0.00 \\ 
 409& 123841.064+591119.08&   0.00&  41.66&  44.05&  97.45&  90.88&  72.66&  62.13&   0.00&  38.14&  22.11&  14.04&   2.53&   0.87&   0.49&   0.00 \\ 
 410& 123846.505+363639.19&   0.00&   7.85&  10.65&  22.04&  26.85&  22.04&  18.83&   0.00&  15.00&   8.06&   5.10&   1.02&   0.38&   0.00&   0.00 \\ 
 411& 123904.289+364530.70&   0.00&   0.00&  11.95&  27.76&  38.26&  33.73&  29.10&   0.00&  14.83&  12.05&   7.56&   1.41&   0.53&   0.07&   0.00 \\ 
 412& 123928.978+580300.67&   0.00&  12.51&  29.94&  69.57&  79.82&  68.30&  58.66&   0.00&  38.90&  24.87&  15.79&   2.98&   1.10&   0.15&   0.00 \\ 
 413& 123936.050+122620.00&  54.73&   0.00& 208.30& 470.80& 497.30& 432.80& 351.50& 239.30& 185.90& 130.70&  60.38&  10.74&   3.02&   0.41&   0.00 \\ 
 414& 124018.902+164629.92& 127.00& 122.80& 192.20& 407.20& 426.90& 378.70& 333.80&   0.00& 192.30& 121.40&  63.86&  11.72&   3.48&   0.63&   0.23 \\ 
 415& 124100.271+452832.96&   0.00&   0.00&  13.12&  30.07&  35.35&  30.94&  26.78&   0.00&  15.03&  11.42&   5.03&   1.33&   0.49&   0.08&   0.00 \\ 
 416& 124204.380+272346.96&   0.00&  49.40&  70.23& 186.50& 187.40& 161.40& 131.80&  99.99&  74.54&  54.86&  20.84&   5.10&   1.58&   0.29&   0.00 \\ 
 417& 124204.666+150905.67&   0.00&   0.00&  84.38& 206.10& 199.20& 165.10& 136.70&   0.00&  90.14&  60.44&  29.19&   6.48&   2.05&   0.57&   0.24 \\ 
 418& 124246.428+114849.30&   0.00&   4.01&   8.84&  21.32&  32.43&  29.05&  25.75&  19.48&  17.43&  13.59&   7.97&   1.66&   0.67&   0.00&   0.00 \\ 
 419& 124252.958+023700.90&  34.16&  41.86&   0.00&   0.00&   0.00&   0.00&   0.00&  19.53&  13.99&   9.36&   4.39&   1.19&   0.43&   0.19&   0.00 \\ 
 420& 124309.629+270024.42&   0.00&   9.46&  13.43&  29.04&  29.47&  24.56&  16.20&  14.25&  10.15&   6.17&   3.49&   0.70&   0.27&   0.00&   0.00 \\ 
 421& 124350.398+315324.87&   9.09&  23.81&  55.60& 127.40& 130.10& 107.80&  91.92&  77.63&  54.97&  40.53&  20.52&   4.38&   1.53&   0.22&   0.10 \\ 
 422& 124354.629+163309.49&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&  10.86&   0.00&   4.68&   5.46&   0.00&   0.51&   0.19&   0.00&   0.00 \\ 
 423& 124406.722+621036.21&   0.00&   0.00&   7.75&  23.09&  31.54&  25.82&  20.91&   0.00&  18.73&  13.59&   8.82&   2.36&   0.89&   0.07&   0.00 \\ 
 424& 124427.307+400733.86&   0.00&  14.17&  11.07&  21.19&  27.24&  22.22&  19.30&   0.00&  12.89&   6.85&   5.68&   1.12&   0.44&   0.07&   0.12 \\ 
 425& 124458.783+140618.37&   0.00&   0.00&  22.43&  39.53&  42.87&  33.35&  28.23&  19.73&  14.16&   8.65&   4.77&   1.15&   0.54&   0.15&   0.00 \\ 
 426& 124521.422-014735.49&   0.00&  17.42&  17.84&  36.37&  41.37&  33.91&  25.53&  20.05&  16.44&  10.96&   5.96&   1.43&   0.59&   0.27&   0.25 \\ 
 427& 124534.169+402559.13&   0.00&  29.15&  62.01& 144.20& 143.00& 120.00& 100.90&   0.00&  60.94&  37.02&  21.18&   4.19&   1.29&   0.20&   0.00 \\ 
 428& 124645.722+345835.08&  56.32&  61.19&  42.31&  60.41&  61.66&  51.83&  45.54&  36.74&  29.34&  20.51&  10.93&   2.40&   0.92&   0.22&   0.00 \\ 
 429& 124700.254+351817.02&   0.00&  17.50&  11.94&  27.50&  31.76&  26.45&  21.35&  17.73&  13.68&  10.97&   4.89&   1.15&   0.47&   0.00&   0.00 \\ 
 430& 124700.708+034643.72&   5.59&   0.00&  19.94&   0.00&  59.19&   0.00&  45.02&  32.03&  32.60&  22.55&  10.90&   2.58&   0.94&   0.23&   0.18 \\ 
 431& 124728.826+384013.83&   0.00&   0.00&  15.52&  33.41&  38.89&  33.80&  28.41&   0.00&  18.95&  12.74&   8.07&   1.45&   0.58&   0.18&   0.00 \\ 
 432& 124755.409+053630.34&  26.22&  14.35&  16.48&  28.43&  25.81&  22.25&  17.32&  13.59&  10.05&   6.71&   3.37&   0.65&   0.24&   0.00&   0.17 \\ 
 433& 124835.986+131116.31&   0.00&   0.00&   8.20&  20.70&  30.37&  27.26&  23.38&  18.24&  15.94&  11.21&   6.71&   1.53&   0.64&   0.00&   0.00 \\ 
 434& 124942.612+313858.65&   0.00&  21.70&  23.17&  48.39&  51.05&  42.03&  34.17&  26.85&  20.69&  13.86&   7.40&   1.97&   0.74&   0.00&   0.10 \\ 
 435& 125004.553+293335.00&   0.00&  12.00&  12.73&  31.67&  32.89&  27.56&  22.29&  21.33&  16.99&  11.48&   5.38&   1.21&   0.43&   0.06&   0.00 \\ 
 436& 125017.088+632520.30&   0.00&   0.00&  15.29&  42.67&  45.56&  37.64&  31.26&   0.00&  21.24&  15.60&   8.51&   1.74&   0.68&   0.16&   0.00 \\ 
 437& 125306.727+181527.48&   0.00&   6.90&  13.03&  29.89&  40.59&  36.76&  31.70&   0.00&  21.80&  15.97&   8.81&   1.83&   0.68&   0.21&   0.00 \\ 
 438& 125633.547+391759.91&   0.00&   0.00&  11.19&  25.85&  27.81&  23.01&  18.18&   0.00&  11.73&   9.09&   6.59&   0.98&   0.37&   0.06&   0.00 \\ 
 439& 125720.429+460323.04&   0.00&   0.00&  98.31& 198.70& 181.60& 146.90& 120.30&   0.00&  63.08&  37.51&  17.02&   4.35&   1.40&   0.64&   0.29 \\ 
 440& 125738.234+313328.00&   0.00&  23.42&  62.64& 151.30& 155.50& 129.10& 112.10&  87.97&  67.43&  47.10&  22.46&   4.94&   1.58&   0.11&   0.00 \\ 
 441& 125744.112+290113.38&  10.40&  38.28&  64.75& 165.40& 162.80& 128.90&  95.41&  50.86&  36.30&  24.14&  10.24&   1.46&   0.44&   0.13&   0.00 \\ 
 442& 125745.302+275421.54&  24.59&  17.58&  23.75&  32.50&  29.94&  25.08&  18.38&  15.85&   9.83&   7.02&   3.64&   0.40&   0.12&   0.00&   0.00 \\ 
 443& 125754.862+270327.24&   0.00&  31.71&  48.08& 108.10& 102.40&  76.46&  57.79&  53.72&  42.57&  28.06&  14.60&   3.29&   1.18&   0.16&   0.00 \\ 
 444& 125820.722+613039.55& 448.70& 483.70& 235.80& 377.10& 290.10& 228.70& 171.70&   0.00& 112.30&  63.99&  37.73&   6.86&   2.22&   1.16&   0.44 \\ 
 445& 125842.590+274537.83& 119.00& 116.30&  59.84& 100.30&  66.50&  46.35&  28.74&  22.88&   6.22&   6.93&   1.10&   0.49&   0.16&   0.07&   0.00 \\ 
 446& 125946.279+274446.55&  17.91&  30.24&  25.81&  48.94&  36.85&  26.41&  20.54&  11.66&   6.22&   4.94&   2.21&   0.34&   0.13&   0.00&   0.00 \\ 
 447& 125948.276+185400.51&   0.00&  69.78&  57.31&  83.03&  75.73&  59.41&  48.39&   0.00&  31.49&  15.36&  10.61&   2.40&   1.17&   0.61&   0.41 \\ 
 448& 125956.251+380724.56&   0.00&   0.00&  10.81&  22.60&  35.05&  31.09&  25.83&   0.00&  16.84&  11.19&   8.63&   1.45&   0.56&   0.00&   0.00 \\ 
 449& 130105.654+280343.38&   0.00&  17.17&  23.16&  40.58&  36.77&  29.62&  23.84&  15.26&  11.95&   8.72&   3.15&   0.59&   0.19&   0.00&   0.00 \\ 
 450& 130130.720+211947.58&   0.00&  26.49&  44.11& 103.90&  96.16&  75.96&  58.78&   0.00&  31.69&  17.86&  13.16&   2.28&   0.85&   0.23&   0.00 \\ 
 451& 130501.548+071428.18&   0.00&  15.84&  34.93&  75.37&  84.66&  71.89&  61.71&  49.16&  36.26&  26.75&  13.51&   2.79&   1.03&   0.20&   0.00 \\ 
 452& 130544.712-033416.00&   0.00& 100.30&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&  36.18&  22.85&  15.88&   2.58&   0.99&   0.68&   0.36 \\ 
 453& 130619.274-005855.78&   0.00&   7.30&  11.58&  27.09&  39.22&  34.10&  27.70&  22.87&  18.99&  12.74&   7.50&   1.66&   0.69&   0.00&   0.00 \\ 
 454& 130733.077+291941.02&  35.86&  39.55&  26.76&  55.76&  47.85&  35.57&  28.56&  19.69&  15.11&   9.76&   4.79&   0.99&   0.36&   0.11&   0.00 \\ 
 455& 130737.766+011019.34&   0.00&  15.94&  14.82&  40.12&  54.49&  50.30&  44.16&  32.70&  25.15&  17.77&  10.75&   2.12&   0.83&   0.12&   0.14 \\ 
 456& 130808.990+103440.12&  49.88&  97.53&  72.57& 134.80& 119.80&  98.02&  77.76&  56.24&  42.29&  29.73&  14.39&   2.91&   1.30&   0.80&   0.33 \\ 
 457& 130843.886+611118.35&   0.00&   0.00&   6.32&  20.10&  27.50&  23.84&  20.44&   0.00&  15.60&  10.39&   5.22&   1.13&   0.46&   0.05&   0.00 \\ 
 458& 130933.156+223318.44&   0.00&  11.91&  12.88&  27.24&  29.23&  23.84&  19.09&  15.16&  11.24&   7.87&   4.00&   0.87&   0.33&   0.09&   0.00 \\ 
 459& 131022.390+362607.80&   0.00&   2.73&  12.30&  22.49&  30.36&  26.34&  23.27&   0.00&  15.38&  12.12&   0.00&   1.20&   0.46&   0.00&   0.00 \\ 
 460& 131107.342+251951.38&   0.00&   8.07&  34.74&  75.65&  88.25&  75.44&  60.86&  47.71&  31.80&  23.55&  11.39&   2.00&   0.71&   0.00&   0.00 \\ 
 461& 131154.862+522504.42&   0.00&   9.38&  15.13&  27.13&  36.06&  31.27&  26.84&   0.00&  18.01&  10.91&   7.91&   1.42&   0.58&   0.00&   0.00 \\ 
 462& 131207.759+391837.33&   0.00&   5.88&  11.36&  23.37&  23.79&  20.00&  17.84&   0.00&   8.33&   0.00&   0.00&   0.55&   0.22&   0.00&   0.00 \\ 
 463& 131431.711+090119.59&   0.00&   3.92&   9.26&  23.95&  26.01&  22.64&  19.34&  17.15&  12.64&   9.09&   3.96&   0.83&   0.25&   0.00&   0.00 \\ 
 464& 131558.706+042131.32&  38.50&  23.87&  54.09& 122.40& 127.60& 108.90&  94.19&  70.84&  52.61&  38.01&  18.37&   3.97&   1.34&   0.77&   0.27 \\ 
 465& 131608.280+294911.77&   0.00&  18.19&  11.33&  29.67&  29.91&  24.84&  19.37&  16.89&  11.49&   7.92&   4.24&   0.95&   0.34&   0.10&   0.00 \\ 
 466& 131648.499+160553.91&   0.00&   3.42&  11.70&  29.10&  30.60&  25.66&  21.03&   0.00&  14.45&   5.12&   5.91&   0.98&   0.40&   0.11&   0.00 \\ 
 467& 131700.478+113746.29&  17.87&  18.93&  18.09&  33.94&  37.78&  31.38&  25.61&  21.49&  16.52&  11.81&   7.15&   1.87&   1.16&   0.92&   0.82 \\ 
 468& 131722.241+462307.77&   0.00&  14.45&  26.40&  44.61&  50.26&  38.59&  29.75&   0.00&  14.59&  10.79&   7.34&   1.24&   0.49&   0.09&   0.13 \\ 
 469& 131740.963+174152.01&   0.00&  25.54&  79.05& 178.60& 180.90& 151.90& 124.00&   0.00&  77.49&  51.24&  25.94&   5.50&   1.85&   0.48&   0.00 \\ 
 470& 132021.432+163039.10&   0.00&  34.87&  36.44&  77.76&  87.52&  73.52&  60.17&   0.00&  32.96&  19.82&  13.62&   2.64&   1.00&   0.19&   0.11 \\ 
 471& 132058.574+465433.36&  41.97&  45.75&  45.81&  74.19&  69.84&  57.06&  45.99&   0.00&  25.51&  13.77&  10.55&   1.94&   0.74&   0.36&   0.12 \\ 
 472& 132104.735+571523.44&   0.00&  30.17&  48.20&  79.84&  71.86&  58.19&  46.66&   0.00&  30.91&  21.68&  13.23&   2.31&   0.84&   0.47&   0.20 \\ 
 473& 132214.945+074814.28&   0.00&   0.00&   7.87&  17.93&  26.78&  23.47&  19.33&  16.14&  13.00&   9.54&   5.50&   1.28&   0.50&   0.00&   0.00 \\ 
 474& 132241.465+324614.58&   0.00&   3.82&  17.16&  40.73&  50.10&  44.96&  39.78&  31.98&  24.72&  18.88&   9.18&   2.01&   0.73&   0.07&   0.12 \\ 
 475& 132256.018+103957.87&  21.07&   9.18&   7.41&  12.52&  24.44&  22.58&  19.43&  16.48&  12.96&  10.10&   6.47&   1.59&   0.59&   0.10&   0.00 \\ 
 476& 132309.715+630008.32&   0.00&  10.62&  12.67&  33.74&  40.27&  34.08&  28.24&   0.00&  20.93&  15.11&   8.96&   1.66&   0.61&   0.00&   0.00 \\ 
 477& 132315.578+630726.73&   0.00&   2.60&   7.35&  22.75&  31.71&  29.82&  26.64&   0.00&  14.60&  10.67&   4.57&   1.21&   0.44&   0.06&   0.00 \\ 
 478& 132415.139+140755.07&   0.00&  33.87&  77.65& 157.40& 159.30& 133.30& 115.40&  81.80&  58.86&  42.45&  21.73&   4.27&   1.50&   0.58&   0.16 \\ 
 479& 132419.778+282150.71&   0.00&   5.04&  10.43&  23.70&  33.00&  30.78&  28.81&  20.82&  18.55&  12.01&   6.17&   1.63&   0.58&   0.06&   0.00 \\ 
 480& 132540.798+070820.95&  57.16&  18.08&  17.86&  31.95&  39.02&  34.78&  27.53&  23.29&  19.88&  14.44&   7.84&   1.44&   0.56&   0.24&   0.12 \\ 
 481& 132542.305+325503.90&   0.00&   4.38&   6.11&  15.50&  26.19&  22.42&  18.70&  15.52&  11.66&   8.69&   5.55&   1.28&   0.47&   0.10&   0.00 \\ 
 482& 132550.630+171410.62&   0.00&  13.97&  24.15&  62.68&  61.66&  51.21&  42.07&   0.00&  28.89&  19.61&   9.01&   2.10&   0.69&   0.16&   0.00 \\ 
 483& 132608.417+255057.18&   0.00&   9.74&  28.88&  65.04&  73.57&  62.96&  54.86&  36.13&  26.80&  22.49&  11.66&   2.11&   0.73&   0.00&   0.00 \\ 
 484& 132722.721+313044.18&  19.09&  51.35&  38.15&  62.05&  55.67&  43.44&  34.87&  29.58&  21.63&  15.27&   7.83&   1.66&   0.55&   0.14&   0.00 \\ 
 485& 133024.746+022325.86&   0.00&   0.00&   9.43&  30.70&  34.10&  28.67&  23.28&  35.23&  26.07&  17.61&   8.34&   1.83&   0.58&   0.38&   0.19 \\ 
 486& 133044.158+224225.49&   0.00&   9.39&  13.82&  34.58&  38.00&  31.65&  27.31&  21.84&  16.62&  11.41&   5.99&   1.41&   0.52&   0.14&   0.13 \\ 
 487& 133156.918+135813.30&   0.00&   5.50&   7.85&  18.89&  25.50&  22.83&  19.66&  16.47&  13.42&   9.29&   5.50&   1.19&   0.46&   0.00&   0.00 \\ 
 488& 133323.791+532130.14&  39.33&  73.36&  83.71& 177.40& 180.30& 152.60& 122.40&   0.00&  60.30&  40.77&  21.38&   4.28&   1.44&   0.45&   0.12 \\ 
 489& 133350.731-001617.68&   0.00&   0.00&  18.29&  41.90&  51.77&  45.32&  38.75&  27.67&  24.04&  15.84&   7.77&   1.93&   0.74&   0.19&   0.00 \\ 
 490& 133418.110-003956.64&   0.00&   0.00&   6.14&  13.26&  19.04&  17.41&  15.19&   0.00&  10.13&   6.72&   4.36&   1.76&   0.75&   0.11&   0.00 \\ 
 491& 133436.547+381944.50&   0.00&   0.00&  58.69&  78.18&  72.04&  58.43&  45.54&   0.00&  23.52&  14.05&   6.43&   1.42&   0.50&   0.41&   0.29 \\ 
 492& 133552.598+452205.97&   0.00&   0.00&  23.55&  55.26&  66.27&  59.30&  52.96&   0.00&  36.07&  27.56&  13.21&   3.27&   1.32&   0.33&   0.00 \\ 
 493& 133602.280+322040.00&  53.90&  55.15&  43.62&  69.08&  65.84&  52.85&  41.63&  35.41&  27.93&  19.25&  10.67&   2.53&   1.13&   0.36&   0.32 \\ 
 494& 133638.748+193448.72&   0.00&   8.87&  20.52&  52.04&  55.20&  47.36&  39.63&   0.00&  26.01&  12.13&   7.17&   1.47&   0.47&   0.06&   0.00 \\ 
 495& 133751.302+354755.79&   0.00&   0.00&  50.96& 116.80& 110.70&  90.82&  72.59&  64.65&  51.64&  37.12&  18.30&   4.96&   1.66&   1.01&   0.42 \\ 
 496& 134041.933+175332.48&   0.00&   0.00&  17.72&  38.08&  37.68&  30.27&  24.40&   0.00&  17.85&  12.20&   6.89&   1.22&   0.44&   0.19&   0.14 \\ 
 497& 134043.375+070428.37&   0.00&  29.90&  19.86&  42.15&  44.17&  35.59&  28.91&  24.12&  18.39&  13.47&   7.04&   1.49&   0.56&   0.09&   0.00 \\ 
 498& 134249.519+541238.87&   0.00&   0.00&  20.33&  29.74&  33.27&  28.01&  22.13&   0.00&  12.98&   8.15&   6.22&   0.95&   0.39&   0.13&   0.00 \\ 
 499& 134516.118+060637.42&   0.00&  16.45&  28.05&  63.33&  71.62&  62.47&  53.37&  44.06&  35.42&  25.70&  12.64&   2.65&   0.98&   0.17&   0.00 \\ 
 500& 134722.030+181719.27&   0.00&   1.55&   4.89&  15.64&  22.75&  19.80&  16.75&   0.00&  13.88&  10.49&   6.14&   1.05&   0.46&   0.00&   0.00 \\ 
 501& 134738.066+174359.34&   0.00&   0.00&  16.39&  38.51&  45.63&  38.36&  32.04&   0.00&  22.86&  10.89&   8.50&   1.66&   0.70&   0.00&   0.00 \\ 
 502& 134802.182+020405.73&  16.32&  46.84&  67.94& 151.30& 142.60& 116.00&  96.00&  76.06&  57.35&  41.41&  18.56&   4.05&   1.33&   0.32&   0.18 \\ 
 503& 134804.301+445032.45&  24.92&  48.98&  28.26&  46.94&  39.59&  30.56&  24.35&   0.00&  14.34&   8.63&   7.68&   1.13&   0.44&   0.26&   0.26 \\ 
 504& 134809.684+623612.69&   0.00&   9.84&  14.30&  36.78&  44.63&  37.51&  29.36&   0.00&  20.10&   9.78&   9.14&   1.48&   0.61&   0.05&   0.00 \\ 
 505& 134822.870+174847.26&   0.00&   0.00&  10.33&  25.60&  26.83&  23.24&  20.25&   0.00&  12.50&   9.98&   4.88&   0.85&   0.25&   0.00&   0.00 \\ 
 506& 134909.103+281956.65&   0.00&   3.17&   4.56&  13.75&  26.03&  23.80&  21.93&  18.03&  13.66&  10.77&   6.53&   1.71&   0.67&   0.05&   0.00 \\ 
 507& 134948.118+212237.80&   0.00&  12.46&  31.47&  68.42&  67.79&  57.66&  47.63&   0.00&  20.42&  19.19&   8.73&   1.69&   0.62&   0.15&   0.00 \\ 
 508& 135005.585-024734.67&   0.00&   0.00&  30.25&  57.26&  60.34&  52.18&  41.84&   0.00&  63.68&  38.57&  23.67&   4.20&   1.59&   0.67&   0.71 \\ 
 509& 135026.501+325615.66&   0.00&  18.43&  24.13&  47.90&  53.44&  45.57&  35.43&  26.93&  21.20&  14.63&   8.42&   1.83&   0.71&   0.31&   0.09 \\ 
 510& 135030.766+012804.72&  14.28&  44.30&  60.24& 141.10& 131.50& 107.70&  86.52&  77.20&  57.31&  38.14&  17.94&   4.00&   1.36&   0.28&   0.31 \\ 
 511& 135124.773+054903.13&  54.15&  92.17&  97.19& 220.60& 205.50& 168.20& 141.10&   0.00& 159.00&  96.97&  50.11&  10.09&   3.04&   0.31&   0.15 \\ 
 512& 135505.537+124812.27&   0.00&   0.00&  10.29&  26.35&  34.77&  30.75&  24.93&  23.25&  17.54&  12.53&   7.30&   1.56&   0.66&   0.24&   0.00 \\ 
 513& 135535.894+084915.55&  54.67&  33.57&  33.07&  68.85&  71.79&  61.46&  52.37&  35.93&  27.93&  21.31&  12.47&   2.57&   0.90&   0.22&   0.00 \\ 
 514& 135556.333+093526.10&   5.24&  11.91&  29.39&  74.18&  75.86&  64.27&  53.11&  45.59&  34.31&  24.74&  11.16&   2.19&   0.73&   0.10&   0.00 \\ 
 515& 135631.582-001608.21&   0.00&   3.04&  10.79&  29.51&  36.65&  31.73&  27.33&  22.93&  18.62&  12.81&   5.96&   1.41&   0.54&   0.00&   0.00 \\ 
 516& 135737.553-022645.98&   0.00& 115.40&  90.34& 162.70& 138.80& 107.70&  83.40&   0.00&  49.48&  31.57&  15.38&   3.13&   1.08&   0.34&   0.13 \\ 
 517& 135908.323+272445.96&  38.99&  25.07&  18.38&  33.17&  31.65&  24.79&  18.40&  14.22&  10.77&   7.05&   3.72&   0.75&   0.31&   0.20&   0.00 \\ 
 518& 135914.218+123653.45&   0.00&   0.00&   5.25&  25.93&  27.99&  24.05&  21.37&  17.26&  13.30&   9.46&   4.81&   1.00&   0.37&   0.13&   0.00 \\ 
 519& 135937.757+283925.97&   0.00&  18.48&  13.26&  29.15&  33.64&  28.83&  23.65&  17.17&  12.33&   8.20&   5.20&   1.06&   0.45&   0.11&   0.00 \\ 
 520& 135949.865+540420.02&   0.00&   0.00&   0.00&  15.21&  32.81&  29.55&  25.77&   0.00&  13.62&  10.26&   7.99&   1.50&   0.54&   0.00&   0.00 \\ 
 521& 140000.850+001518.57&   0.00&  34.45&  14.70&  58.71&  57.51&  46.91&  39.77&   0.00&  20.25&  11.93&   7.37&   1.56&   0.61&   0.20&   0.00 \\ 
 522& 140004.891+300533.72&   0.00&  33.84&  40.21&  64.97&  63.70&  52.20&  39.96&  33.64&  24.27&  16.99&   8.58&   1.83&   0.66&   0.39&   0.11 \\ 
 523& 140014.345+502324.97&   0.00&  14.66&  31.87&  66.86&  81.85&  73.93&  62.99&   0.00&  41.62&  24.19&  16.54&   3.00&   1.11&   0.05&   0.00 \\ 
 524& 140148.566+061534.60&   0.00&  11.52&  19.05&  48.19&  56.11&  47.95&  41.75&  35.28&  26.07&  18.64&   9.18&   1.94&   0.70&   0.08&   0.00 \\ 
 525& 140247.854+530751.61&   0.00&   7.05&  16.35&  31.26&  38.59&  33.86&  30.38&   0.00&  20.78&  10.32&  10.40&   1.64&   0.64&   0.14&   0.00 \\ 
 526& 140348.946+271843.24&   0.00&  31.05&  20.74&  32.08&  36.59&  33.76&  23.04&   0.00&  17.23&  12.80&   5.56&   1.31&   0.55&   0.18&   0.00 \\ 
 527& 140429.249+102225.92&  10.95&  12.92&  14.14&  26.84&  26.22&  22.00&  19.08&  15.73&  11.08&   8.50&   4.34&   0.85&   0.33&   0.00&   0.00 \\ 
 528& 140436.542+171804.52&   0.00&   9.07&  16.22&  33.91&  45.94&  40.81&  36.51&   0.00&  23.44&  16.67&  11.47&   3.13&   2.06&   0.64&   0.47 \\ 
 529& 140455.613+135246.81&   0.00&   6.33&  13.15&  29.24&  31.23&  26.29&  21.02&  18.11&  14.04&   9.27&   5.03&   1.11&   0.41&   0.10&   0.00 \\ 
 530& 140529.830+110923.79&   0.00&  14.81&  13.96&  37.39&  43.24&  36.73&  28.62&  32.74&  19.83&  17.53&  10.50&   1.96&   0.79&   0.09&   0.00 \\ 
 531& 140535.683+070143.27&   9.75&  15.66&  16.37&  34.63&  35.35&  28.53&  24.43&  20.97&  15.14&  11.29&   5.35&   1.18&   0.41&   0.07&   0.00 \\ 
 532& 140634.150+372142.15&   0.00&   6.48&  16.14&  35.19&  47.00&  41.67&  34.50&   0.00&  23.42&  14.86&   9.94&   1.91&   0.74&   0.06&   0.00 \\ 
 533& 140635.978+084523.87&   0.00&  28.18&  36.93&  95.75&  89.62&  71.46&  58.10&  52.22&  37.96&  25.65&  12.54&   2.65&   0.91&   0.24&   0.00 \\ 
 534& 140644.287+261906.64&   0.00&   0.00&  15.24&  34.58&  39.48&  33.92&  28.19&   0.00&  15.92&  13.30&   8.08&   1.60&   0.71&   0.20&   0.00 \\ 
 535& 140656.482+124513.74&   0.00&  13.34&  12.25&  29.90&  33.11&  30.30&  23.67&  20.19&  13.69&  12.05&   4.68&   0.86&   0.27&   0.00&   0.00 \\ 
 536& 140713.495+163403.29&   0.00&   4.18&  27.50&  67.68&  71.26&  60.27&  52.27&   0.00&  39.33&  18.37&  13.02&   2.62&   0.87&   0.37&   0.13 \\ 
 537& 140728.121+262451.31&   0.00&  11.86&  20.49&  36.61&  37.33&  31.09&  26.85&   0.00&  18.49&  10.45&   3.22&   1.03&   0.39&   0.21&   0.15 \\ 
 538& 140801.615+514226.05&   0.00&  29.98&  37.44&  71.47&  77.01&  66.33&  54.58&   0.00&  30.33&  22.25&  12.75&   2.33&   0.88&   0.43&   0.00 \\ 
 539& 140845.458+135041.06&   0.00&   0.00&  37.26&  59.64&  63.58&  55.45&  46.64&  33.90&  27.17&  19.29&  10.09&   2.22&   0.83&   0.25&   0.00 \\ 
 540& 140943.224-000036.88&  23.05&  11.00&  17.52&  37.14&  39.92&  32.59&  27.32&  21.60&  12.75&  10.62&   5.27&   1.12&   0.40&   0.00&   0.00 \\ 
 541& 141003.672+603229.82&   0.00&   0.00&  40.32&  69.93&  79.40&  68.38&  58.97&   0.00&  35.62&  22.39&  13.08&   2.77&   1.06&   0.24&   0.17 \\ 
 542& 141104.169+400918.45&   0.00&   0.00&  35.37&  64.16&  61.02&  51.34&  40.03&   0.00&  23.57&  12.85&  11.02&   1.86&   0.68&   0.38&   0.27 \\ 
 543& 141109.737+265051.37&   0.00&   0.00&  11.72&  26.51&  27.45&  22.24&  18.16&   0.00&  13.79&   5.75&   4.57&   0.92&   0.35&   0.08&   0.14 \\ 
 544& 141117.014+205233.48&   0.00&   0.00&  18.48&  43.59&  43.78&  33.28&  24.17&   0.00&  18.93&  12.19&   5.71&   1.10&   0.41&   0.22&   0.11 \\ 
 545& 141125.037+314551.35&   0.00&  10.60&  11.42&  24.61&  27.62&  21.96&  16.78&   0.00&  11.95&   8.36&   5.17&   0.98&   0.38&   0.00&   0.00 \\ 
 546& 141126.856+614516.65&  97.64&  73.88&  48.62&  82.68&  79.53&  64.77&  53.47&   0.00&  36.75&  22.53&  13.02&   2.62&   0.95&   0.42&   0.24 \\ 
 547& 141127.494+243809.54&   0.00&  72.74&  62.87& 111.90&  94.65&  75.18&  62.08&   0.00&  41.42&  28.58&  13.96&   2.84&   0.90&   0.08&   0.00 \\ 
 548& 141143.166+450353.05&   0.00&  19.26&  18.45&  31.68&  30.83&  26.40&  21.28&   0.00&  10.28&   9.26&   4.46&   0.95&   0.34&   0.22&   0.00 \\ 
 549& 141239.722+223509.83&   0.00&   3.97&   9.84&  20.67&  24.42&  20.97&  18.06&   0.00&  14.66&   8.54&   5.68&   1.02&   0.38&   0.00&   0.00 \\ 
 550& 141241.962+261707.15&   0.00&   7.59&  13.41&  31.77&  38.28&  31.14&  24.72&   0.00&  19.91&  11.80&   8.28&   1.64&   0.61&   0.21&   0.12 \\ 
 551& 141256.630+223125.38&   0.00&  12.69&  31.93&  55.60&  55.95&  48.38&  38.35&   0.00&  22.77&  13.87&  10.85&   1.78&   0.70&   0.37&   0.00 \\ 
 552& 141342.266+522809.97&   0.00&   8.57&  15.58&  33.11&  45.99&  40.26&  35.22&   0.00&  21.93&  13.61&   9.74&   2.04&   0.88&   0.34&   0.00 \\ 
 553& 141419.296-031111.52&  93.69& 258.50& 182.30& 414.00& 440.50& 369.30& 323.80&   0.00& 185.30& 117.40&  62.28&   7.65&   2.35&   1.21&   0.33 \\ 
 554& 141505.167-023339.76&  11.70&   0.00&  15.87&  28.37&  32.98&  27.57&  21.79&   0.00&  10.19&   9.21&   4.99&   1.11&   0.44&   0.20&   0.18 \\ 
 555& 141517.150+152139.00&   0.00&  16.56&  11.57&  24.66&  31.99&  26.82&  23.83&   0.00&  10.88&   8.18&   4.99&   1.21&   0.46&   0.00&   0.00 \\ 
 556& 141625.630+340050.20&  20.80&  21.09&  21.99&  38.17&  37.58&  30.41&  23.93&   0.00&  14.76&   5.82&   5.04&   0.91&   0.35&   0.00&   0.00 \\ 
 557& 141626.558+252125.29&   8.88&  20.07&  30.55&  61.39&  60.93&  49.35&  41.34&   0.00&  23.82&  14.51&   7.52&   1.71&   0.64&   0.19&   0.00 \\ 
 558& 141728.728+602113.88& 143.60& 129.70&  75.32&  86.56&  64.50&  51.01&  42.89&   0.00&  30.80&  16.88&  11.26&   2.37&   0.84&   0.42&   0.23 \\ 
 559& 141808.993+401245.52&   0.00&   9.56&  19.07&  41.27&  50.42&  43.15&  37.07&   0.00&  25.86&  14.25&  11.25&   1.95&   0.74&   0.05&   0.00 \\ 
 560& 141854.103+050547.48&   0.00& 262.50& 144.20& 306.00& 258.10& 204.30& 153.20&   0.00&  95.75&  66.87&  33.78&   6.17&   2.18&   1.38&   0.48 \\ 
 561& 141854.149+272738.29&   0.00&  13.17&  12.72&  29.84&  34.98&  30.16&  26.79&   0.00&  22.39&  12.96&   9.14&   1.53&   0.57&   0.14&   0.00 \\ 
 562& 141950.878+312620.57&  18.27&   5.68&  22.50&  46.47&  48.55&  40.03&  33.13&   0.00&  18.64&  15.21&   6.37&   1.58&   0.59&   0.07&   0.00 \\ 
 563& 142026.890+063550.99&   0.00&  28.93&  30.76&  41.47&  44.09&  32.83&  27.79&  17.47&  14.10&   8.47&   4.77&   1.07&   0.42&   0.15&   0.00 \\ 
 564& 142112.278+543023.69&   0.00&   5.84&   5.03&  20.93&  27.63&  23.57&  18.40&   0.00&  19.29&  13.54&   8.09&   1.21&   0.42&   0.07&   0.00 \\ 
 565& 142257.727+225441.43& 1275.00& 784.00& 181.90& 186.30& 110.20&  74.11&  50.80&   0.00&  22.51&  13.04&   7.60&   1.52&   0.52&   0.29&   0.16 \\ 
 566& 142355.627+390732.82&   0.00&   9.50&  13.36&  32.05&  32.83&  27.89&  23.16&   0.00&  13.90&   9.53&   4.22&   1.11&   0.38&   0.12&   0.00 \\ 
 567& 142455.692+264438.98&   0.00&   0.00&   7.32&  17.20&  25.46&  23.07&  19.07&   0.00&  14.09&  10.01&   6.24&   1.18&   0.51&   0.07&   0.00 \\ 
 568& 142658.445+421615.53&   0.00&   3.35&   3.78&   6.36&  11.92&   9.59&   7.61&   0.00&   0.00&   0.00&   0.00&   0.52&   0.19&   0.00&   0.11 \\ 
 569& 142736.686+430202.29&   0.00&  20.42&  23.49&  44.77&  42.59&  34.54&  30.43&   0.00&  18.62&  10.09&   7.54&   1.24&   0.45&   0.06&   0.00 \\ 
 570& 142808.419+062545.01&   0.00&  29.25&  35.67&  86.63&  97.13&  82.21&  68.30&   0.00&  38.00&  25.17&  12.80&   2.99&   1.19&   0.23&   0.00 \\ 
 571& 142848.228+274149.66&   0.00&   7.33&  22.69&  52.56&  54.42&  44.72&  37.54&   0.00&  28.97&  14.18&   9.59&   1.86&   0.65&   0.00&   0.00 \\ 
 572& 142926.477+552945.85&  31.96&  31.33&  28.32&  54.17&  57.80&  48.09&  38.46&   0.00&  25.23&  15.83&   9.22&   1.91&   0.70&   0.06&   0.00 \\ 
 573& 143055.824+000451.33&   0.00&  10.80&  22.12&  47.34&  46.51&  37.64&  30.76&  24.13&  19.00&  12.18&   6.09&   1.33&   0.42&   0.09&   0.00 \\ 
 574& 143057.521-013939.64&   0.00&   5.69&  19.88&  45.86&  46.77&  39.17&  32.76&  27.72&  21.68&  15.37&   7.76&   1.76&   0.59&   0.17&   0.11 \\ 
 575& 143101.510+580443.22&  74.37&  34.42&  18.56&  40.41&  47.37&  38.20&  29.44&   0.00&  15.51&  14.26&   8.63&   1.63&   0.69&   0.16&   0.00 \\ 
 576& 143137.968+021942.27&  13.40&  16.54&  16.85&  30.60&  29.74&  24.76&  23.67&  17.54&  11.86&   7.51&   5.44&   1.03&   0.40&   0.08&   0.00 \\ 
 577& 143140.270+030154.09&   0.00&   8.34&  11.40&  23.59&  27.63&  23.53&  21.03&  17.87&  12.81&   8.35&   5.01&   1.26&   0.52&   0.21&   0.15 \\ 
 578& 143146.399+341719.01&  25.06&  48.47&  50.96& 110.50& 104.00&  81.79&  68.01&   0.00&  43.78&  26.34&  14.71&   3.17&   1.14&   0.30&   0.18 \\ 
 579& 143224.026+512428.59&   0.00&  12.80&  24.59&  49.65&  57.50&  46.83&  38.98&   0.00&  24.45&  11.50&  10.74&   1.96&   0.78&   0.29&   0.00 \\ 
 580& 143241.832+374054.27&   0.00&   0.00&  32.52&  76.52&  77.47&  63.00&  52.32&   0.00&  29.12&  17.96&   9.60&   2.56&   0.95&   0.06&   0.00 \\ 
 581& 143300.154+055525.45&   0.00&  12.95&  18.75&  39.70&  46.61&  41.00&  35.51&  28.72&  24.29&  16.07&   8.88&   1.93&   0.70&   0.10&   0.00 \\ 
 582& 143326.743+114728.86&   0.00&   0.00&  21.48&  46.53&  56.27&  49.50&  39.69&  33.86&  27.13&  18.50&   9.49&   2.16&   0.82&   0.06&   0.00 \\ 
 583& 143347.899+230748.14&   3.34&   0.00&   0.00&   0.00&   0.00&   0.00&  44.16&   0.00&  33.53&  18.17&  12.35&   2.35&   0.89&   0.06&   0.00 \\ 
 584& 143350.006+233407.82&   0.00&  57.48&  42.51&  77.61&  75.48&  59.91&  50.62&   0.00&  33.26&  19.46&  14.56&   2.28&   0.89&   0.51&   0.26 \\ 
 585& 143414.026+030140.28&   0.00&   8.11&  11.73&  20.11&  31.48&  26.44&  20.11&  16.07&  11.28&   8.27&   5.15&   1.19&   0.46&   0.07&   0.00 \\ 
 586& 143454.804+080306.39&   0.00&  32.55&  14.61&  28.11&  33.13&  26.30&  20.13&  19.16&  15.25&  10.20&   5.17&   1.25&   0.50&   0.08&   0.00 \\ 
 587& 143553.215+184719.78&   0.00&   0.00&  18.68&  38.10&  40.17&  34.40&  30.86&   0.00&  18.72&  11.74&   5.29&   1.22&   0.37&   0.11&   0.00 \\ 
 588& 143614.866+334940.87&   2.75&   7.68&  12.88&  32.84&  32.41&  27.02&  22.53&   0.00&  13.09&   8.15&   6.26&   0.97&   0.33&   0.08&   0.00 \\ 
 589& 143635.635+443351.52&   0.00&   0.00&  53.67& 126.10& 124.20& 102.00&  86.44&   0.00&  52.82&  32.95&  17.12&   3.80&   1.25&   0.13&   0.12 \\ 
 590& 143827.098+144116.81&   0.00&   7.41&  11.92&  31.01&  36.30&  30.52&  25.50&   0.00&  14.77&  12.31&   9.21&   1.31&   0.51&   0.05&   0.09 \\ 
 591& 143841.184+001025.26&   0.00&   3.04&  13.85&  36.64&  40.73&  36.10&  29.74&  24.65&  20.09&  13.76&   6.50&   1.44&   0.49&   0.00&   0.00 \\ 
 592& 143854.007+253454.57&   0.00&   0.00&  15.50&  25.97&  29.28&  25.60&  20.34&   0.00&  13.80&  11.58&   0.00&   0.95&   0.33&   0.05&   0.00 \\ 
 593& 144006.192+170020.17&   0.00&   0.00&  15.46&  36.00&  37.69&  31.56&  25.62&   0.00&  16.20&  10.54&   5.83&   1.12&   0.42&   0.00&   0.00 \\ 
 594& 144021.259+034612.81&  15.53&  12.07&  21.24&  31.86&  26.31&  22.58&  12.22&   9.52&   8.59&   3.04&   2.75&   0.64&   0.19&   0.00&   0.00 \\ 
 595& 144058.145+124855.41&   0.00&   5.13&  10.93&  24.40&  28.22&  23.86&  21.04&  16.14&  14.55&   9.07&   4.94&   1.07&   0.40&   0.00&   0.00 \\ 
 596& 144108.110+120255.07&   0.00&  18.16&  14.68&  25.76&  34.23&  28.71&  25.51&  18.61&  16.88&  12.28&   6.89&   1.26&   0.50&   0.06&   0.00 \\ 
 597& 144157.809+243649.25&   0.00&   0.00&  30.05&  49.94&  50.72&  41.93&  33.99&   0.00&  23.10&  12.13&   6.66&   1.34&   0.42&   0.30&   0.24 \\ 
 598& 144200.211+495449.11&   0.00&   9.95&  22.31&  43.00&  55.66&  49.68&  41.97&   0.00&  23.47&  16.80&  10.66&   2.23&   0.84&   0.11&   0.12 \\ 
 599& 144205.254+515153.25&   0.00&   0.00&  46.18&  80.46&  85.64&  72.01&  57.41&   0.00&  30.15&  25.01&  10.57&   2.50&   0.84&   0.08&   0.00 \\ 
 600& 144206.475+254725.94&   0.00&  13.42&  11.78&  27.08&  37.82&  33.06&  27.88&   0.00&  21.06&  16.24&  11.04&   1.71&   0.63&   0.05&   0.00 \\ 
 601& 144220.342+181900.04&  56.05&  69.38&  35.07&  83.08&  82.43&  70.24&  54.93&   0.00&  36.34&  24.48&  12.17&   2.54&   0.82&   0.14&   0.09 \\ 
 602& 144229.851+222014.97&  36.13&  37.66&  28.95&  53.47&  46.50&  35.36&  23.46&   0.00&  14.50&   9.09&   4.93&   1.00&   0.32&   0.00&   0.00 \\ 
 603& 144315.468+115224.06&   0.00&  17.98&  39.10&  85.62&  95.98&  81.80&  69.12&  58.12&  45.54&  33.62&  17.14&   3.31&   1.18&   0.11&   0.00 \\ 
 604& 144400.794+211850.53&   0.00&   0.00&  14.77&  26.45&  30.04&  25.14&  20.65&   0.00&  12.42&  12.06&   5.48&   1.14&   0.42&   0.06&   0.00 \\ 
 605& 144436.895+264137.41&  27.40&   0.00&  20.95&  44.02&  47.15&  40.01&  35.35&   0.00&  21.59&  12.57&   6.82&   1.54&   0.49&   0.19&   0.00 \\ 
 606& 144446.735+635042.71&   0.00&   0.00&  14.44&  40.75&  46.61&  41.43&  33.87&   0.00&  22.37&  18.50&   8.98&   1.93&   0.65&   0.15&   0.00 \\ 
 607& 144539.480+553651.07&   0.00&   6.82&   6.62&  12.41&  21.93&  20.83&  18.57&   0.00&  12.57&  11.98&   5.52&   1.32&   0.52&   0.05&   0.00 \\ 
 608& 144721.562+051352.34&   9.41&  17.90&  27.20&  60.86&  66.47&  55.43&  46.41&   0.00&  33.45&  20.85&  12.45&   2.47&   0.92&   0.07&   0.00 \\ 
 609& 144752.466+324111.73&   0.00&   9.42&  12.18&  28.97&  30.57&  26.20&  22.58&  19.26&  14.79&  10.50&   4.98&   1.10&   0.35&   0.00&   0.00 \\ 
 610& 144816.049+173305.94&   0.00& 159.10&  68.14& 198.00& 189.60& 147.60& 117.60&   0.00&  66.77&  40.93&  20.04&   3.51&   1.36&   1.23&   1.52 \\ 
 611& 144854.276+313929.01&  13.40&  45.83&  56.15& 127.50& 115.30&  93.04&  74.85&   0.00&  46.98&  30.73&  15.35&   3.44&   1.15&   0.46&   0.08 \\ 
 612& 145009.391+181937.35&   0.00&  10.66&  24.42&  51.15&  52.69&  44.79&  33.15&   0.00&  23.40&  10.59&   9.31&   1.50&   0.50&   0.14&   0.00 \\ 
 613& 145035.138+162223.59&   0.00&   0.00&   9.21&  20.89&  27.18&  23.20&  18.74&   0.00&  17.15&   5.47&   5.08&   1.17&   0.48&   0.05&   0.00 \\ 
 614& 145105.630+180735.43&   0.00&   0.00&  14.21&  27.42&  31.03&  26.07&  22.04&   0.00&  13.23&   8.50&   5.05&   1.05&   0.34&   0.05&   0.00 \\ 
 615& 145119.735+395353.65&   0.00&  10.61&  12.75&  31.22&  43.71&  37.85&  32.13&   0.00&  18.76&  11.88&   5.97&   1.75&   0.70&   0.26&   0.13 \\ 
 616& 145133.857+022658.62&   3.33&   7.29&  18.12&  39.11&  39.50&  32.58&  27.60&  24.41&  18.80&  12.70&   6.46&   1.43&   0.49&   0.06&   0.00 \\ 
 617& 145208.652+165805.27&   0.00&   0.00&  17.11&  50.34&  52.86&  45.71&  39.29&   0.00&  10.60&   0.00&   0.00&   1.38&   0.47&   0.21&   0.00 \\ 
 618& 145220.189+154927.80&   0.00&   0.00&  19.22&  76.91&  85.63&  69.66&  56.20&   0.00&  26.44&  18.17&  11.35&   2.11&   0.81&   0.20&   0.12 \\ 
 619& 145237.118+082226.86&   0.00&  38.89&  22.68&  34.97&  43.09&  35.12&  28.40&  23.65&  17.24&  12.15&   7.43&   1.81&   0.83&   0.33&   0.19 \\ 
 620& 145245.468+025321.34&   0.00&  17.35&  10.01&  25.55&  33.63&  26.72&  21.21&  16.22&  13.15&   8.56&   5.29&   1.24&   0.48&   0.12&   0.00 \\ 
 621& 145408.638+201241.79&   0.00&  29.09&  16.82&  39.66&  46.29&  41.28&  35.07&   0.00&  20.30&  10.51&   7.79&   1.80&   0.72&   0.27&   0.00 \\ 
 622& 145428.925+231936.44&   0.00&  45.07&  36.13&  87.61&  89.06&  78.48&  64.13&   0.00&  33.72&  19.27&  14.95&   2.42&   0.95&   0.56&   0.12 \\ 
 623& 145440.678+203834.87&   0.00&   0.00&  14.73&  27.98&  30.16&  25.94&  19.89&   0.00&  12.46&   9.05&   3.89&   1.21&   0.51&   0.24&   0.22 \\ 
 624& 145455.445+453126.60&  20.08&  39.62& 128.00& 293.30& 302.00& 260.70& 222.80&   0.00& 129.20&  84.40&  47.01&   7.29&   2.20&   0.31&   0.20 \\ 
 625& 145505.446+131651.64&   0.00&  29.74&  37.06&  89.08&  88.93&  74.22&  61.38&   0.00&  40.33&  22.95&  12.11&   3.01&   1.09&   0.82&   0.73 \\ 
 626& 145511.364+190420.42&   0.00&   2.78&  21.36&  28.87&  31.80&  25.14&  22.81&   0.00&   0.00&   0.00&   0.00&   0.57&   0.19&   0.00&   0.00 \\ 
 627& 145555.006+622307.12&   0.00&  43.99&  30.13&  71.11&  64.98&  51.52&  40.96&   0.00&  23.03&  15.35&   8.42&   1.67&   0.61&   0.35&   0.39 \\ 
 628& 145934.022+371953.81&   0.00&   9.36&  19.50&  36.23&  47.25&  41.64&  35.78&   0.00&  21.06&  12.89&   9.52&   1.63&   0.67&   0.19&   0.00 \\ 
 629& 145939.811+021804.20&  11.37&   7.02&  10.44&  22.58&  21.81&  17.49&  14.26&  11.75&   8.01&   5.84&   2.39&   0.51&   0.16&   0.07&   0.00 \\ 
 630& 150522.258+072334.96&   4.98&  12.11&  15.30&  42.60&  43.00&  34.12&  27.20&  24.80&  18.87&  13.09&   6.29&   1.50&   0.56&   0.09&   0.00 \\ 
 631& 150546.274+245406.85&   0.00&   0.00&   3.14&   6.65&  12.82&  11.06&   9.37&   0.00&   0.00&   0.00&   0.00&   0.65&   0.22&   0.00&   0.00 \\ 
 632& 150604.202+300229.13&   0.00&   9.30&  13.11&  28.88&  40.35&  35.82&  29.15&   0.00&  21.10&  15.05&   9.38&   1.74&   0.69&   0.00&   0.00 \\ 
 633& 150635.563+321035.77&   0.00&  27.77&  29.78&  68.94&  71.65&  59.50&  51.32&  41.39&  31.87&  21.36&  10.68&   2.24&   0.77&   0.10&   0.09 \\ 
 634& 150724.302+413556.51&   0.00&  12.33&  15.93&  36.18&  45.92&  38.46&  31.75&   0.00&  20.41&  19.78&  11.92&   1.88&   0.75&   0.04&   0.00 \\ 
 635& 150926.474+152132.04&   0.00&  11.07&  11.52&  26.23&  33.22&  28.76&  22.81&   0.00&  21.28&  14.42&   9.98&   1.95&   0.79&   0.06&   0.00 \\ 
 636& 151010.680+182242.74&   0.00&  23.74&  48.70&  68.23&  71.50&  57.13&  46.25&   0.00&  22.71&  18.52&   6.45&   1.83&   0.69&   0.45&   0.14 \\ 
 637& 151025.534+092459.09&   0.00&  45.66&  47.25& 115.50& 117.80&  97.16&  74.53&  66.49&  50.39&  34.17&  17.31&   3.56&   1.23&   0.26&   0.00 \\ 
 638& 151052.826+095534.44&  54.78&  37.71&  31.15&  57.73&  63.70&  54.43&  43.83&  35.63&  28.08&  18.93&  10.65&   2.33&   0.95&   0.46&   0.10 \\ 
 639& 151105.964+550605.28&   0.00&  15.40&   9.75&  11.33&  13.84&  10.54&   8.24&   0.00&   0.00&   0.00&   0.00&   0.53&   0.18&   0.00&   0.08 \\ 
 640& 151111.402+054027.02&   0.00&  28.24&  41.01&  86.72&  75.83&  59.61&  50.31&  37.49&  25.36&  19.13&   8.43&   1.73&   0.53&   0.12&   0.00 \\ 
 641& 151151.362+230903.77&   0.00&   0.00& 416.30& 747.80& 673.80& 570.20& 467.70&   0.00& 376.50& 233.00& 121.80&  20.75&   6.47&   4.12&   2.65 \\ 
 642& 151248.146+160001.69&   0.00&  16.29&  15.40&  26.99&  29.71&  26.37&  18.89&   0.00&  14.79&   9.89&   6.41&   0.96&   0.36&   0.13&   0.12 \\ 
 643& 151354.677+553302.44&   0.00&   0.00&   6.33&  23.17&  34.42&  31.25&  26.96&   0.00&  22.50&  11.92&   8.74&   1.46&   0.61&   0.08&   0.00 \\ 
 644& 151433.674+025728.23&   0.00&   9.67&  22.02&  60.86&  66.09&  52.98&  47.89&  41.73&  33.28&  23.35&  11.49&   2.83&   1.06&   0.17&   0.00 \\ 
 645& 151528.812+325813.42&   0.00&   9.07&  14.50&  36.27&  36.85&  30.66&  25.66&   0.00&  17.74&  12.16&   6.58&   1.29&   0.44&   0.12&   0.00 \\ 
 646& 151550.506+060114.31&   0.00&   3.74&   7.99&  22.94&  23.71&  19.94&  16.19&   0.00&  11.96&  10.00&   5.32&   1.09&   0.35&   0.00&   0.00 \\ 
 647& 151552.030+312322.50&   0.00&   0.00&  24.68&  53.64&  50.93&  42.36&  36.45&   0.00&  24.24&  17.54&  10.09&   1.74&   0.55&   0.09&   0.00 \\ 
 648& 151711.479+265804.35&   0.00&   8.28&  10.27&  30.24&  33.56&  29.02&  24.35&   0.00&  13.73&   9.16&   0.00&   0.96&   0.33&   0.13&   0.00 \\ 
 649& 151742.415+484843.65&   0.00&  12.53&  31.91&  65.26&  66.57&  55.77&  46.44&   0.00&  19.36&  12.01&   6.62&   1.61&   0.52&   0.20&   0.09 \\ 
 650& 151743.608+284654.25&   0.00&   0.00&  14.38&  27.85&  27.99&  21.55&  17.44&   0.00&   9.79&   9.23&   6.06&   0.88&   0.33&   0.00&   0.00 \\ 
 651& 151845.850+233536.81&   0.00&   0.00&  11.03&  21.46&  30.96&  26.69&  22.06&   0.00&  14.78&  11.49&   8.02&   1.26&   0.50&   0.08&   0.00 \\ 
 652& 151915.545+162415.88& 175.00& 150.10&  94.53& 153.60& 136.20& 107.70&  86.40&   0.00&  45.56&  31.52&  19.70&   3.87&   1.45&   0.68&   0.30 \\ 
 653& 152038.333+215254.26&   0.00&   9.15&  20.26&  46.60&  50.74&  43.05&  37.90&   0.00&  21.77&  17.93&  11.08&   1.78&   0.60&   0.11&   0.00 \\ 
 654& 152057.010+371520.39&  84.39& 106.00&  61.09& 107.30&  91.38&  68.85&  50.46&   0.00&  32.92&  19.97&  10.39&   2.24&   0.85&   0.30&   0.24 \\ 
 655& 152058.913+421254.39&   0.00&   3.94&   9.45&  23.64&  25.72&  21.79&  17.86&   0.00&  14.55&   8.94&   4.35&   1.04&   0.35&   0.09&   0.00 \\ 
 656& 152139.418+205923.22&   0.00&   0.00&  11.09&  23.11&  33.47&  30.06&  23.94&   0.00&  15.83&   8.65&   6.21&   1.46&   0.59&   0.06&   0.00 \\ 
 657& 152159.186+021022.45&  61.09& 141.40& 124.10& 216.10& 189.20& 143.80&  99.87&  94.43&  66.08&  46.88&  24.62&   4.30&   1.69&   1.06&   0.39 \\ 
 658& 152236.773-015035.89&   0.00&   2.43&   5.27&  17.27&  21.47&  20.45&  17.36&  16.00&  13.90&   9.62&   5.06&   1.08&   0.37&   0.14&   0.00 \\ 
 659& 152321.888+140922.96&   0.00&   6.06&  12.51&  25.83&  30.92&  27.10&  22.44&   0.00&  20.96&   8.31&   6.88&   1.24&   0.46&   0.09&   0.00 \\ 
 660& 152351.432+084734.68&   0.00&  27.30&  26.59&  62.16&  50.05&  37.33&  30.92&  17.84&  12.13&   8.00&   3.59&   0.61&   0.20&   0.00&   0.00 \\ 
 661& 152419.411+054415.06&   0.00&  31.03&  25.19&  53.90&  44.53&  32.67&  27.08&  22.69&  18.07&  12.13&   6.46&   1.39&   0.48&   0.15&   0.18 \\ 
 662& 152426.506+080908.04& 164.60& 377.70& 222.90& 413.90& 327.80& 250.70& 193.50& 151.40& 119.20&  78.17&  38.01&   8.64&   3.02&   1.48&   1.05 \\ 
 663& 152507.925+213353.71&   0.00&   0.00&  11.64&  23.35&  26.84&  21.97&  21.75&   0.00&  13.19&   7.55&   4.76&   0.86&   0.27&   0.05&   0.00 \\ 
 664& 152541.561+260225.17&   0.00&   0.00&  26.45&  50.60&  52.76&  41.37&  33.66&   0.00&  19.50&  14.27&   8.20&   1.60&   0.63&   0.24&   0.00 \\ 
 665& 152633.046+064053.43&  19.68&  29.47&  67.85& 134.00& 129.10& 106.70&  92.09&  74.12&  56.59&  38.44&  16.97&   3.15&   0.96&   0.09&   0.00 \\ 
 666& 152847.789+032321.28&   0.00&   9.51&   5.74&  15.86&  29.05&  26.88&  22.42&  17.68&  14.56&  11.00&   6.70&   1.50&   0.56&   0.00&   0.00 \\ 
 667& 152859.100+245646.77&   0.00&  13.15&  12.24&  34.03&  40.09&  33.45&  28.40&   0.00&  18.85&  13.02&   7.01&   1.37&   0.51&   0.07&   0.00 \\ 
 668& 152906.422+543337.66&   0.00&   0.00&   7.95&  19.84&  26.77&  22.66&  19.30&   0.00&  13.27&   8.04&   6.50&   1.16&   0.41&   0.06&   0.00 \\ 
 669& 152929.902+271205.43&   0.00&   0.00&  77.76& 149.90& 125.90& 103.50&  76.82&   0.00&  81.25&  52.66&  24.77&   4.30&   1.33&   0.22&   0.19 \\ 
 670& 153004.238+413203.25&   0.00&   0.00&   9.16&  23.13&  29.25&  24.67&  20.82&   0.00&  14.47&   8.51&   5.65&   1.19&   0.45&   0.08&   0.00 \\ 
 671& 153016.063+373346.16&   0.00&   0.00& 141.20& 251.80& 214.00& 167.70& 132.00&   0.00&  84.63&  52.82&  29.30&   8.11&   4.06&   1.66&   1.36 \\ 
 672& 153057.062+304324.72&   0.00&   0.00&   2.06&   4.43&   9.28&   7.84&   6.20&   0.00&   0.00&   0.00&   0.00&   7.70&   3.96&   1.93&   1.38 \\ 
 673& 153144.602+064304.27&   0.00&   0.00&  45.15& 119.90& 105.10&  80.69&  61.63&  46.68&  37.99&  21.47&  11.78&   2.76&   1.05&   0.51&   0.33 \\ 
 674& 153344.952+121557.16&  20.00&  25.85&  19.48&  34.56&  34.50&  28.56&  23.85&   0.00&  15.10&   9.64&   4.41&   1.08&   0.44&   0.18&   0.22 \\ 
 675& 153426.004+173747.13& 255.90& 199.40& 146.50& 212.40& 176.40& 141.20& 114.90&   0.00&  78.48&  51.12&  25.92&   5.58&   1.77&   0.61&   0.32 \\ 
 676& 153507.114+202743.09&   0.00&  46.32&  37.43&  65.10&  74.47&  61.33&  49.67&   0.00&  22.73&  16.07&  12.69&   2.09&   0.86&   0.36&   0.10 \\ 
 677& 153534.061+123410.18&  38.46&   0.00&  67.04& 139.60& 131.40& 105.70&  86.25&   0.00&  53.10&  33.65&  18.14&   4.17&   1.51&   0.40&   0.21 \\ 
 678& 153703.367+135944.15&  52.67& 133.10& 127.90& 271.80& 228.60& 178.90& 138.80&   0.00&  92.78&  56.49&  32.35&   7.41&   5.04&   3.37&   3.34 \\ 
 679& 153724.245-015317.93&   0.00&  16.90&  20.18&  36.40&  36.55&  30.10&  23.25&  19.08&  14.88&  10.08&   5.53&   1.13&   0.39&   0.00&   0.00 \\ 
 680& 153852.301+253945.69&   0.00&   0.00&   7.52&  18.03&  28.58&  24.70&  20.74&   0.00&  15.74&  10.38&   6.88&   1.40&   0.55&   0.00&   0.00 \\ 
 681& 153854.842+171259.05&  98.81&   0.00&  58.13& 120.20& 122.80& 103.00&  80.61&   0.00&  52.44&  33.17&  22.33&   4.31&   1.67&   0.83&   0.30 \\ 
 682& 154012.458+072841.27&   0.00&  43.26&  39.08&  67.62&  73.79&  62.79&  51.61&  42.38&  32.83&  22.76&  12.65&   2.70&   1.00&   0.00&   0.00 \\ 
 683& 154128.740-014346.89&   0.00&   0.00&  26.74&  56.77&  57.24&  47.80&  40.92&  32.65&  25.40&  18.73&  10.00&   2.28&   0.83&   0.44&   0.27 \\ 
 684& 154224.125+234053.94&   0.00&  11.71&   0.00&  21.02&  35.25&  29.89&  25.42&   0.00&  14.75&  12.49&   7.66&   1.51&   0.60&   0.12&   0.00 \\ 
 685& 154228.282+431538.39& 123.30&   0.00&  53.17&  75.77&  69.61&  56.38&  45.28&   0.00&  28.84&  21.58&   9.74&   2.49&   0.97&   0.50&   0.31 \\ 
 686& 154234.522+211120.67&   0.00&   0.00&   7.75&  20.77&  23.41&  19.38&  17.02&   0.00&  12.13&   7.16&   4.04&   0.89&   0.31&   0.04&   0.00 \\ 
 687& 154322.404+331018.62&   0.00&   9.83&  18.25&  33.87&  36.45&  30.71&  26.40&   0.00&  15.20&  13.22&   7.60&   1.30&   0.45&   0.09&   0.07 \\ 
 688& 154401.810+180805.27&   0.00&   0.00&  12.24&  22.17&  30.55&  27.15&  23.35&   0.00&  18.07&  14.90&   7.94&   1.73&   0.74&   0.06&   0.00 \\ 
 689& 154518.526+354220.10&   0.00&   0.00&  32.00&  36.59&  39.09&  32.33&  29.11&   0.00&   0.00&   0.00&   0.00&   0.86&   0.28&   0.06&   0.00 \\ 
 690& 154520.782+345251.07&   0.00&   7.51&  17.06&  36.96&  44.24&  35.34&  26.29&   0.00&  15.44&   9.84&   6.34&   1.37&   0.56&   0.00&   0.10 \\ 
 691& 154715.816+443343.11&   0.00&   8.34&  13.35&  33.09&  33.55&  27.88&  20.23&   0.00&  18.60&  10.37&   4.80&   1.08&   0.38&   0.09&   0.10 \\ 
 692& 154733.650+051753.28&   0.00&  54.45&  30.76&  50.02&  46.04&  34.32&  26.19&  21.62&  16.40&  11.25&   6.38&   1.36&   0.54&   0.18&   0.25 \\ 
 693& 154806.173+142227.12&   0.00&   0.00&  14.00&  34.57&  30.85&  26.32&  18.90&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00&   0.00 \\ 
 694& 154810.771+191229.34&   0.00&   6.60&  20.78&  48.89&  47.50&  38.39&  31.28&   0.00&  20.14&  15.57&   9.09&   1.60&   0.57&   0.00&   0.00 \\ 
 695& 154859.695+105950.90&   0.00&   0.00&  22.65&  46.32&  44.98&  37.67&  31.00&   0.00&  22.09&   8.80&   5.99&   1.38&   0.46&   0.31&   0.28 \\ 
 696& 154917.702+470505.04&   0.00&  16.42&  28.78&  53.00&  57.25&  46.82&  38.60&   0.00&  25.79&  13.30&   9.49&   1.70&   0.62&   0.09&   0.00 \\ 
 697& 154919.351+572321.03&   0.00&   4.03&   7.02&  20.79&  31.08&  27.63&  23.78&   0.00&  16.19&  11.94&   7.67&   1.48&   0.63&   0.08&   0.06 \\ 
 698& 154944.938+133437.51&   0.00&   7.92&  11.22&  30.52&  40.44&  35.49&  33.75&   0.00&  20.68&  10.24&   9.42&   1.85&   0.82&   0.00&   0.00 \\ 
 699& 155004.610+303502.54&   0.00&  11.07&  11.55&  27.45&  32.70&  27.42&  23.81&   0.00&  14.10&   0.00&   0.00&   1.14&   0.47&   0.13&   0.00 \\ 
 700& 155016.526+194923.99&   0.00&   6.17&  17.04&  45.34&  56.79&  49.46&  45.60&   0.00&  26.86&  17.31&  10.99&   2.32&   0.82&   0.08&   0.00 \\ 
 701& 155054.050+422540.42&   0.00&   0.00&  21.17&  47.68&  48.92&  40.67&  34.84&   0.00&  21.42&  16.15&   6.92&   1.43&   0.52&   0.05&   0.00 \\ 
 702& 155125.817+135031.73&   0.00&   0.00&  13.48&  34.50&  41.15&  34.90&  30.15&   0.00&  16.13&  10.97&   7.39&   1.49&   0.59&   0.09&   0.00 \\ 
 703& 155159.849+004444.29&   0.00&   0.00&  35.58&  40.61&  52.55&  45.09&  41.54&  36.15&  26.38&  15.51&   9.01&   1.62&   0.65&   0.24&   0.19 \\ 
 704& 155353.419+141534.45&   4.89&  17.11&  41.62& 103.10& 105.50&  88.44&  73.76&   0.00&  50.43&  27.45&  17.42&   3.54&   1.20&   0.11&   0.00 \\ 
 705& 155406.770+444130.14&   0.00&  17.71&  26.07&  53.44&  52.08&  41.19&  34.24&   0.00&  24.45&  17.42&   8.03&   1.55&   0.51&   0.04&   0.00 \\ 
 706& 155435.539+291319.92&  53.59&  71.77& 161.40& 314.80& 334.20& 276.90& 228.50&   0.00& 115.30&  74.50&  41.60&   6.81&   2.30&   0.51&   0.08 \\ 
 707& 155523.753+023932.98&   0.00&  12.85&   5.48&  19.32&  23.87&  20.31&  17.24&   0.00&  12.01&   6.51&   6.51&   1.02&   0.42&   0.14&   0.00 \\ 
 708& 155545.110+082439.95&   0.00&   0.00&  21.84&  48.77&  52.73&  45.50&  39.15&  30.07&  22.65&  17.05&   8.26&   1.74&   0.62&   0.00&   0.00 \\ 
 709& 155555.582+214431.80&   0.00&   0.00&  27.73&  53.88&  51.73&  44.30&  39.41&   0.00&  29.58&  19.35&   9.37&   2.04&   1.47&   0.99&   2.28 \\ 
 710& 155650.011+165925.23&  42.65&  48.72&  29.27&  43.46&  43.98&  32.74&  24.72&   0.00&  18.06&   8.17&   8.84&   1.39&   0.57&   0.31&   0.22 \\ 
 711& 155728.906+472004.91&   0.00&  13.87&  17.17&  40.12&  44.32&  37.32&  29.92&   0.00&  13.54&  10.51&   5.20&   1.39&   0.54&   0.10&   0.00 \\ 
 712& 155742.074+392655.56&   0.00&  22.79&  41.84& 107.00& 114.10&  96.53&  81.98&   0.00&  49.09&  33.73&  18.88&   3.47&   1.14&   0.13&   0.00 \\ 
 713& 155815.722+180208.51&   0.00&   0.00&  11.30&  44.68&  42.79&  35.03&  31.14&   0.00&  17.57&  10.60&   3.79&   1.00&   0.35&   0.09&   0.00 \\ 
 714& 160014.062+050339.47&   0.00&   0.00&   8.89&  19.59&  26.90&  23.05&  19.86&   0.00&  13.25&   5.42&   6.96&   1.18&   0.44&   0.00&   0.00 \\ 
 715& 160022.670+124527.99&   0.00&  50.58& 118.70& 261.00& 250.30& 210.70& 176.30&   0.00& 117.10&  70.68&  39.28&   6.32&   1.99&   0.13&   0.00 \\ 
 716& 160051.494+150904.56&  71.85& 109.20& 266.10& 572.90& 555.10& 479.10& 397.00&   0.00& 224.00& 136.20&  66.75&  11.23&   3.38&   0.80&   0.15 \\ 
 717& 160151.384+042222.15&  36.64&  48.48&  37.77&  64.30&  61.35&  49.73&  41.62&   0.00&  29.17&  19.63&  11.71&   2.05&   0.76&   0.30&   0.24 \\ 
 718& 160154.204+160016.80&  25.60&  36.90&  28.79&  47.85&  34.18&  24.39&  15.92&   0.00&   0.00&   0.00&   0.00&   0.45&   0.14&   0.00&   0.00 \\ 
 719& 160154.746+204410.08&   0.00&   5.81&  12.88&  27.94&  29.10&  24.86&  21.17&   0.00&  17.12&  11.26&   4.99&   0.97&   0.30&   0.00&   0.00 \\ 
 720& 160156.700+122453.90&   0.00&  19.02&  24.66&  56.05&  57.54&  48.56&  41.39&   0.00&  28.31&  19.49&   7.52&   1.87&   0.66&   0.20&   0.14 \\ 
 721& 160210.668+024505.15&   0.00&  13.40&  18.32&  37.88&  46.38&  36.37&  29.11&   0.00&  16.03&   9.86&   7.56&   1.51&   0.62&   0.08&   0.00 \\ 
 722& 160229.244+335736.10&   0.00&   0.00&  17.79&  48.48&  48.30&  40.35&  35.14&   0.00&  23.14&  15.37&   8.26&   1.79&   0.62&   0.26&   0.18 \\ 
 723& 160303.636+214150.87&  21.11&  48.19& 100.20& 213.30& 188.80& 140.90&  97.57&   0.00&  73.92&  50.00&  24.31&   4.39&   1.34&   0.00&   0.12 \\ 
 724& 160343.330+101958.38&   0.00&   4.81&  10.59&  16.70&  24.90&  22.18&  18.92&   0.00&   0.00&   0.00&   0.00&   0.98&   0.39&   0.10&   0.00 \\ 
 725& 160417.304+155503.82&   0.00&   0.00&   0.00&  31.94&  39.19&  33.70&  32.67&   0.00&   0.00&   0.00&   0.00&   0.62&   0.16&   0.00&   0.00 \\ 
 726& 160448.737+170327.00&   0.00&  12.91&  18.58&  38.03&  42.45&  36.39&  31.30&   0.00&  22.67&  17.43&   9.40&   1.75&   0.78&   0.26&   0.00 \\ 
 727& 160614.844+205011.37&   0.00&   0.00&   4.19&  14.54&  22.25&  21.21&  19.99&   0.00&  14.88&  10.73&   6.42&   1.38&   0.57&   0.17&   0.13 \\ 
 728& 160630.118+183515.53&   0.00&  10.28&  23.18&  52.60&  49.88&  41.20&  35.38&   0.00&  28.18&  15.85&   9.05&   1.65&   0.52&   0.11&   0.00 \\ 
 729& 160724.758+114154.41&   0.00&   6.76&  12.74&  26.02&  30.50&  23.88&  19.31&   0.00&  11.10&   8.36&   0.00&   1.08&   0.42&   0.00&   0.00 \\ 
 730& 160740.301+203630.02&   0.00&   0.00&   4.77&  14.24&  19.75&  18.25&  16.48&   0.00&  11.98&   7.82&   5.72&   0.92&   0.35&   0.00&   0.00 \\ 
 731& 160808.717+394755.92&  50.14&  37.20&  31.21&  61.61&  63.97&  51.81&  41.79&   0.00&  28.78&  14.06&  12.08&   2.12&   0.83&   0.14&   0.00 \\ 
 732& 160812.264+155913.55&   0.00&   4.82&   8.31&  19.90&  26.95&  22.95&  19.11&   0.00&  12.50&   9.75&   5.87&   1.13&   0.44&   0.00&   0.00 \\ 
 733& 160813.092+362255.19&   0.00&  11.79&  19.53&  38.66&  37.96&  31.01&  26.40&   0.00&  21.21&  10.70&   6.33&   1.27&   0.44&   0.14&   0.13 \\ 
 734& 161122.747+091558.05&   0.00&  14.64&  24.28&  49.53&  52.05&  42.32&  35.76&   0.00&  22.33&  14.19&   6.77&   1.55&   0.54&   0.08&   0.00 \\ 
 735& 161129.184+331434.13&   0.00&  29.73&   9.92&  14.84&  22.02&  15.50&  11.19&   0.00&   9.12&   0.00&   0.00&   1.49&   0.76&   0.42&   0.17 \\ 
 736& 161330.187+510335.57& 457.80& 479.20& 226.70& 370.40& 271.50& 196.30& 137.70&   0.00&  46.52&  22.09&  12.06&   2.30&   0.77&   0.40&   0.14 \\ 
 737& 161446.824+085606.53& 117.30&  97.89&  37.53&  53.19&  44.30&  35.35&  28.21&   0.00&  17.30&  10.44&   7.23&   1.38&   0.46&   0.00&   0.00 \\ 
 738& 161756.021+092035.67&   0.00&   6.51&  12.21&  28.27&  29.21&  24.49&  21.40&   0.00&  16.17&   8.30&   5.57&   1.04&   0.28&   0.08&   0.00 \\ 
 739& 161816.466+094506.37&   0.00&  20.17&  33.23&  75.40&  76.28&  62.26&  51.55&   0.00&  35.71&  21.43&   9.97&   2.33&   0.78&   0.07&   0.00 \\ 
 740& 161925.980+215939.96&   0.00&   5.14&  13.77&  33.07&  34.18&  28.56&  24.93&   0.00&  17.30&  10.72&   6.83&   1.73&   0.82&   0.45&   0.50 \\ 
 741& 162049.637+160944.45&   0.00&   0.00&   9.99&  31.01&  35.72&  30.61&  27.03&   0.00&  18.20&  11.44&   3.11&   1.26&   0.45&   0.34&   0.22 \\ 
 742& 162100.811+211006.10&  32.13&  82.12& 252.40& 569.10& 564.40& 465.00& 377.10&   0.00& 247.90& 159.40&  76.73&  11.83&   3.68&   0.68&   0.32 \\ 
 743& 162124.029+075947.78&  29.63&  46.25&  49.87& 109.60& 103.80&  81.33&  61.63&   0.00&  35.68&  24.72&  18.19&   2.64&   0.89&   0.25&   0.00 \\ 
 744& 162200.283+235531.84&   0.00&  11.41&  15.12&  37.42&  36.41&  29.96&  23.57&  19.24&  14.35&  11.12&   5.24&   1.08&   0.34&   0.18&   0.15 \\ 
 745& 162205.705+185950.58&   0.00&   0.00&  28.25&  46.94&  44.47&  35.64&  29.04&   0.00&  16.44&   6.86&   7.59&   1.28&   0.44&   0.24&   0.16 \\ 
 746& 162415.134+170105.53&   0.00&   0.00& 122.60& 227.00& 173.20& 127.30&  55.14&   0.00&   0.00&   0.00&   0.00&   1.01&   0.27&   0.13&   0.00 \\ 
 747& 162440.783+081727.79&   0.00&   8.41&  11.56&  31.08&  31.56&  25.16&  21.10&   0.00&  14.28&   7.62&   4.21&   0.97&   0.34&   0.19&   0.00 \\ 
 748& 162503.350+070402.94&   0.00&   0.00&  22.88&  44.02&  43.59&  36.41&  30.30&   0.00&  18.23&  11.95&   5.87&   1.21&   0.38&   0.16&   0.00 \\ 
 749& 162507.680+091714.28&   0.00&  35.20&  35.80&  57.60&  52.71&  38.60&  29.63&   0.00&  11.27&   7.10&   4.75&   1.15&   0.47&   0.00&   0.00 \\ 
 750& 162702.561+432833.94&  81.10& 151.60& 251.90& 610.00& 611.80& 522.60& 433.00&   0.00& 271.00& 170.30&  90.52&  14.16&   4.11&   0.80&   0.20 \\ 
 751& 162718.799+255229.63&   0.00&  11.53&  17.55&  35.20&  38.33&  31.66&  26.85&  21.68&  16.04&  12.25&   5.98&   1.33&   0.53&   0.23&   0.13 \\ 
 752& 162740.726+132634.53&   0.00&   0.00&  16.91&  50.75&  50.85&  41.86&  32.53&   0.00&  25.53&  12.22&   8.13&   1.73&   0.56&   0.34&   0.27 \\ 
 753& 162755.956+480051.14&   2.67&  12.88&  12.15&  29.05&  31.67&  26.92&  23.13&   0.00&  15.84&   0.00&   6.89&   1.19&   0.44&   0.09&   0.00 \\ 
 754& 162800.151+413335.35&   0.00&   5.03&   6.72&  15.15&  24.64&  22.23&  20.15&   0.00&  14.09&  11.27&   8.02&   1.67&   0.68&   0.26&   0.11 \\ 
 755& 162930.528+423447.31&   0.90&   5.67&  17.31&  40.16&  43.14&  36.64&  31.81&   0.00&  20.75&  14.21&   8.78&   1.54&   0.55&   0.00&   0.00 \\ 
 756& 162938.266+302924.92&   0.00&  18.50&  42.09& 110.80& 121.80& 106.80&  93.50&  76.13&  59.63&  41.05&  20.91&   4.46&   1.45&   0.20&   0.00 \\ 
 757& 163159.906+431754.46&   0.00&   0.00&   7.68&  17.82&  26.36&  23.99&  21.21&   0.00&  12.95&  13.04&   7.27&   1.38&   0.53&   0.06&   0.00 \\ 
 758& 163214.198+241150.97&   0.00&  21.13&  25.17&  42.77&  38.08&  31.22&  24.67&   0.00&  16.07&   9.43&   3.58&   0.95&   0.29&   0.06&   0.00 \\ 
 759& 163607.692+284408.39&   0.00&   0.00&  28.42&  76.17&  92.29&  79.01&  61.65&  40.64&  34.87&  23.05&  12.41&   2.48&   0.89&   0.11&   0.00 \\ 
 760& 163658.750+173946.79&   0.00&   0.00&  51.13& 117.50& 122.70&  97.77&  86.32&   0.00&  56.82&  30.30&  21.14&   4.15&   1.59&   0.69&   0.00 \\ 
 761& 163835.054+440349.43&   0.00&   0.00&  20.87&  44.48&  43.77&  37.00&  29.23&   0.00&  16.69&  17.33&   6.99&   1.68&   0.57&   0.31&   0.16 \\ 
 762& 163859.402+250402.91&  50.05&  24.56&  23.66&  32.62&  38.33&  29.51&  24.81&   0.00&  16.00&   9.42&   6.70&   1.28&   0.56&   0.26&   0.15 \\ 
 763& 163916.397+273333.90&   0.00&  23.57&  29.59&  73.47&  71.72&  56.53&  46.01&  40.84&  30.23&  22.15&  10.14&   2.46&   0.80&   0.10&   0.00 \\ 
 764& 164255.162+415335.63&   5.04&  33.49&  53.95& 132.20& 123.70& 100.30&  81.00&   0.00&  61.32&  33.56&  19.31&   4.12&   1.49&   0.33&   0.13 \\ 
 765& 164300.041+281944.61&   0.00&  81.90&  65.08& 182.30& 187.40& 149.80& 109.60&  83.55&  64.57&  43.33&  20.71&   4.10&   1.62&   0.14&   0.00 \\ 
 766& 164608.266+363705.21&   0.00&  24.73&  20.16&  79.06&  95.01&  90.10&  55.61&   0.00&  31.53&  19.85&  12.87&   2.38&   0.83&   0.26&   0.00 \\ 
 767& 164610.478+324258.73&   0.00&   6.91&   6.29&  21.08&  23.32&  20.14&  17.01&   0.00&  15.08&   9.49&   6.31&   1.20&   0.49&   0.00&   0.00 \\ 
 768& 165030.946+295601.02&   0.00&  19.23&  25.20&  49.71&  49.79&  39.85&  33.11&  26.67&  19.99&  12.98&   6.55&   1.38&   0.55&   0.19&   0.00 \\ 
 769& 165437.337+295415.33&   0.00&   0.00&   0.00& 184.50& 147.00& 101.80&  67.07&   0.00&  34.19&  25.54&  14.11&   2.57&   0.95&   0.53&   0.00 \\ 
 770& 165639.288+184021.69&   0.00& 101.10&  25.58&  53.40&  49.97&  38.64&   0.00&   0.00&  22.58&  10.66&   6.98&   3.46&   1.01&   0.12&   0.00 \\ 
 771& 165648.641+314702.38&  87.94& 117.60&  24.54&  68.83&  71.85&  59.23&  47.11&   0.00&  40.75&  26.36&  14.68&   3.01&   1.10&   0.53&   0.40 \\ 
 772& 165804.771+632608.97&  29.15&  31.79&  46.56&  99.15& 101.20&  84.74&  73.70&   0.00&  47.35&  28.69&  16.80&   2.30&   0.92&   0.27&   0.00 \\ 
 773& 165820.664+245628.86&  22.38&  33.67&  28.43&  60.07&  72.92&  61.15&  44.06&   0.00&  35.93&  20.81&  11.27&   1.27&   0.46&   0.23&   0.00 \\ 
 774& 165902.064+371514.36&   0.00&  20.50&   8.61&  24.21&  26.11&  22.26&  18.42&   0.00&  11.05&  11.05&   5.90&   2.55&   1.02&   0.58&   0.19 \\ 
 775& 165958.032+213640.06&   0.00&  60.33&  77.23& 125.10& 118.50&  92.14&  68.00&   0.00&  42.40&  22.79&  15.26&   1.72&   0.63&   0.10&   0.18 \\ 
 776& 170057.230+601924.84&   0.00&  13.65&  19.52&  46.59&  50.55&  43.58&  37.35&   0.00&  20.90&  13.57&   4.11&   1.30&   0.49&   0.08&   0.00 \\ 
 777& 170128.190+190337.74&   0.00&   0.00&   7.91&  15.88&  25.29&  22.10&  18.65&   0.00&  14.64&   9.78&   5.39&   1.42&   0.55&   0.28&   0.07 \\ 
 778& 170252.474+630710.07&   0.00&  15.60&  19.23&  34.86&  38.62&  33.61&  28.87&   0.00&  15.46&  11.43&   5.95&   0.94&   0.35&   0.19&   0.09 \\ 
 779& 170356.712+622848.28&   0.00&  19.69&  10.33&  24.42&  26.96&  22.36&  20.06&   0.00&  10.85&   5.55&   2.87&   2.06&   0.71&   0.09&   0.05 \\ 
 780& 170557.425+630055.58&  13.66&  31.20&  38.57&  81.76&  73.97&  57.22&  45.48&   0.00&  33.64&  23.71&   9.50&   2.54&   0.95&   0.32&   0.05 \\ 
 781& 170636.588+334720.44&   0.00&  35.91&  51.49& 101.80& 104.10&  85.89&  67.88&   0.00&  31.08&  23.05&  11.89&   1.49&   0.53&   0.00&   0.00 \\ 
 782& 171430.331+321508.77&   0.00&   0.00&  15.69&  39.56&  42.33&  34.29&  28.71&   0.00&  19.59&  11.83&   7.21&   0.99&   0.36&   0.07&   0.00 \\ 
 783& 171546.258+582255.47&   0.00&  15.84&  17.82&  35.73&  36.20&  30.52&  26.60&   0.00&  13.82&   9.79&   4.02&   3.32&   1.28&   0.34&   0.17 \\ 
 784& 172010.834+274214.75& 111.40&  96.70&  54.51& 103.60& 104.90&  87.15&  71.11&   0.00&  46.68&  28.49&  20.18&   0.90&   0.34&   0.05&   0.04 \\ 
 785& 172036.091+631722.47&   0.00&   3.19&   8.29&  20.68&  24.90&  21.03&  18.21&   0.00&  11.28&   9.41&   5.60&   0.89&   0.34&   0.05&   0.04 \\ 
 786& 173139.158+544631.48&   0.00&   0.00&  43.37&  69.21&  65.79&  53.23&  45.43&   0.00&  28.15&  16.28&  10.48&   2.08&   0.77&   0.51&   0.28 \\ 
 787& 174133.046+540325.42&   0.00&  27.09&  25.54&  49.51&  44.77&  35.75&  29.19&   0.00&  12.74&   8.04&   6.25&   1.17&   0.41&   0.13&   0.00 \\ 
 788& 210443.855-073145.45&   0.00&  13.83&  13.51&  20.41&  36.10&  34.74&  30.56&   0.00&  18.52&  13.95&   7.09&   1.96&   0.71&   0.12&   0.13 \\ 
 789& 211230.600-005022.42&   0.00&  81.94&  22.94&  47.96&  50.52&  39.69&  33.13&  20.35&  16.58&   9.81&   5.84&   1.26&   0.52&   0.16&   0.00 \\ 
 790& 211348.163-063059.63&   0.00&  20.26&  36.67&  53.16&  57.95&  50.91&  38.36&   0.00&  29.74&   9.92&  11.56&   1.77&   0.68&   0.16&   0.00 \\ 
 791& 211948.178+004021.76&   0.00&   6.66&  23.83&  50.31&  54.95&  46.69&  39.00&  23.67&  18.54&  13.74&   5.55&   1.03&   0.31&   0.00&   0.00 \\ 
 792& 212036.403-063722.61&   0.00&   0.00&   6.22&  18.40&  23.69&  21.16&  18.36&   0.00&  15.39&  11.83&   4.86&   0.97&   0.38&   0.07&   0.00 \\ 
 793& 212233.367+010016.52&  33.52&  33.50&  23.38&  37.46&  40.57&  33.01&  27.16&  20.35&  16.33&  11.89&   6.39&   1.69&   0.86&   0.32&   0.00 \\ 
 794& 213556.916+000328.71&   4.15&  10.28&  17.64&  35.18&  33.57&  27.21&  23.00&  20.27&  14.90&  10.65&   4.90&   1.00&   0.34&   0.00&   0.00 \\ 
 795& 214307.529-080727.48&   0.00&   6.48&  19.92&  32.70&  48.70&  46.08&  36.23&   0.00&  24.82&  13.07&  10.55&   1.91&   0.68&   0.00&   0.00 \\ 
 796& 214456.719-070708.13&   0.00&  13.12&  16.62&  37.66&  38.35&  31.79&  25.30&   0.00&  20.18&  12.55&   3.20&   1.10&   0.39&   0.14&   0.00 \\ 
 797& 215735.446-005021.44&   0.00&   7.20&   7.99&  20.71&  31.36&  28.10&  22.12&  20.46&  18.29&  14.98&   6.92&   2.16&   0.82&   0.22&   0.00 \\ 
 798& 220122.889+002516.09&   0.00&   5.20&   6.50&  19.89&  30.48&  27.77&  23.53&  19.16&  16.77&  10.34&   6.32&   1.38&   0.56&   0.00&   0.00 \\ 
 799& 220545.533-092916.59&   5.51&   8.46&  12.31&  28.35&  29.99&  23.94&  19.47&   0.00&  13.21&   9.23&   3.73&   0.85&   0.36&   0.00&   0.00 \\ 
 800& 223138.119-080652.61&   0.00&   7.06&   5.41&  18.49&  22.51&  20.95&  19.66&   0.00&   7.49&   6.22&   2.64&   0.86&   0.31&   0.00&   0.00 \\ 
 801& 225348.322-084624.58&   7.52&  18.88&  27.29&  54.92&  58.18&  49.34&  40.70&   0.00&  24.40&  17.94&   9.44&   2.02&   0.77&   0.17&   0.15 \\ 
 802& 225506.799+005839.92&  64.86&   0.00& 154.60& 312.10& 343.00& 315.10& 285.40& 226.90& 181.60& 118.60&  56.98&  11.79&   3.40&   0.57&   0.20 \\ 
 803& 230128.246-083355.81&  17.84&  19.16&  24.10&  37.52&  42.01&  36.20&  30.26&   0.00&  19.02&  15.26&  10.59&   1.49&   0.61&   0.24&   0.00 \\ 
 804& 231947.688+004316.07&   5.97&  13.86&  21.04&  41.23&  41.39&  34.86&  29.65&  19.65&  16.88&  11.40&   6.71&   1.47&   0.51&   0.14&   0.17 \\ 
 805& 233712.763-105800.32&  15.75&  43.31& 111.40& 258.90& 264.00& 224.60& 187.40&   0.00& 114.20&  66.77&  32.86&   6.19&   1.98&   0.40&   0.00 \\ 
 806& 234640.250-090754.15&   0.00&   3.98&   7.57&  18.93&  25.55&  23.57&  19.34&   0.00&  11.10&   8.14&   4.94&   0.98&   0.38&   0.00&   0.15 \\ 
 807& 234743.507-103447.41&   0.00&  14.34&  31.27&  79.18&  84.04&  69.21&  57.50&   0.00&  33.31&  21.64&  12.08&   2.60&   0.96&   0.14&   0.00 \\ 
 808& 235355.800-102113.77&   1.85&   4.91&  12.39&  25.94&  25.97&  22.94&  17.18&   0.00&  15.55&   5.89&   5.16&   0.83&   0.29&   0.00&   0.00 \\ 

